ARES: Adaptive, Reconfigurable, Erasure coded, atomic Storage

Atomicity or strong consistency is one of the fundamental, most intuitive, and hardest to provide primitives in distributed shared memory emulations. To ensure survivability, scalability, and availability of a storage service in the presence of failures, traditional approaches for atomic memory emulation, in message passing environments, replicate the objects across multiple servers. Compared to replication based algorithms, erasure code-based atomic memory algorithms has much lower storage and communication costs, but usually, they are harder to design. The difficulty of designing atomic memory algorithms further grows, when the set of servers may be changed to ensure survivability of the service over software and hardware upgrades, while avoiding service interruptions. Atomic memory algorithms for performing server reconfiguration, in the replicated systems, are very few, complex, and are still part of an active area of research; reconfigurations of erasure-code based algorithms are non-existent. In this work, we present ARES, an algorithmic framework that allows reconfiguration of the underlying servers, and is particularly suitable for erasure-code based algorithms emulating atomic objects. ARES introduces new configurations while keeping the service available. To use with ARES we also propose a new, and to our knowledge, the first two-round erasure code based algorithm TREAS, for emulating multi-writer, multi-reader (MWMR) atomic objects in asynchronous, message-passing environments, with near-optimal communication and storage costs. Our algorithms can tolerate crash failures of any client and some fraction of servers, and yet, guarantee safety and liveness property. Moreover, by bringing together the advantages of ARES and TREAS, we propose an optimized algorithm where new configurations can be installed without the objects values passing through the reconfiguration clients.

==> algorithm_atomic_v3.tex <==

			In this section, we present an implementation of the DAPs,  that satisfies the properties in Property~\ref{property:dap},  for a configuration $c$,  with $n$ servers 
			 using a $[n, k]$ MDS coding scheme for storage. We implement an instance of the algorithm in a 
			%Atomicity is always guaranteed. 
 configuration of  $n$ server processes. 
 We store each coded element $c_i$, corresponding to an object  at server $s_i$, where $i=1, \cdots, n$.
			% However, liveness is  guaranteed under the assumption that the number of write operations concurrent with a read  operation is at most $\delta$. The precise definition of concurrency depends on the algorithm itself, and appears later in this section. The \treas{}~algorithm has significantly reduced storage and communication cost, compared to replication, when $\delta$ is limited.
			%
%
%Expressing an atomic algorithm in terms of the DAP primitives serves multiple purposes.
%First, describing an algorithm according to template algorithm $A_1$  allows one to proof
%that the algorithm is \textit{safe} (atomic) 
%% it enables ease of reasoning about the safety of the algorithm  
%% given that atomicity holds if 
%by just showing that the appropriate DAP properties hold, and the algorithm is \textit{live} if the 
%implementation of each primitive is live. 
%Secondly, the safety and liveness proofs for more complex algorithms (like \ares{} in Section \ref{sec:ares}) % algorithm  
%become easier as one may reason on the DAP properties that are satisfied by the primitives used,
%without involving the underlying implementation of those primitives. 
%Moreover, describing a reconfiguration algorithm using DAPs, provides the flexibility 
%to vary the  implementations DAPs from configuration to configuration, as long as the DAPs satisfy certain  properties. 
%%
%%is easier where  complex operations like reconfiguration is done, where the implementation of data-access primitives can vary from one configuration to another,  while
%%hiding the details of the underlying atomic algorithm implementation. 
%%
%%
%%As we show 
%%In Section \ref{sec:algorithm}, we discuss how \ares{} may change the primitives mechanisms
%%such data access primitives allows us to design 
%%a reconfigurable atomic storage service that can utilize different atomic implementation 
%%in each established configuration without affecting the safety guarantees of the service.
%%Such approaches can adapt to the configuration design, and vary the performance of the service
%%based on the environmental conditions.
%% In other words, ABD \cite{ABD96} can be used for 
%%maximum fault tolerance and when majority quorums are used, whereas fast algorithms 
%%similar to the ones presented in \cite{CDGL04, FNP15}, could be used in configurations 
%%that satisfy the appropriate participation bounds. 
%
%
 The implementations of DAP primitives used in \ares{} are shown  
%\nnrev{by implementing the}{the} 
%DAP primitives \nnrev{as}{are implemented} 
in Alg.~\ref{fig:casopt}, and the servers' responses in Alg.~\ref{fig:casopt:server}.
%At a high level, both the read and write operations take two phases to complete (similar to the ABD algorithm).
	%, and each consists of two phases. 
	%As in algorithm $A_1$, a write operation  
%$\pi$,  \nnrev{ the writer  selects}{discovers} the maximum tag $t^*$ from
% a quorum in $\quorums{c}$ by executing $\dagettag{c}$;  creates  a new tag $t_w = tag(\pi) =  (t^*.z + 1, w)$ by 
 %incorporating the writer's own ID; and 
%it performs a $c.\act{put-data}(\tup{t_w, v})$ to propagate that pair to a quorum in $c$.
%A read operation performs $\dagetdata{c}$ to retrieve a tag-value pair, $\tup{\tg{},v}$ form configuration $c$, and then 
%it performs a $c.\act{put-data}(\tup{\tg{},v})$ to propagate that pair to the servers $\servers{c}$. 

%A write operation is similar to the read but before 
%performing the $\act{put-data}$ action it generates a new tag which associates with the value to be written. 
%

%\begin{algorithm}[!ht]
%		\begin{algorithmic}[2]
%			\begin{multicols}{2}
%				{\footnotesize
%					%\Part{Generic Algorithm $A_1$}
%					\Operation{read}{} 
%					%\State $wCounter\gets wCounter+1$
%					\State $\tup{t, v} \gets \dagetdata{c}$
%					\State $\daputdata{c}{ \tup{t,v}}$
%					\State return $ \tup{t,v}$
%					\EndOperation
%					\Statex
%					\Operation{write}{$v$} 
%					%\State $wCounter\gets wCounter+1$
%					\State $t \gets \dagettag{c}$
%					\State $t_w \gets \tup{t.z + 1,  w}$
%					\State $\daputdata{c}{\tup{t_w,v}}$
%					\EndOperation
%					%\EndPart
%				}
%			\end{multicols}
%			\end{algorithmic}
%		\caption{Read and write operations of algorithm template $A_1$}
%		\label{algo:atomicity:generic1}
%		\vspace{-1em}
%	\end{algorithm}
%		\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}	
			\begin{algorithm*}[!ht]
				\begin{algorithmic}[2]
					{\small
					\begin{multicols}{2}
							\State{ at each process $\pr_i\in\idSet$}
							%\remove{
%										{\scriptsize
%				%\Part{Generic Algorithm $A_1$}
%				\Operation{read}{} 
%				%\State $wCounter\gets wCounter+1$
%				\State $\tup{t, v} \gets \dagetdata{c}$
%				\State $\daputdata{c}{ \tup{t,v}}$
%				\State return $ \tup{t,v}$
%				\EndOperation
%				\Statex
%				\Operation{write}{$v$} 
%				%\State $wCounter\gets wCounter+1$
%				\State $t \gets \dagettag{c}$
%				\State $t_w \gets inc(t)$
%				\State $\daputdata{c}{\tup{t_w,v}}$
%				\EndOperation
%				%\EndPart
%			}%}
	
							\Statex
							\Procedure{c.get-tag}{}
							%	\State {\bf send} $(\text{\act{query}},\rdr)$ to every server $s\in \bigcup_{cseq[i]}members(\qs_{cseq[i].conf})$
							\State {\bf send} $(\text{{\sc query-tag}})$ to each  $s\in \servers{c}$
							\State {\bf until}   $\pr_i$ receives $\tup{t_s,e_s}$ from $\left\lceil \frac{n + k}{2}\right\rceil$ servers in $\servers{c}$
							\State $t_{max} \gets \max(\{t_s : \text{ received } \tup{t_s,v_s} \text{ from } s \})$
							\State {\bf return} $t_{max}$
							\EndProcedure
							
							\Statex
							
							\Procedure{c.get-data}{}
							%	\State {\bf send} $(\text{{\sc query}},\rdr)$ to every server $s\in \bigcup_{cseq[i]}members(\qs_{cseq[i].conf})$
								\State {\bf send} $(\text{{\sc query-list}})$ to each  $s\in \servers{c}$
								\State {\bf until}    $\pr_i$ receives $List_s$ from each server $s\in\srvSet_g$ s.t. $|\srvSet_g|=\left\lceil \frac{n + k}{2}\right\rceil$ and  $\srvSet_g\subset \servers{c}$ 
								\State  $Tags_{*}^{\geq k} = $ set of tags that appears in  $k$ lists	\label{line:getdata:max:begin}
								\State  $Tags_{dec}^{\geq k} =$ set of tags that appears in $k$ lists with values
								\State  $t_{max}^{*} \leftarrow \max Tags_{*}^{\geq k} $
                                \State  $t_{max}^{dec} \leftarrow \max Tags_{dec}^{\geq k} $ \label{line:getdata:max:end}
								\If{ $t_{max}^{dec} =  t_{max}^{*}$} 
								    \State  $v \leftarrow $ decode value for $t_{max}^{dec}$
								\EndIf
								%\State $List_M \triangleq \bigcup_{s \in \srvSet_g}  List_s$
								%$\State  $\forall t$, $List_M(t) \triangleq \{ (t, v): (t,v) \in List_M \}$  
								%\State $\forall t$, $T(t') \triangleq \{t: (t,v) \in List_M(t) \wedge t \geq t' \}$
								%\State $t_r \gets \max \{t : (t, *) \in List_M ~\wedge |List_M(t)| \geq k~\wedge |T(t)| \leq \delta \}$
								%\State $v_s\gets \text{decode from }  List_M(t_{r}))$
								\State {\bf return} $\tup{t^{dec}_{max},v}$
							\EndProcedure
							
							\Statex				
							
							\Procedure{c.put-data}{$\tup{\tg{},v})$}
								\State $\Coded = [(\tg{}, e_1), \ldots, (\tg{}, e_n)]$, $e_i = \Phi_i(v)$
								\State {\bf send} $(\text{{\sc write}}, \tup{\tg{},e_i})$ to each $s_i \in \servers{c}$
								\State {\bf until} $\pr_i$ receives {\sc ack} from $\left\lceil \frac{n + k}{2}\right\rceil$ servers in $\servers{c}$
							\EndProcedure
							%\EndPart
							
							
							
%							\Part{write($v$)}\EndPart
%							\Part{\underline{\GetTag}} {
%								\State  Send  $(\QueryTag)$ to all servers $\mathcal{S}$.
%								\State  Await responses from majority
%								\State  Select the max tag  $t^*$
%							}\EndPart
%							\Statex
%							\Part{\underline{\PutData}} {
%								\State $t_w = (t^{*}.z + 1, w)$.  
%								\State $\Coded = [(t_w, c_1), \ldots, (t_w, c_n)]$, $c_i = \Phi_i(v)$
%								\State Send  $(\CodedElementTag, \Coded)$ to all servers $\mathcal{S}$.
%								\State Terminate after $\left\lceil \frac{n + k}{2}\right\rceil$ acks
%							}	\EndPart
							
%							\Statex
%							\Part{read}\EndPart
%							\Part{\underline{\GetData}} {
%								\State  Send $(\QueryList)$ to all servers $\mathcal{S}$.
%								\State  Wait for $\left\lceil \frac{n+k}{2}\right\rceil$ $Lists$ 
%								\State  Select the max tag, $t_r$, the corresponding value, $v_r$, is decodable using the $Lists$; additionally   $t_r$ is among the highest distinct $\delta$ tags received in any $Lists$.
%							}\EndPart	
%							\Statex
%							\Part{\underline{\PutData}} {
%								\State $\Coded = [(t_r, c_1), \ldots, (t_r, c_n)]$, $c_i = \Phi_i(v_r)$
%								\State Send $(\CodedElementTag, \Coded)$ to all servers $\mathcal{S}$.
%								\State Wait for $\left\lceil \frac{n + k}{2}\right\rceil$ acks
%								\State Return $v_r$
%							}	\EndPart
%							
%							
					\end{multicols}
				}
				\end{algorithmic}	
				\caption{DAP implementation 
					%for  template $A_1$ to implement 
					for  \ares{}. }
				\label{fig:casopt}
				\vspace{-1em}
			\end{algorithm*}
		

	\begin{algorithm*}[!ht]
	\begin{algorithmic}[2]
		{\small
		\begin{multicols}{2}
				\State{at each server $s_i \in \mathcal{S}$ in configuration $c_k$}
				\Statex
				\State{\bf State Variables:}%{ 										
					%\Statex $(t_{loc}, v_{loc}) \in \mathcal{T} \times {\mathcal V}$, initially   $(t_0, v_0)$
					%\Statex $status \in \{active, repair\}$, initially $active$
					\Statex $List \subseteq  \mathcal{T} \times \mathcal{C}_s$, initially   $\{(t_0, \Phi_i(v_0))\}$
				%}\EndPart
			
			\Statex
			\Receive{{\sc query-tag}}{$s_i,c_k$}
				\State $\tg{max} = \max_{(t,c) \in List}t$
				\State Send $\tg{max}$ to $q$
			\EndReceive
			\Statex
	
			
			\Receive{{\sc query-list}}{$s_i,c_k$}
				\State Send $List$ to $q$
			\EndReceive
\State
			\Receive{{\sc put-data}, $\tup{\tg{},e_i}$}{$s_i,c_k$}
				\State $List \gets List \cup \{ \tup{\tg{}, e_i}  \}$ 
				\If{$|List| > \delta+1$}
					\State $\tg{min}\gets\min\{t: \tup{t,*}\in List\}$
				%	\Statex
                                              \Statex  ~~~~~~~~/* remove the coded value and retain the tag */
					%\State $List \gets List \backslash~\{\tup{\tg{},e}: \tg{}=\tg{min} ~\wedge~\tup{\tg{},e}\in List\} \cup \{  (  \tg{min}, \bot)  \}$\label{line:server:removemin}
					\State $List \gets List \backslash~\{\tup{\tg{},e}: \tg{}=\tg{min} ~\wedge \tup{\tg{},e}\in List\}$
					\State $List \gets List  \cup \{  (  \tg{min}, \bot)  \}$\label{line:server:removemin}
				\EndIf
				\State  Send {\sc ack} to $q$
			\EndReceive
			
%				\Statex
%				\Part {\underline{\GetTagResp,recv $\QueryTag$ from writer $w$}} {
%					%\If{ $status = active$ }
%					\State $t^* = \max_{(t,c) \in List}t$
%					\State Send $t^*$ to $w$
%					\Statex %\EndIf
%				}\EndPart
%				%										\Statex
%				\Part {\underline{\GetDataResp, recv $\QueryList$ from reader $r$}} {
%					%\If{ $status = active$ }
%					\State Send  $List$ to $r$
%					%\EndIf
%				}\EndPart
%				%	
%				\Statex
%				\Part{ \underline{\PutDataResp, recv $\CodedElementTag, (t, c_i)$ from $p$ }}{
%					%\If{$status = active$}
%					\State $List \leftarrow List \cup \{ (t, c_i)  \}$ 
%					\If{ $|List| > \delta + 1$ } 
%					\State  Retain the (tag, coded-element) pairs for the $\delta +1 $ highest tags in $List$, and delete the rest.
%					\EndIf 
%					\State  Send ack to $p$.
%					%\EndIf
%					
%				}\EndPart
				\end{multicols}
			}
	\end{algorithmic}	
	\caption{The response protocols at  any server $s_i \in {\mathcal S}$ in  
					\ares{} for client requests.}\label{fig:casopt:server}
					\vspace{-1em}
\end{algorithm*}		
 Each server $s_i$ stores one  state variable,  $List$,  which is a set of up to $(\delta + 1)$  (tag, coded-element) pairs. Initially the set at $s_i$ contains a single element, $List = \{ (t_0,  \Phi_i(v_0)\}$.   Below we describe the implementation of the DAPs.
%
%				At a high-level, the algorithm (see Fig.~\ref{fig:casopt}) is a natural generalization of the $ABD$ algorithm accounting for the fact that we use MDS codes.
	
$\dagettag{c}$: A  client,  during the execution of a  $\dagettag{c}$ primitive, queries all the servers in $\servers{c}$ for the highest tags in their  $Lists$, and awaits responses from $\left\lceil \frac{n+k}{2} \right\rceil$ servers.
% with $k \geq \frac{2n}{3}$. 
A server upon receiving the {\sc get-tag} request, 
responds to the client with the highest tag, as $\tg{max} \equiv \max_{(t,c) \in List}t$. 
Once the client receives the tags from $\left\lceil \frac{n+k}{2} \right\rceil$ servers,  it selects  the highest  tag $t$ and returns it . 
							
 $c.\act{put-data}(\tup{t_w, v})$: During the  execution of the primitive  $c.\act{put-data}(\tup{t_w, v})$,  a client 
 % computes the coded elements for each of the $n$ servers, and 
 sends the  pair  $(t_w, \Phi_i(v))$ to each server $s_i\in\servers{c}$.  
 When a server $s_i$ receives a message $(\text{\sc put-data}, t_w, c_i)$ , it adds the pair in its local $List$, 
 trims the pairs with the smallest tags exceeding the length $(\delta+1)$ of the $List$ , and replies 
 with an ack to the client.
 %
 %Every time a $(\text{\sc put-data}, t_w, c_i)$  message arrives at a server $s_i$, 
 %from a writer, 
 %the pair gets added to the $List$. As the size of the $List$ at each $s_i$ is bounded by $(\delta+1)$, then following an insertion in the $List$, $s_i$ trims the coded-elements associated with the smallest tags. 
 In particular, $s_i$ replaces the coded-elements of the older tags with $\bot$, and maintains only the coded-elements associated with the 
 	$(\delta+1)$ highest tags in the $List$ (see Line Alg.~\ref{fig:casopt:server}:\ref{line:server:removemin}).
 %which is then garbage collected to keep tag and coded-element pairs of the highest  $(\delta+1)$ tags, and by replacing the coded-elements of the older tags with $\bot$,  a symbol that signifies garbage-collected coded-elements. 
  The client completes the primitive operation after getting acks from $\left\lceil \frac{n+k}{2} \right\rceil$ servers.
			
	$\dagetdata{c}$:	A  client, during the execution of a  $\dagetdata{c}$ primitive, queries all the servers in $\servers{c}$ for their  local variable $List$, and awaits responses from $\left\lceil \frac{n+k}{2} \right\rceil$ servers. Once the client receives $Lists$ from $\left\lceil \frac{n+k}{2} \right\rceil$ servers,  it selects the highest  tag $t$, such that: $(i)$ its corresponding value $v$ is decodable from the coded elements in the lists; and $(ii)$ $t$ is the highest tag seen from the responses of at least $k$ $Lists$ 
			(see lines Alg.~\ref{fig:casopt}:\ref{line:getdata:max:begin}-\ref{line:getdata:max:end}) and returns the pair $(t, v)$. 
Note that in the case where anyone of the above conditions is not satisfied the corresponding read operation does not complete.
% \newpage
%\begin{theorem} \label{thm:storage_TREAS}
%	The worst-case total storage cost of \treas{} algorithm is  $(\delta +1 )\frac{n}{k}$.
%\end{theorem}
%\proofremove{
%	\begin{proof}
%		The maximum number of  (tag, coded-element) pair in the $List$ is $\delta+1$, and the size of each coded element is 
%		$\frac{1}{k}$ while the tag variable is a metadata and therefore, not counted. So, the total storage cost is $(\delta +1)\frac{n}{k}$.
%	\end{proof}
%}
%
%We next state  the communication cost for the write and read operations in  \treas{}. Once again, note that we ignore the communication cost arising from exchange of meta-data.
%
%\begin{theorem} \label{treas:write_cost}
%	The communication cost associated with a successful  write operation in \treas{} is at most $\frac{n}{k}$. 
%\end{theorem}
%\proofremove{
%	\begin{proof}
%		During read operation, in the $\act{get-tag}$ phase the servers responds with their highest tags variables, which are metadata. However, in the $\act{put-data}$ phase, the reader sends each server the  coded elements of size  $\frac{1}{k}$ each, and hence the total cost of communication for this is $\frac{n}{k}$. Therefore, we have the worst case communication cost of a write operation is $ \frac{n}{k}$.
%	\end{proof}
%}
%\begin{theorem} \label{radonc:read_cost}
%	The communication cost associated with a successful read operation in \treas{} is at most $(\delta +2)\frac{n}{k}$. 
%\end{theorem}
%\proofremove{
%	\begin{proof}
%		During read operation, in the $\act{get-data}$ phase the servers responds with their $List$ variables and hence each such list 
%		is of size at most $(\delta +1)\frac{1}{k}$, and then counting all such responses give us $(\delta +1)\frac{n}{k}$.  In the $\act{put-data}$ phase, the reader sends each server the  coded elements of size  $\frac{1}{k}$ each, and hence the total cost of communication for this is $\frac{n}{k}$. Therefore, we have the worst case communication cost of a read operation is 
%		$(\delta+2) \frac{n}{k}$.
%	\end{proof}
%}
%

\section{Correctness,  performance and latency  of \ares{}}\label{sec:ares_safety}
In this section, we prove the atomicity property of \ares{}. We also provide an analysis of its storage and communication costs, and the 
latency of read and write operations. The atomicity property of \ares{} hinges on the Property~\ref{property:dap} 
of the DAP implementation in each individual configuration used in~\ares{}. Therefore, we start by proving, in subsection~\ref{sec:safety:a},  that 
Property~\ref{property:dap} holds for the DAP implementation in Section~\ref{ssec:dap:impl}. 
Based on this, in subsection ~\ref{sec:safety:b}, we prove the atomicty of \ares{}. Next, in sub-section~\ref{sec:safety:c}, we derive the storage
and communication costs of read and write operations, and in sub-section ~\ref{sec:safety:d}, we derive the latency
of reads and writes in terms of the minimum and maximum delays of any point-to-point messages of the 
underlying network.
Due to lack of space proofs are omitted and can be found in the 
% of the following Theorem is produced in the 
extended version of the paper~\cite{ARES:Arxiv:2018}.	

\subsection{Safety (Property~\ref{property:dap})  proof of the DAP{s}}\label{sec:safety:a}
%\vspace{-1.em}
\myparagraph{Correctness.} 
In this section we are concerned with only one configuration $c$, consisting of a set of servers 
%$\mathcal{S}$
$\servers{c}$.
%, and a set of reader and writer clients $\mathcal{R}$ and $\mathcal{W}$, respectively. In other words, 
%in such static system the sets $\mathcal{S}$, $\mathcal{R}$ and $\mathcal{W}$ are fixed, and 
We assume that at most $f \leq \frac{n-k}{2}$ servers from $\servers{c}$ may crash.  
Lemma~\ref{casflex:data-access:consistent} states that the DAP implementation 
 satisfies the  consistency properties Property~\ref{property:dap}  which will be used to 
%of \treas{}, \nn{and in turn by Theorem \ref{atomicity:A1}} these 
imply the atomicity of the \ares{} algorithm. 
%which implies the atomicity city properties and consequently the
%atomicity property 
%(Theorem~\ref{thm:atomicity_radonc}).			
%\myparagraph{Liveness and Safety Conditions.}\blue{
%The \treas{} algorithm we present satisfy \myemph{wait-free termination} (Liveness) and \myemph{atomicity} (Safety).
%}
	%Due to lack of space the proof of the following Theorem is produced in the Appendix.	
\label{sec:primitives}
\input{tag_primitives_v3.tex}
						
 \begin{theorem}[Safety]\label{casflex:data-access:consistent}
Let $\Pi$ a set of complete DAP operations of Algorithm \ref{fig:casopt} in a configuration $c\in\confSet$,
$\act{c.get-tag}$, $\act{c.get-data}$ and $\act{c.put-data}$,
of an execution $\EX$. Then, every pair of operations $\phi,\op\in\Pi$ satisfy Property \ref{property:dap}.
% The data-access primitives, i.e., $\act{get-tag}$, $\act{get-data}$ and $\act{put-data}$ primitives implemented in any configuration  $c$
% in this section satisfy Property~\ref{property:dap}.
\end{theorem}


\proofremove{
\begin{proof}
As mentioned above we are concerned with only configuration $c$, and therefore, in our proofs we will be concerned with only one
configuration. Let $\alpha$ be some execution of \treas{}, then we consider two cases for $\pi$ for proving property $C1$:  $\pi$ is a  $\act{get-tag}$ operation, or $\pi$ is a $\act{get-data}$ primitive. 

 %\item[ C1 ]  If $\phi$ is a  $\daputdata{c}{\tup{\tg{\phi}, v_\phi}}$, for $c \in \confSet$, $\tg{1} \in\tsSet$ and $v_1 \in \valSet$,
 %and $\pi$ is a $\dagettag{c}$ (or a $\dagetdata{c}$) 

 %that returns $\tg{\pi} \in \tsSet$ (or $\tup{\tg{\pi}, v_{\pi}} \in \tsSet \times \valSet$) and $\phi$ completes before $\pi$ in $\EX$, then $\tg{\pi} \geq \tg{\phi}$.
Case $(a)$: $\phi$ is   $\daputdata{c}{\tup{\tg{\phi}, v_\phi}}$ and  $\pi$ is a $\dagettag{c}$ returns $\tg{\pi} \in \tsSet$. Let $c_{\phi}$ and $c_{\pi}$ denote the clients that invokes $\phi$ and $\pi$ in $\alpha$. Let $S_{\phi} \subset \mathcal{S}$ denote the set of $\left\lceil \frac{n+k}{2} \right \rceil$ servers that responds to $c_{\phi}$, during $\phi$. Denote by $S_{\pi}$ the set of $\left\lceil \frac{n+k}{2} \right \rceil$ servers that responds to $c_{\pi}$, during $\pi$.  Let $T_1$ be a point in execution $\alpha$ 
after the completion of $\phi$ and before the invocation of $\pi$. Because $\pi$ is invoked after $T_1$, therefore, at $T_1$ each of the servers in $S_{\phi}$ contains $t_{\phi}$ in its $List$ variable. Note that, once a tag is added to $List$, it is never removed. Therefore, during $\pi$, any server in $S_{\phi}\cap S_{\pi}$ responds with $List$ containing $t_{\phi}$ to $c_{\pi}$. Note that since  $|S_{\sigma^*}| = |S_{\pi}| =\left\lceil \frac{n+k}{2} \right \rceil $ implies
				 $| S_{\sigma^*} \cap S_{\pi} | \geq k$, and hence $t^{dec}_{max}$ at $c_{\pi}$, during $\pi$ is at least as large as $t_{\phi}$, i.e., $t_{\pi} \geq t_{\phi}$. Therefore, it suffices to to prove our claim with respect to the tags and the decodability of  its corresponding value.


Case $(b)$: $\phi$ is   $\daputdata{c}{\tup{\tg{\phi}, v_\phi}}$ and  $\pi$ is a $\dagetdata{c}$ returns $\tup{\tg{\pi}, v_{\pi}} \in \tsSet \times \valSet$. 
As above, let $c_{\phi}$ and $c_{\pi}$ be the clients that invokes $\phi$ and 
$\pi$. Let $S_{\phi}$ and $S_{\pi}$ be the set of servers that responds to $c_{\phi}$ and $c_{\pi}$, respectively. Arguing as above, 
 $| S_{\sigma^*} \cap S_{\pi} | \geq k$ and every server in  $S_{\phi} \cap S_{\pi} $ sends $t_{\phi}$ in response to $c_{\phi}$, during 
 $\pi$, in their $List$'s and hence $t_{\phi} \in Tags_{*}^{\geq k}$. Now, because $\pi$ completes in $\alpha$, hence we have 
 $t^*_{max} = t^{dec}_{max}$. Note that $\max Tags_{*}^{\geq k} \geq \max Tags_{dec}^{\geq k}$ so 
  $t_{\pi} \geq \max Tags_{dec}^{\geq k} = \max Tags_{*}^{\geq k} \geq t_{\phi}$. Note that each tag is always associated with 
  its corresponding value $v_{\pi}$, or the corresponding coded elements $\Phi_s(v_{\pi})$ for $s \in \mathcal{S}$.

Next, we prove the $C2$ property of DAP for the \treas{} algorithm. Note that the initial values of the $List$ variable in each servers $s$ in $\mathcal{S}$ is 
$\{ (t_0, \Phi_s(v_{\pi}) )\}$. Moreover, from an inspection of the steps of the algorithm, new tags in the $List$ variable of any servers of any servers is introduced via $\act{put-data}$ operation. Since $t_{\pi}$ is returned by a $\act{get-tag}$ or 
$\act{get-data}$ operation then it must be that either $t_{\pi}=t_0$ or $t_{\pi} > t_0$. In the case where $t_{\pi} = t_0$ then we have nothing to prove. If $t_{\pi} > t_0$ then there must be a $\act{put-data}(t_{\pi}, v_{\pi})$ operation $\phi$. To show that for every $\pi$ it cannot be that $\phi$ completes before $\pi$, we adopt by a contradiction. Suppose for every $\pi$, $\phi$ completes before $\pi$ begins, then clearly $t_{\pi}$ cannot be returned $\phi$, a contradiction.
\end{proof}
}			
	\remove{
				\begin{theorem}[Atomicity]  \label{thm:atomicity_radonc}
					Any well-formed and fair execution of \treas{},  is atomic.
				\end{theorem}
		}
	\myparagraph{Liveness.} \label{sec:treas_liveness}
    To reason about the liveness of the proposed DAPs, we define a concurrency parameter $\delta$ which  captures all the  $\act{put-data}$ operations that overlap with the $\act{get-data}$, until the time the client has all data needed to attempt decoding a value. However, we ignore those $\act{put-data}$ operations that might have started in the past, and never completed yet, if their tags are less than that of any $\act{put-data}$ that completed before the  $\act{get-data}$  started. This allows us to ignore $\act{put-data}$ operations due to failed clients, while counting concurrency, as long as the failed $\act{put-data}$ operations are followed by a successful $\act{put-data}$ that completed before the $\act{get-data}$ started. 				
\kmk{In order to define the amount of concurrency  in  our specific implementation of the DAPs presented in this section the}  following definition captures the $\act{put-data}$ operations that overlap with the $\act{get-data}$, until  the client has all data required to  decode the value.
				
\begin{definition}[Valid $\act{get-data}$ operations]
A $\act{get-data}$  operation $\pi$ from a process $p$ is \myemph{valid}  if 
%the associated client 
$p$ does not crash until the reception of $\left\lceil \frac{n+k}{2} \right\rceil$ responses during the{\GetData} phase. 
\end{definition}
					
				
				\begin{definition}[$\act{put-data}$ concurrent with a valid $\act{get-data}$] \label{defn:concurrent}
					Consider a valid $\act{get-data}$ operation $\pi$ from a process $p$. 
					Let $T_1$ denote the point of initiation of $\pi$. For $\pi$, let $T_2$ denote the earliest point of time during the execution when $p$ 
					%the associated client 
					receives all the $\left\lceil \frac{n+k}{2} \right\rceil$ responses.
					% For a valid repair,  let $T_2$ denote the point of time during the execution when the repair completes, and takes the associated server back to the active state. 
					Consider the set $\Sigma = \{ \phi: \phi$ is any $\act{put-data}$ operation that completes before $\pi \text{ is initiated} \}$, and let $\phi^* = \arg\max_{\phi \in \Sigma}tag(\phi)$. Next, consider the set $\Lambda = \{\lambda:  \lambda$  is any $\act{put-data}$ operation that starts before $T_2 \text{ such that } tag(\lambda) > tag(\phi^*)\}$. We define the number of $\act{put-data}$ concurrent with the valid $\act{get-data}$  $\pi$ to be the cardinality of the set $\Lambda$.
				\end{definition}
							
Termination (and hence liveness)  of the DAPs is guaranteed in an execution $\EX$, provided that a process 
	no more than $f$ servers in $\servers{c}$ crash, and no more that $\delta$ $\act{put-data}$ may be concurrent at any point in $\EX$. 
	%in  property of an algorithm,  we mean that 
	If the failure model is satisfied, then any operation invoked by a non-faulty client will collect the necessary replies
	% process terminates  
	independently of the progress of any other client process in the system. Preserving $\delta$ on the other hand,
	ensures that any operation will be able to decode a written value. These are captured in the following theorem:

				\begin{theorem}[Liveness]  \label{thm:liveness_radonc}
					Let $\EX$ be well-formed and fair execution of DAPs, with an $[n, k]$ MDS code, 
					where $n$ is the number of servers out of which no more than $\frac{n-k}{2}$ may crash, 
					%and $k  > n/3$,
					 and $\delta$ be the maximum number of $\act{put-data}$ operations concurrent with any 
					 valid $\act{get-data}$ operation. 
					 Then any $\act{get-data}$ and $\act{put-data}$ operation $\op$ 
					 invoked by a process $\pr$  terminates in $\EX$ if $\pr$
					 does not crash between the invocation and response steps of $\op$.\vspace{-.5em}
				\end{theorem}
		\proofremove{		
				\begin{proof}
				Note that in the read and write operation the  $\act{get-tag}$ and $\act{put-data}$ operations initiated by any non-faulty client  always complete.
				Therefore, the liveness property with respect to any write operation is clear because it uses only  $\act{get-tag}$ and $\act{put-data}$ operations of the DAP. So, we focus on proving the liveness property of any read operation $\pi$, 
				specifically,   the  $\act{get-data}$ operation completes. Let $\alpha $ be and execution of \treas{} and let 
				$c_{\sigma^*}$ and $c_{\pi}$ be the clients that invokes the write operation $\sigma^*$ and 
				read operation $c_{\pi}$, respectively.
				
				Let $S_{\sigma^{*}}$ be the set of 
				$\left\lceil \frac{n+k}{2} \right \rceil$ servers that responds to 
				$c_{\sigma^*}$, in the $\act{put-data}$ operations, in $\sigma^*$.
				 Let $S_{\sigma^{\pi}}$ be the set of $\left\lceil \frac{n+k}{2} \right \rceil$ servers that responds to  $c_{\pi}$ during the  $\act{get-data}$ step of $\pi$. Note that in $\alpha$ at the point execution $T_1$, just before the execution of  $\pi$, none of the the write operations in 
				 $\Lambda$ is complete. Observe that,  by algorithm design, the coded-elements corresponding to  $t_{\sigma^*}$ are garbage-collected from the $List$ variable of a server only if more than $\delta$ higher tags are introduced by subsequent writes into the server.  Since the number of concurrent writes  $|\Lambda|$, s.t.  $\delta > | \Lambda |$ the corresponding value of tag $t_{\sigma^*}$ is not garbage collected in $\alpha$, at least until execution point $T_2$  in  any of the servers in $S_{\sigma^*}$.
				 
				 Therefore, during the execution fragment between the execution points $T_1$ and $T_2$ of the execution $\alpha$, the tag and coded-element pair is present in the $List$ variable of every in $S_{\sigma^*}$ that is active. As a result, the tag and coded-element pairs, $(t_{\sigma^*}, \Phi_s(v_{\sigma^*}))$ exists in the $List$ received from any
				  $s \in S_{\sigma^*} \cap S_{\pi}$ during operation $\pi$. Note that since $|S_{\sigma^*}| = |S_{\pi}| =\left\lceil \frac{n+k}{2} \right \rceil $ hence
				 $| S_{\sigma^*} \cap S_{\pi} | \geq k$ and hence 
				 $t_{\sigma^*} \in Tags_{dec}^{\geq k} $, the set of decodable tag, i.e., the value $v_{\sigma^*}$ can be decoded
				  by $c_{\pi}$ in $\pi$, which demonstrates that $Tags_{dec}^{\geq k}  \neq \emptyset$. Next we want to 
				  argue that 
				  $t_{max}^* = t_{max}^{dec}$ via a contradiction: we assume 
				  $ \max Tags_{*}^{\geq k}  >  \max Tags_{dec}^{\geq k}  $. Now, consider any tag $t$, which  exists due to our assumption,  such that, 
				  $t \in Tags_{*}^{\geq k} $,  $t \not\in Tags_{dec}^{\geq k} $ and $t > t_{max}^{dec}$.
			%	 
				 Let $S^k_{\pi} \subset S$ be any subset of $k$ servers that responds with $t^*_{max}$ in their $List$ variables to $c_{\pi}$. Note that since $k >  n/3$ hence $|S_{\sigma^*} \cap S_{\pi}|  \geq \left\lceil \frac{n+k}{2} \right \rceil +  \left\lceil \frac{n+1}{3} \right \rceil \geq 1$, i.e., $S_{\sigma^*} \cap S_{\pi} \neq \emptyset$. Then $t$ 
				 must be in some servers in $S_{\sigma^*}$ at $T_2$ and since $t > t_{max}^{dec} \geq t_{\sigma^*}$. 
				 Now since $|\Lambda| < \delta$ hence $(t, \bot)$ cannot be in any server at $T_2$  because there are not enough concurrent write operations (i.e., writes in $\Lambda$) to garbage-collect the coded-elements corresponding to tag $t$, which also holds  for tag  $t^{*}_{max}$. In that case, $t$ must be in $Tag_{dec}^{\geq k}$, a contradiction.
%
				\end{proof}
}





==> algorithm_v8.tex <==

\algblockdefx[Operation]{Operation}{EndOperation}%
[2]{{\bf operation} $\act{#1}$(#2)}%
{{\bf end operation}}
\algblockdefx[Procedure]{Procedure}{EndProcedure}%
[2]{{\bf procedure} $\act{#1}$(#2)}%
{{\bf end procedure}}
\algblockdefx[Receive]{Receive}{EndReceive}%
[2]{{\bf Upon receive} (#1)$_{\text{ #2 }}${\bf from} $q$}%
{{\bf end receive}}

In this section, we describe \ares{}.
%As opposed to its predecessors \cite{LS02, AKMS09}, \ares{} 
In the presentation of  \ares{} algorithm
%, compared to its predecessors \cite{LS02, AKMS09}, 
we decouple the reconfiguration service from the shared memory emulation, by utilizing
the DAPs presented in Section \ref{ssec:dap}. This allows \ares{},
to handle both the reorganization of the servers that host the data, as well as utilize 
a different atomic memory implementation per configuration. It is also important to 
note that \ares{} adopts a client-server architecture and separates the reader, writer 
and reconfiguration processes from the server processes that host the object data.
 %
\kmk{More precisely, \ares{} algorithm comprises  of three major components: $(i)$ The reconfiguration protocol which consists
 of invoking, and subsequently installing new configuration via the \act{reconfig} operation by recon clients.
 $(ii)$ The read/write protocol for executing the \act{read} and \act{write} operations invoked by readers and writers.
 $(iii)$ The implementation of the DAPs for each installed configuration 
 that respect 
 %the consistency properties  (
 Property~\ref{property:dap} and 
 which are used by the 
 %on top of which the 
 \act{reconfig}, \act{read} and 
 \act{write} operations. } %are implemented.}
 
%In the rest of the section we first provide the specification of the reconfiguration mechanism used in \ares{},
%along with the properties that this service offers. Then, we discuss the implementation of read and write 
%operations and how they utilize the reconfiguration service to ensure atomicity even in cases where 
%read/write operations are concurrent with reconfiguration operations. The read and write operations are 
%described in terms of the data access primitives presented in Section \ref{ssec:dap} and we show that
%if the DAP properties are satisfied then \ares{} preserves atomicity. This allows \ares{} to deploy the transformation
%of any atomic read/write algorithm \nn{in terms of the presented DAPs} without compromising consistency. 

%show the correctness of \ares{} when using 
% the DAP of two different algorithms: (1) of the classic replication algorithm \mwABD{}, and (2) of the new algorithm \flexCAS{} that uses erasure codes. 
%We show that \ares{} preserves atomicity independently from the DAP it utilizes. 

%will show how our reconfiguration
%service can be combined with 
%%implementations of {\sc get} and {\sc put} primitives 
%a replication algorithm to implement atomic read/write objects,
%and finally we will show how to modify the {\sc get} and {\sc put}
%primitives of the replicated algorithm to allow the use of erasure 
%codes without violating safety.
 
%\paragraph{State Variables} Here we describe the state variables in the writers, readers and servers.
%
%\myemph{Servers}:~ $\tg{}\in\N \times\wSet,~v\in V$

%\paragraph{Preliminaries:} Before proceeding with the description of the algorithm we provide 
%the data types we use and the external services we assume. 
%%Here we describe the state variables in the writers, readers and servers.


%From the definition we can conclude that if a the consensus instance $\consensus{c}$ 
%%runs over a configuration $c$ and 
%decides a value $c_k$ 
%then any subsequent invocation of $Cons[c]$ over the same configuration $c$ will decide $c_k$.  

\subsection{Implementation of the Reconfiguration Service.}
%\vspace{-.5em}
\label{ssec:recbox} 
In this section, we describe the reconfiguration service in \ares{}.
The service relies on an underlying sequence of configurations (\kmk{already proposed or installed 
by \act{reconfig} operations}), 
%which can be  
%\textit{updated} by reconfiguration clients and \textit{read} by any client in $\idSet$. 
%Our service revolves around the idea that configurations are stored in the form of
%Configurations are stored 
%The set of configurations proposed by various reconfiguration clients, by invoking reconfiguration operations, are stored  in the form of 
in the from of a  ``distributed list'', which we refer to as the \myemph{global configuration sequence (or list)} $\gseq$. 
Conceptually, $\gseq$ represents
%The data type \myemph{configuration sequence}  
an ordered list of pairs $\langle c, status \rangle$, where $c$ is a configuration identifier ($ c \in \confSet$),  
 and a binary state variable $status \in \{F, P\}$
%. The variable $status$ associated with $c$,
that denotes whether $c$ is \myemph{finalized} ($F$) or is still \myemph{pending} ($P$). 
\nn{Initially,  $\gseq$ contains a single element, say $\tup{c_0, F}$, 
	%denote the first element of $\gseq$,
	 which is known to every participant in the service.}

\nn{ To facilitate the creation of $\gseq$, each}
server in $\servers{c}$ maintains a local variable $nextC  \in  \{\confSet \cup \{\bot\}\}\times\{P,F\}$, %(to point to the next configuration in $\gseq$), $nextC \in  \{\confSet \cup \{\bot\}\}\times\{P,F\}$,
which is used to point to the configuration that follows $c$ in $\gseq$. 
Initially, at any server  $nextC = \tup{\bot, F}$. Once $nextC$ it is set to a value %in $\confSet$ 
it is never altered.  As we show below, 
at any point in the execution of~\ares{} and in any configuration $c$, the 
%set of values, that are not equal to $\bot$, stored in 
$nextC$ variables of the non-faulty servers  in $c$ that are not equal to $\bot$ agree, i.e., 
 $\{s.nextC : s \in \servers{c} \wedge s.nextC\neq \bot\}$ is either empty of has only one element.
%We use the notation $|\cseq{seq}|$ to denote the length of a sequence.

 Clients discover the configuration that follows a $\tup{c,*}$
in the sequence by contacting a subset of servers in $\servers{c}$ and collecting their $nextC$ variables. 
%Each server in $\servers{c}$ has a variable $nextC$ (one for each configuration), $nextC \in  \{\confSet \cup \{\bot\}\}\times\{P,F\}$,
%which is used to point to the configuration that follows $c$ in $\gseq$. 
Every client in $\idSet$ maintains a local variable $cseq$ that is expected to  be some subsequence of 
$\gseq$.  Initially, at every client the value of  $cseq$ is $\tup{c_0,F}$.
We use the notation $\cseq{x}$ (a caret over some name) to denote state variables
that assumes values from the domain $\{\confSet \cup \{\bot\}\}\times\{P,F\}$. %\nn{[NN: By element you mean the pair here?]} 
 %or $\cseq{config}$, or $\cseq{c}$, etc.

Reconfiguration clients may introduce new configurations,
each associated with a unique configuration identifier from $\confSet$.
 Multiple clients may concurrently attempt to introduce 
different configurations for same next link  in  $\gseq$.
\ares{} uses consensus to resolve such conflicts: 
\nn{a subset of servers in $\servers{c}$, in each configuration $c$,  
%collectively 
implements a distributed consensus service (such as 
  Paxos~\cite{L98}, RAFT~\cite{Raft}) , denoted by $\consensus{c}$. }
%that runs on a subset of servers in the configuration $c$.

%
%We implement $\gseq$ as follows. 
%In any configuration $c$, every server in $\servers{c}$ has a configuration sequence variable $cseq$, 
%initially $\tup{c_0,F}$, where new configurations can be added to the end of the list. 
%Every server in $\servers{c}$ has a variable $nextC$, $nextC \in  \{\confSet \cup \{\bot\}\}\times\{P,F\}$. Initially, at any server  $nextC = \tup{\bot, F}$, and once it is set to a value %in $\confSet$ 
%it is never altered. For any 
%$c \in \confSet$,  at any point in time, all the values of $nextC$, such that $nextC \neq \tup{\bot,F}$, in the processes  in $\servers{c}$ are the same.


% Our service revolves around the idea that configurations are stored in the form of a “distributed linked
%list“ (similar to a block-chain), which we refer to as the \textit{global configuration sequence}, denoted by $\gseq$.
%
%, where reconfig clients introduce new configurations.
%In our setting, we assume throughout an execution of \ares, every configuration is attempted to be reconfigured at most once.
 %
% Multiple  clients may attempt concurrently to introduce 
%a different configuration for the same index $i$ in the $\gseq$.
%\ares{} uses consensus to resolve such conflicts. In particular, each configuration $c$  
%is associated with an external consensus service, denoted by $\consensus{c}$,  
%that runs on a subset of servers in the configuration $c$.
%We use the data-type  $status\in\{F,P\}$, corresponding to a configuration, say $c$,  to denote whether  $c$ is \myemph{finalized} ($F$) 
%or is still \myemph{pending} ($P$).
%Each reconfigurer may change the system configuration by introducing a new configuration identifier. 
%So essentially, $\gseq$
%%The data type \myemph{configuration sequence}  
%is an array  of pairs $\langle c, status \rangle$, where $c \in \confSet$  and $status \in \{F, P\}$. We denote each such pair %\nn{[NN: By element you mean the pair here?]} 
%by the caret over a variable name, e.g., $\cseq{x}$ or $\cseq{config}$, or $\cseq{c}$, etc.
 
% \nnrev{At any point in an execution of \ares{},}{For any  
% $c_i, c_j \in \confSet$, we say that $c_i$ points to $c_j$ %(or there link 
%% (denote as $c_i \rightarrow c_j$)
% %\nn{[NN: This notation conflicts with the before notation we used in the definition of atomicity in the model. Maybe we can remove the definition there to save space and just point the reader to Lynch's book.]} 
% in $\gseq$, in a state $\state$  if at that point in the execution where a   server in $\servers{c_j}$
% %\nn{[NN: I think here does not have to be a majority of servers. A server sets its variable only after consensus has decided]} in $\servers{c_i}$ 
% has $nextC = c_j$. 

%To link a configuration $c_1$ 
%to a configuration $c_2$, a process needs to \textit{inform} (by setting the state variable $nextC$ to $c_2$) 
% we set a state variable ($nextC$) to $c_2$, 
%Each link of the list, say from configuration $c_1$ to $c_2$ is created by setting the $nextC$ state variable to $c_2$,  
%a proper subset of servers in $\servers{c_1}$ for the existence of $c_2$. 
%When a subsequent process wants to retrieve the configuration that follows 
%$c_1$ by contacting a proper set of servers in $\servers{c_1}$.
%Servers maintain a different $nextC$ variable for each configuration, which 
%initially, 
%at any server that are added  the variable $nextC$ 
%is set to $\bot$, as each server may participate in multiple configurations. 
% Each reconfiguration client starts with an initial non-empty configuration sequence $cseq$. In order, for the 
% reconfiguration operation to be successful it is necessary that the initial $cseq$ has a configuration whose $status$ is finalized.
% Each reconfigurer attempts to install a new 
% configuration $c$ in the system whenever it invokes a  $\act{reconfig}(c)$ action. 
 
%Briefly, the $\act{add-config}$ action atomically appends the local configuration sequence of the
%$\recBox$, say $cseq_{box}$, by $\tup{c,P}$ and returns the resulting configuration sequence through the $\act{add-config-ack}$
%action. The \act{read-config} returns $cseq_{box}$ through the associated 
%ack action, and finally the $\act{finalize-config}$ action marks the elements with indices between $start$ and $end$ in $cseq_{box}$
%with $\tup{*,F}$.
The  reconfiguration service consists of two major components: 
$(i)$ \myemph{sequence traversal}, responsible of discovering a  recent configuration in $\gseq$, and 
$(ii)$  \myemph{reconfiguration operation} that installs new configurations in $\gseq$.  

\begin{algorithm*}[!ht]
	%\hrule \F
	\begin{algorithmic}[2]
		\begin{multicols}{2}	{\small
				\Procedure{read-config}{$seq$}
				\State $\mu = \max(\{j: seq[j].status = F\})$	\label{line:readconfig:final}
				%\State $\nu = |cseq|$
				\State $\cseq{c} \gets seq[\mu]$ %.cfg$
				%\State {\bf send} $(\text{{\sc read-config}}, recon_i)$ to each   $s\in \bigcup_{\mu \leq i \leq \nu} \servers{currCfg}$
				\While{$\cseq{c} \neq \bot$}
				%\State {\bf send} $(\text{\act{read-config}}, recon_i)$ to each $s\in \servers{c}$
				%\State {\bf until}  $\forall j,  \mu \leq j\leq \nu$  $\wedge$  
				%$\exists\quo{},  \quo{} \in \quorums{cseq[j].cfg}$ s.t. $ \forall s\in\quo{},  recon_i$  receives $cseq_s$ from $s$ 
				%\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\forall s\in\quo{}, recon_i$  receives $nextC_s$ from $s$
				%\State $ell \gets \max_{cseq'\text{ received }}(|cseq'|)$
				\State $ \cseq{c}' \gets$\act{get-next-config}$(\cseq{c}.cfg)$ 
				\If{$ \cseq{c}' \neq\bot$} 
				\State $\mu\gets \mu+1$				\label{line:readconfig:increment}
				\State $seq[\mu] \gets \cseq{c}'$	\label{line:readconfig:assign}
				\State \act{put-config}$(seq[\mu-1].cfg, seq[\mu])$ 	\label{line:readconfig:put}
				\State $\cseq{c} \gets seq[\mu]$ \label{line:newconfig:assign}
				\EndIf
				\EndWhile
				\State {\bf return} $seq$
				\EndProcedure
				
				\Statex
				
				\Procedure{get-next-config}{$c$}
				\State {\bf send} $(\text{{\sc read-config}})$ to each $s\in \servers{c}$
				\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $rec_i$ receives $nextC_s$ from $\forall s\in\quo{}$
				\If{$\exists s\in \quo{}\text{ s.t. } \status{nextC_s} = F$} 
					\State {\bf return} $nextC_s$
				\ElsIf{$\exists s\in \quo{}\text{ s.t. } \status{nextC_s} = P$} 
						\State {\bf return} $nextC_s$
					\Else
						\State {\bf return} $\bot$
				\EndIf 
				\EndProcedure
				
				\Statex
				
				\Procedure{put-config}{$c, nextC$}
				\State {\bf send} $(\text{{\sc write-config}}, nextC)$ to each $s\in \servers{c}$
				\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $rec_i$ receives {\sc ack} from $\forall s\in\quo{}$
				\EndProcedure	
		}\end{multicols}	
	\end{algorithmic}
	%\hrule \B
	\caption{Sequence traversal at each process $\pr\in\idSet$ of algorithm \ares.}
	\label{algo:parser}
	\vspace{-1em}
\end{algorithm*}

\myparagraph{Sequence Traversal.} 
Any \act{read/write/reconfig} operation $\op$ utilizes the sequence traversal mechanism  to discover the 
latest state of the global configuration sequence, as well as to ensure that such a state is discoverable
by any subsequent operation $\op'$. 
%
\kmk{See Fig.~\ref{fig:reconfig} for an example execution in the 
case of a reconfig operation.} \nn{In a high level, a client starts by 
collecting the $nextC$ variables from a quorum of servers in a configuration $c$,
such that $\tup{c,F}$ is the last  
finalized configuration in that client's local $cseq$ variable (or $c_0$ 
if no other finalized configuration exists). If any server $s$
returns a $nextC$ variable such that $nextC.cfg\neq\bot$,
then the client $(i)$ adds $nextC$ in its local $cseq$, $(ii)$ propagates $nextC$ 
in a quorum of servers in  $\servers{c}$, and $(iii)$ 
repeats this process in the configuration $nextC.cfg$. 
The client terminates when all servers reply with $nextC.cfg=\bot$.} 
%
More precisely, the sequence parsing consists of three actions (see Alg.~\ref{algo:parser}):  
%$(i)$ \act{get-next-config}(), to discover the next configuration, 
%$(ii)$ \act{put-config}(), which \nn{writes back $nextC$ to a quorum of servers},
%%makes sure the at least a majority of the servers in a configuration has $nextC$ to the same configuration 
%and  $(iii)$ \act{read-config}(), which finally returns \nn{the updated configuration sequence}. %a recent configuration in $\gseq$.
%%All three actions are part of the \textit{read/write/reconfig} operations. 
%We do present their specification and implementations 
%% here and we just 
%%refer to them during the description of the \textit{read/write/reconfig} operations. In high level, a $\act{read-config}$ 
%%action starts with a given configuration sequence and tries to append it with the latest installed configurations, a 
%%$\act{put-config}$ action propagates a configuration id to the servers of a given configuration, and lastly a
%%$\act{get-next-config}$ returns the configuration that follows a given configuration. More precisely the three 
%%actions are implemented 
%as follows (Alg.~\ref{algo:parser}):
%%\begin{itemize}
%%	\item 

\act{get-next-config}$(c)$:
	The action $\act{get-next-config}$ returns the configuration that follows $c$ in $\gseq$.
	During  \act{get-next-config}$(c)$, a client sends {\sc read-config}
	messages to all the servers in $\servers{c}$, and waits for replies containing $nextC$
	%. Once a server receives such a message responds with the value  of its $nextC$ variable. 
	%Once it receives replies 
	from a quorum in $\quorums{c}$. If there exists a reply with 
	%that contains a 
	$nextC.cfg\neq\bot$ 
	the action returns $nextC$; otherwise it returns $\bot$.  
	
%	\item 
\act{put-config}$(c, c')$:  
The $\act{put-config}(c, c')$ action propagates $c'$ to a quorum of servers in $\servers{c}$.
     During the action, the client  sends $( \mbox{{\sc write-config}}, c')$ messages,  
	to  the servers in $\servers{c}$ and waits for each server $s$ in some quorum $Q\in\quorums{c}$ to respond. 
	
%	\item 
\act{read-config}$(seq)$: 
	A $\act{read-config}(seq)$  sequentially traverses the installed configurations 
	%in $\gseq$ \nnrev{and  attempts  to set the status of the last configuration in $\gseq$ to $F$}{
	in order to discover the latest state of the sequence $\gseq$. 
	%This action accepts a configuration sequence $seq$ as an input and 
	%traverses the ``links'' between configurations to establish the latest form of the global configuration sequence. 
	At invocation, the client starts with the 
	last finalized configuration $\tup{c, F}$ in the given $seq$ (Line A\ref{algo:parser}:\ref{line:readconfig:final}), 
	%say $c=\config{\cseq{c_{\mu}}}$, 
	and  enters a loop to  traverse  $\gseq$ by  invoking  $\act{get-next-config}(c)$, which returns the next configuration, say $\cseq{c}'$.
	While  $\cseq{c}' \neq \bot$, then: (a) $\cseq{c}'$ is appended at the end of the sequence $seq$;
	(b) a $\act{put-config}(c, \cseq{c}')$ is invoked to inform a quorum of servers in $\servers{c}$  to update the value of their
 $nextC$ variable to $\cseq{c}'$;
	and (c) variable $c$ is set to $\config{\cseq{c}'}$. %and $c’ = \act{get-next-config}(c_r)$. 
%The	$\act{put-config}(c, c_r)$ action is done in order to ensure that subsequent operations will retrieve a link to configuration $c_r$ from $\servers{c}$. 
	%the see the links as the current reconfiguration operations.
	If $\cseq{c}' = \bot$ the loop terminates and the action  \act{read-config} returns $seq$. 
%\end{itemize}


\begin{algorithm*}[!h]
	%\hrule \F
	\begin{algorithmic}[2]
		\begin{multicols}{2}{\small
				\State at each reconfigurer $rec_i$ 
				\State {\bf State Variables:}
				%\State  $\tg{}\in\N^+\times\wSet,~v\in V$
				\State  $cseq[] s.t. cseq[j]\in\confSet\times\{F,P\}$ with members:
				%\State $cseq[j].cfg\in\confSet$, the configuration identifier
				%\State $cseq[j].status\in\{F,P\}$, the configuration status 
				\State {\bf Initialization:} 
				\State $cseq[0] = \tup{c_0,F}$
				%\State $tg{}\gets \tup{0,\bot}, v \gets \bot, cseq[0] = \tup{c_0,F}$
				
				\Statex		
				
				\Operation{reconfig}{c} 
				%\State $wCounter\gets wCounter+1$
				\If {$c \neq \bot$} 		\label{line:install:valid}
				\State $cseq\gets$\act{read-config}$(cseq)$
				\State $cseq \gets \text{\act{add-config}}(cseq, c)$ %\Comment{Read the latest configuration sequence}
				\State $\text{\act{update-config}}(cseq)$
				\State $cseq\gets\text{\act{finalize-config}}(cseq)$
				\EndIf
				\EndOperation
				
				%				\Statex
				%				
				%				
				%				\Procedure{read-config}{$seq$}
				%				\State $\mu = \max(\{j: seq[j].status = F\})$	\label{line:readconfig:final}
				%				%\State $\nu = |cseq|$
				%				\State $c \gets seq[\mu].cfg$
				%				%\State {\bf send} $(\text{{\sc read-config}}, recon_i)$ to each   $s\in \bigcup_{\mu \leq i \leq \nu} \servers{currCfg}$
				%				\While{$c \neq \bot$}
				%				%\State {\bf send} $(\text{\act{read-config}}, recon_i)$ to each $s\in \servers{c}$
				%				%\State {\bf until}  $\forall j,  \mu \leq j\leq \nu$  $\wedge$  
				%				%$\exists\quo{},  \quo{} \in \quorums{cseq[j].cfg}$ s.t. $ \forall s\in\quo{},  recon_i$  receives $cseq_s$ from $s$ 
				%				%\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\forall s\in\quo{}, recon_i$  receives $nextC_s$ from $s$
				%				%\State $ell \gets \max_{cseq'\text{ received }}(|cseq'|)$
				%				\State $nextC \gets$\act{read-next-config}$(c)$ 
				%				\If{$nextC.cfg\neq\bot$} 
				%				\State $\mu\gets \mu+1$				\label{line:readconfig:increment}
				%				\State $seq[\mu] \gets nextC$	\label{line:readconfig:assign}
				%				\State \act{put-config}$(seq[\mu-1].cfg, seq[\mu])$
				%				\State $c \gets seq[\mu].cfg$
				%				\Else
				%				\State $c \gets \bot$
				%				\EndIf
				%				\EndWhile
				%				\State {\bf return} $seq$
				%				\EndProcedure
				
				\Statex	
				\Procedure{add-config}{$seq$, $c$}
				%\State $\mu\gets\max(\{j: cseq[j].status = F\})$
				%\State $\nu \gets |cseq|$
				%\State $\mu'\gets\max(\{j: cseq'[j].status = F\})$
				\State $\nu \gets |seq|$
				\State $c' \gets seq[\nu].cfg$
				\State $d\gets \consensus{c'}.propose(c)$
				\State $seq[\nu+1]\gets \tup{d,P}$ 				\label{line:addconfig:assign}
				\State $\act{put-config}(c', \tup{d,P})$		\label{line:addconfig:put}
				\State  {\bf return} $seq$
				\EndProcedure
				
				\Statex
				
				\Procedure{update-config}{$seq$}
				\State $\mu\gets\max(\{j: seq[j].status = F\})$
				\State $\nu\gets |seq|$ 
				
				\State $M \gets \emptyset$
				\For{$i=\mu:\nu$}
				\State $\tup{t, v}  \gets \dagetdata{\config{seq[i]}}$
				\State $M  \gets M \cup  \{ \tup{\tg{}, v} \}$ \label{line:reconfig:max}
				\EndFor
				\State $\tup{\tg{},v} \gets \max_{t} \{ \tup{t, v}: \tup{t, v} \in M\}$
				%\State $\tup{\tg{},v} \gets \text{\act{get-data}}(cseq, \mu, \nu)$
				\State $seq[\nu].\act{put-data}(\tup{\tg{},v})$
				\EndProcedure
				
				\Statex	
				
				
				\Procedure{finalize-config}{$seq$}
				\State $\nu = |seq|$
				\State $seq[\nu].status \gets F$	\label{line:status:finalize}
				\State $\act{put-config}(seq[\nu-1].cfg, seq[\nu])$
				\State \textbf{return} $seq$ 
				\EndProcedure
				
				%				\Statex	
				%				
				%				\Procedure{read-next-config}{$c$}
				%				\State {\bf send} $(\text{{\sc read-config}})$ to each $s\in \servers{c}$
				%				\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $rec_i$ receives $nextC_s$ from $\forall s\in\quo{}$
				%				\If{$\exists s\in \quo{}\text{ s.t. } nextC_s.cfg\neq\bot$} 
				%				\State {\bf return} $nextC_s$
				%				\Else
				%				\State {\bf return} $\bot$
				%				\EndIf 
				%				\EndProcedure
				%				
				%				\Statex
				%				
				%				\Procedure{put-config}{$c, cfgPtr)$}
				%				\State {\bf send} $(\text{{\sc write-config}}, cfgPtr)$ to each $s\in \servers{c}$
				%				\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $rec_i$ receives {\sc ack} from $\forall s\in\quo{}$
				%				\EndProcedure
				
				%				\Statex
				%				
				%				\Procedure{get-data}{$c$}
				%				%	\State {\bf send} $(\text{{\sc query}},\rdr)$ to every server $s\in \bigcup_{cseq[i]}members(\qs_{cseq[i].conf})$
				%				\State {\bf send} $(\text{{\sc query}})$ to each  $s\in \servers{c}$
				%				\State {\bf until}    $\exists \quo{}, \quo{}\in\quorums{c}$ s.t. 
				%				\State\TT $rec_i$ receives $\tup{t_s,v_s}$ from $\forall s\in\quo{}$ 
				%				\State $t_{max} \gets \max(\{t_s : recon_i \text{ received } \tup{t_s,v_s} \text{ from } s \})$
				%				\State {\bf return} $\{\tup{t_s,v_s}:t_s=t_{max} \wedge ~rec_i \text{ received } \tup{t_s,v_s} \text{ from } s\}$
				%				\EndProcedure
				%				
				%				\Statex	
				%				
				%				\Procedure{put-data}{$c, \tup{\tg{},v})$}
				%				\State {\bf send} $(\text{{\sc write}}, \tup{\tg{},v})$ to each $s \in \servers{c}$
				%				\State {\bf until} $\exists \quo,  \quo \in \quorums{c}$ s.t. $rec_i$ receives {\sc ack} from $\forall s\in\quo{}$
				%				\EndProcedure
				
				%\Statex \red{we need the server part for the reconfigurer}
				
		}\end{multicols}	
	\end{algorithmic}
	%\hrule \B
	\caption{Reconfiguration protocol of algorithm \ares.}
	\label{algo:reconfigurer}
	\vspace{-1em}
\end{algorithm*}

\begin{algorithm*}[!ht]
	%\hrule \F
	\begin{algorithmic}[2]
		\begin{multicols}{2}{\small
			\State at each server $s_i$ in configuration $c_k$
			\State{\bf State Variables:}
			\State  $\tg{}\in\N \times\wSet$, initially, $\tup{0,\bot}$
			\State $v\in V$, intially, $\bot$
			\State $nextC\in \confSet\times \{P,F\}$, initially $\tup{\bot,P}$
			%\State  $msgType\in\{~seen\subseteq\mathcal{V}\cup\{w\}$	
			%\State{\bf Initialization:}
			%\State $\tg{}\gets \tup{0,\bot}, v \gets \bot$
			
			\Statex
			
			\Receive{{\sc read-config}}{$s_i,c_k$}
			\State send $nextC$ to $q$
			\EndReceive
			
			\Statex
			
			\Receive{{\sc write-config}, $cfgT_{in}$}{$s_i,c_k$}
			\If{$nextC.cfg=\bot~\vee~nextC.status=P$} \label{line:server:finalize}
			\State $nextC\gets cfgT_{in}$
			\EndIf
			\State send {\sc ack} to $q$
			\EndReceive
			
%			\Statex	
%			
%			\Receive{{\sc query-tag}}{$s_i,c_k$} %\Comment{Called upon reception of a message}
%				\State $\act{handle-get-tag(c_k)}$
%				%\State send $\tg{}$ to $q$
%			\EndReceive
%			
%			\Statex
%			
%			\Receive{{\sc query}}{$s_i,c_k$}
%				\State $\act{handle-get-data(c_k)}$
%				%\State send $\tup{\tg{}, v}$ to $q$
%			\EndReceive
%			
%			\Statex
%			
%			\Receive{{\sc write}, $\tup{\tg{in}, v_{in}}$}{$s_i,c_k$}
%				\State $\act{handle-put-data(c_k)}$
%%				\If {$\tg{in}> \tg{}$} 	\label{line:server:tg-comparison}
%%					\State  $\tup{\tg{},v}\gets \tup{\tg{in},v_{in}}$ \label{line:server:update}
%%				\EndIf
%%				\State  send  {\sc ack} to $q$ 	\label{line:server:reply}
%			\EndReceive
%	
			
		}\end{multicols}	
	\end{algorithmic}
	%\hrule \B
	\caption{Server protocol of algorithm \ares.}
	\label{algo:server}
	\vspace{-1em}
\end{algorithm*}

\myparagraph{Reconfiguration operation.}
%Consensus is used at the heart of reconfiguration, in order to establish the order on the proposed configurations. 
%	In each configuration $c$, a consensus protocol runs on the servers in  $\servers{c}$, and any reconfiguration client can  
%	propose a configuration $c'\neq c$ on the consensus instance of configuration $c$.
%In particular, 
A reconfiguration operation $\act{reconfig}(c)$, $c \in \mathcal{C}$,  invoked by any reconfiguration client 
$rec_i$, attempts to append $c$ to $\gseq$. \kmk{The set of server processes in $c$ are not a part of any other configuration different 
from $c$.} \nn{In a high-level, $rec_i$ first executes a sequence traversal to discover 
the latest state of $\gseq$. Then it attempts to add the new configuration $c$, at the end of the 
discovered sequence by proposing $c$ in the consensus instance of the last configuration in the sequence. 
The client accepts and appends the decision of the consensus instance (that might be different than $c$).
Then it attempts to transfer the latest value of the read/write object to the latest installed configuration. 
Once the information is transferred, $rec_i$ finalizes the last configuration in its local sequence and 
propagates the finalized tuple to a quorum of servers in that configuration.}
%
The operation consists of four phases, executed consecutively by $rec_i$ (see Alg.~\ref{algo:reconfigurer}): 
%$(i)$  $\act{read-config}$, reads the recent global configuration sequence;  
%$(ii)$ $\act{add-config}$, attempts to append a new configuration $c$;
% $(iii)$ $\act{update-config}$, scans for the most recent object value (w.r.t. their tags)
%  in the set of configurations in its local state variable $cseq$, and writes this value to the most recent 
%  configuration in $cseq$, $(iv)$ $\act{finalize-config}$, sets the $status$ component 
%  of the last tuple  in the local $cseq$ to $F$. More precisely:

$\act{read-config}(seq)$: The phase $\act{read-config}(seq)$ at $rec_i$, reads the recent global configuration 
sequence as described in the sequence traversal. 
%The phase $\act{read-config}(seq)$ at $rec_i$, 
% reads the recent global configuration sequence 
% %client of the system 
% starting with  some initial guess\footnote{An external directory service can be use to get the information on an active configuration. For  more information on this see ~\cite{aguileratutorial}.} of $seq$. %\nn{[NN: Maybe we can add a footnote saying that a guess can be provided by a DNS like service?]}
%% Beginning from the last finalized configuration $c_{\mu}$ in $cseq$, 
%% %that is in $status$ as $P$ , 
%% $\act{read-config}(cseq)$  traverses  the links of the reconfiguration list successively discovering the new configuration from a current one by reading the $nextC$ variable, via request-response phase,   from a quorum of servers from one configuration to another. 
%%The traversal of a link from $c_1$ to $c_2$ is done by calling function $\act{read-next-config}(c_1)$, which essentially request the $nextC$ variables from a quorum of servers in $c_1$ and returns a valid configuration (i.e. $c_2 \neq \bot$) if at least one of the responses return a non-$\bot$, otherwise, it returns $\bot$.
%%Following each $\act{read-next-config}(c_1)$ call that returns a valid configuration, $rec_i$ sends the pair 
%%$\tup{c_1, F}$ to the servers in $c_1$, and awaits acknowledgements from a quorum in $c_1$. The servers
%%receiving $\tup{c_1, F}$ sets is $nextC$ to $\tup{c_1, F}$ and sends an acknowledgement to $rec_i$. This
%%write-back is done in order to ensure that subsequent  reconfig operations can see the links as the current reconfiguration operations. 
%As described above, the $\act{read-config}$ action completes the traversal by returning a possibly 
%extended configuration sequence to $cseq$.

$\act{add-config}(seq, c)$: The $\act{add-config}(seq, c)$ attempts to append a new configuration $c$ to the end of  \nnrev{$\gseq$}{$seq$ (client's view of $\gseq$)}. Suppose the last configuration in $seq$ is $c'$ (with status either $F$ or $P$), then in order to decide the 
most recent configuration, $rec_i$ invokes $\consensus{c'}.propose(c)$, on the consensus object associated with configuration $c'$. 
Let  $d\in\confSet$ be the configuration identifier decided by the consensus service.
If $d \neq c$,  this  implies that another (possibly concurrent) reconfiguration operation, invoked  by a reconfigurer $rec_j\neq rec_i$, proposed and succeeded $d$  as the configuration to follow $c'$.
%imply that $d$ is a another configuration already added into the global configuration sequence, possibly due to another reconfiguration operation by some reconfiguration client.
 In this case, $rec_i$  adopts $d$ as it own propose configuration, by  adding $\tup{d, P}$ to the end of its local $cseq$ (entirely ignoring $c$),
 using the operation $\act{put-config}(c', \tup{d, P})$, and returns the extended configuration $seq$.
 %and continues executing the remaining phases of the reconfiguration operation. 
 %Next, via the 
\remove{
\nn{[NN: We have talked about the action below so we can remove this description.]}

$\act{put-config}(c', \tup{d, P})$:
Once the $cseq$ is appended, $rec_i$ invokes the 
action $c'.\act{put-config}(\tup{d, P})$, to send $\tup{d,P}$ to a quorum of servers in $\servers{c'}$. 
%and awaits
% responses from a quorum; and upon receiving 
%such a message sets the value $nextC$ to $\tup{d, P}$ and responds with an acknowledgement to $rec_i$. 
Finally, $cseq$ is updated to the extended configuration sequence $seq'$ returned by the $\act{add-config}$ action. 
}

$\act{update-config}(seq)$:
Let us denote by $\mu$ the index of the last configuration in the local sequence $cseq$, at $rec_i$, 
such that its corresponding status is 
$F$; and $\nu$ denote the last index of $cseq$.  Next $rec_i$ invokes $\act{update-config}(cseq)$, which 
gathers the tag-value pair corresponding to 
the maximum tag in each of the configurations in $\cseq{cseq[i]}$ for $\mu \leq i \leq \nu$,
and transfers that pair to the configuration that was added by the $\act{add-config}$ action. 
The $\act{get-data}$ and $\act{put-data}$ DAPs are used to transfer the value of the object to the new configuration, 
and they are implemented \nnrev{respectively}{with respect} to the 
%atomic algorithm that is used in each of the 
configuration that is accessed. 
%During the  execution of the procedure  $\act{get-data}(cseq[i])$, $rec_i$ sends requests the tag-value  to all servers  in  $cseq[i]$ and awaits responses from a quorum.  
Suppose $\tup{t_{max}, v_{max}}$  is the tag value pair corresponding to the highest tag among the responses from all the $\nu - \mu + 1$ configurations. Then, 
 $\tup{t_{max}, v_{max}}$  is written to the configuration $d$ via the invocation of  
 $\config{\cseq{cseq[\nu]}}.\act{put-data}(\tup{\tg{max},v_{max}})$.
 
 {\footnotesize
	\begin{figure}[!t]
		\begin{center}
			\includegraphics[width=0.5\textwidth]{ReconFig-v4.png}
			\caption{Illustration of an execution of the reconfiguration steps.}
			\label{fig:reconfig}
		\end{center}
		\vspace{-2.3em}
	\end{figure}
}

\sloppy$\act{finalize-config}(cseq)$:
Once the tag-value pair is transferred, in the last phase of the reconfiguration operation,  $rec_i$ executes %the procedure call 
$\act{finalize-config}(cseq)$, 
%during which, it 
to update the status of the last configuration in $cseq$, say $d = \config{\cseq{cseq[\nu]}}$, to $F$. 
%and writes to a quorum of the penultimate configuration of $cseq$, i.e., $cseq[\nu -1]$ and completes the reconfiguration operation.
The reconfigurer $rec_i$ informs a quorum of servers in the previous configuration $c=\config{\cseq{cseq[\nu-1]}}$, i.e.  in some $Q \in \quorums{c}$, 
about the change of status, by executing the $\act{put-config}(c, \tup{d,F})$ action. 

\myparagraph{Server Protocol.}
Each server  responds to requests from clients (Alg.~\ref{algo:server}). 
A server waits for \nnrev{five}{two} types of messages: {\sc read-config} and  {\sc write-config}.
% {\sc query}, {\sc query-tag}, and {\sc write} messages. 
When a {\sc read-config } message is received for a particular configuration $c_k$, then the server returns $nextC$ variables of the servers in $\servers{c_k}$. %\nn{[NN:again this notation]} 
A {\sc write-config} message attempts to update the $nextC$ variable of the server with a particular tuple $cfgT_{in}$.
A server changes the value of its local $nextC.cfg$ in two cases: (i) $nextC.cfg=\bot$, or (ii) $\status{nextC}= P$.

Fig.~\ref{fig:reconfig} 
%\nn{[NN: this is wrong numbering. probably has to do with the numbering of algorithms]} 
illustrates an example execution of a reconfiguration operation
$\act{recon}(c_5)$. %and the traversal of a concurrent write operation. 
In this example, the reconfigurer $rec_i$ goes through a number of configuration queries (\act{read-next-config})
before it reaches configuration $c_4$ in which a quorum of servers replies with $nextC.cfg=\bot$. 
There it proposes $c_5$ to the consensus object of $c_4$ ($\consensus{c_4}.propose(c_5)$ on arrow 10), and 
once $c_5$ is decided, $\act{recon}(c_5)$ completes after executing $\act{finalize-config}(c_5)$.



%\red{Recent reconfiguration attempts with some 
% configuration is are attempted to be added to the end of the list as the last recent link $c_{\nu}$ to $c$.  The status variable $status$ for such a configuration is set to $P$ in a quorum of servers.
%%
% A reconfig client $rc$, executing $recon(rc)$ executes three main steps. During the first step (  Line XXX $cseq \leftarrow read-config(cseq))$, $rc$ traverses the links of the reconfigurations successively discovering the new configuration from a current one by reading the $nextC$ variable  from a quorum of servers in the current configuration. Note the initial configuration is the final 
% configuration in $cseq$ such that its status is in $F$.
% }
%\blue{
%The reconfiguration protocol aims to install a new configuration and transfer the knowledge from previous configurations
%to the newly installed configuration. In particular, when a reconfiguration is invoked, the reconfigurer issues an 
%$\act{add-config}(c)$ action to the $\recBox$ attempting to add its proposed configuration to the configuration sequence
%stored in the $\recBox$. The $\recBox$ atomically appends its local configuration sequence and returns the appended 
%configuration sequence, $cseq$, to the reconfigurer. Notice that the newly added configuration $c$ appears as the last 
%element of the sequence $cseq[|cseq|]=\tup{c,P}$.
%%
%We assume a consensus service that can be executed by the members of a configuration. In each configuration
%$k$ we run a consensus instance to agree on the configuration id of $k+1$. The servers maintain a $cseq$ 
%array and are queried for the configuration identifier in a particular index.  
%}
%\paragraph{State Variables} Here we describe the state variables in the writers, readers and servers.
%
%\myemph{Servers}:~ $\tg{}\in\N \times\wSet,~v\in V$
%		%$cseq[~]$, array with elements in $\confSet\times\{F,P\}$ with members:
%		%	$cseq[i].conf\in\confSet$, the configuration identifier
%		%	 $cseq[i].status\in\{F,P\}$, the pending or finalized status 


%
%\begin{algorithm}[!ht]
%	\caption{$\rdIOA{\text{ReconBox}}{}$ Automaton: Signature of the ReconBox service} \label{ioa:reconbox-sig}
%	\begin{algorithmic}[2]
%		\begin{multicols}{2}{\small
%%				
%%				\State {\bf Data Types:}
%%				\State\T $\msgSet \subseteq \{\text{\sc{read},\sc{write}\}}\times\tup{\Nat\times\valSet}\times\Nat$
%%				
%%				\Statex
%%				
%				\Part{Signature}{ \label{line:reconbox-sig}
%				%	\State {\bf Input:}
%					\State\T $\act{add-config}(c), c\in \confSet$
%					\State\T $\act{read-config}$
%					\State\T $\act{finalize-config}(start, end)$, ~$start,end\in \N^+$
%					
%				%	\Statex
%					
%				%	\State {\bf Output:}
%					%\State\T $\act{add-config-ack}(cseq)$, $cseq[i]\in\confSet\times\{F,P\}, 0\leq i \leq |cseq|$
%					%\State\T $\act{read-config-ack}(cseq)$, ~$cseq[i]\in\confSet\times\{F,P\}, 0\leq i \leq |cseq|$
%					%\State\T $\act{finalize-config-ack}$ 
%	%				\State {\bf Internal:}
%				}\EndPart \label{line:reconbox-sig-end}
%		}\end{multicols}
%	\end{algorithmic}	
%\end{algorithm}


%Let the  $\act{recon}(c_5)$ operation be invoked by a reconfigurer $rec_i$. 
%%and the write operation by %$\act{read-next-config}(c_3)$ step executed by 
%%some writer $w$.
%During the first round of communication (arrow 1 in figure), $rec_i$ queries a quorum of servers in $c_0$ (noted by $Q_0$) and finds
%out $c_1$ as the next configuration (i.e. the link $c_0$ to $c_1$ in the global configuration sequence),
%via $\act{read-next-config}(c_0)$ 
%. %(arrow heads 1 and 2). 
%That is, at least a single server in the quorum $Q_0$ replied with $nextC$, where $nextC.cfg=c_1$ to $rec_i$.
%Next, in the second round of communication, $rec_i$ writes back $c_1$ to some 
%quorum in $c_0$ via the step $\act{put-config}(c_0, c_1)$ (see arrow 2).  In the subsequent steps $rec_i$ 
%communicates with configurations $c_1$, $c_2$ and $c_3$, in a similar manner like the above two communication rounds for $c_0$ (see arrows 3-8). 
%However,  in the first communication round with servers in  $c_4$, $rec_i$ discovers that all servers in a quorum of 
%servers in $c_4$ replied with 
%%the $nextC$ returned from
%$nextC$ such that $nextC.cfg=\bot$ (arrow 9). In other words, a link from $c_4$ to another configuration is not discovered by $rec_i$. As a result, 
%$rec_i$ proposes $c_5$ to the consensus object in $c_4$, i.e.,  it invokes $\consensus{c_4}.propose(c_5)$ (arrow 10) and 
%$\consensus{c_4}.propose(c_5)$ returns $c_5$, i.e., $c_5$ is decided as the next configuration after $c_4$. Next, $rec_i$ writes $c_5$ to a 
%quorum of servers in $c_4$ via the $\act{put-config}(c_4, c_5)$ (arrow 11), and completes the operation after executing $\act{finalize-config}(c_5)$. 
%Writer $w$  
%%happens to 
%starts its operation 
%%and the 
%with an initial guess of $cseq$ 
%%it starts with has 
%that contains $c_3$ as the last 
%configuration with 
%%its corresponding 
%a $status$ as $F$. With the two rounds of communication  (arrow heads a, b, c and d) with the servers in $c_3$,
%$w$ discovers $c_4$. However, similar communication rounds with the servers in $c_4$ returns $\bot$, i.e.,  $\act{read-next-config}(c_4)$ returns $\bot$.

%To install a new configuration the reconfigurer has to execute the following steps: (i) attempt to add the 
%new configuration, (ii) transfer the latest data to the new configuration, and (iii) mark the new configuration 
%as finalized. Below we describe each action separately: 
%\begin{itemize}
%	\item \myemph{add-config}: The \act{add-config}(c) action attempts to add the proposed configuration $c$ at 
%	the end of the current configuration sequence. In brief, a new configuration is added by following these steps:
%	(i) perform a read-config at a guessed configuration and by following the finalized configurations try to establish 
%	a sequence with a single finalized and a set of pending configs, (ii) propose $c$ by running consensus on the 
%	last discovered configuration (trying to establish the immediately next config), and (iii) once you receive the 
%	decided configuration propagate the new sequence to the latest config.
%\end{itemize}
%
%The read-config operation needs to have a mechanism to discover the latest finalized configuration. 
%Thus when we try to read the configuration sequence from 
%
%The reconfigurer finalizes the last configuration in its $cseq$ as this is the last configuration he added. 
%To do so he first sets the status of the last configuration, say $c$, to $F$ and propagates its local $cseq$ 
%to the following configurations in sequence: (i) contacts a quorum in $c$, and then (ii) contacts a quorum in 
%$cseq[\mu]$, where $\mu$ is the last finalized configuration of $cseq$ (before $c$). This way we ensure that



%\subsection{\ares{} over a Replicated Atomic Read/Write Object}
%\label{ssec:replicated} 

%To demonstrate that the reconfiguration service provides sufficient properties to implement 
%a reconfigurable atomic read/write object, we first present  an algorithm 
%where the distributed object is replicated among the set of servers. 
%The read and write operations (Algorithms \ref{algo:writer} and \ref{algo:reader}) are similar
%to the two phase classic algorithm of \cite{ABD96}, when they are not concurrent with a reconfiguration operation. 


\begin{algorithm*}[!ht]
	%\hrule \F
	\begin{algorithmic}[2]
		\begin{multicols}{2}{\small
				\Part{Write Operation}
				\State at each writer $w_i$ 
				%\State {\bf State Variables:}
				%\State  $\tg{},\tg{max}\in\N^+\times\wSet,~v\in V, terminate\in\{true,false\}$
				%\State  $cseq[~]$, array with elements in $\confSet\times\{F,P\}$ with members:
				%\State\T $cseq[i].conf\in\confSet$, the configuration identifier
				%\State\T $cseq[i].status\in\{F,P\}$, the pending or finalized status 
				%\State {\bf Initialization:} 
				%\State $\tg{}\gets \tup{0,w_i}$
				%\State $v \gets \bot$
				%\State $cseq[0] = \tup{c_0,F}, terminate={\bf false}$
				\State {\bf State Variables:}
				%\State  $\tg{}\in\N^+\times\wSet,~v\in V$
				\State  $cseq[] s.t. cseq[j]\in\confSet\times\{F,P\}$ with members:
				%\State\T $cseq[j].cfg\in\confSet$, the configuration identifier
				%\State\T $cseq[j].status\in\{F,P\}$, the configuration status 
				\State {\bf Initialization:} 
				\State $cseq[0] = \tup{c_0,F}$
				
				\Statex		
				
				\Operation{write}{$val$}, $val \in V$ 
				%\State $wCounter\gets wCounter+1$
				\State $cseq\gets$\act{read-config}($cseq$)  \label{line:writer:readconfig} %\Comment{Read the latest configuration sequence}
				\State $\mu\gets\max(\{i: cseq[i].status = F\})$ \label{line:writer:lastfin}
				\State $\nu\gets |cseq|$ 
				\For{$i=\mu:\nu$}
				\State $\tg{max} \gets \max(\config{cseq[i]}.\act{get-tag}(), \tg{max})$  \label{line:writer:max}
				\EndFor
				\State $\tup{\tg{},v} \gets \tup{ \tup{\tg{max}.ts+1, \wrt_i}, val}$ \label{line:writer:increment}
				\State $done \gets false$
				\While{{\bf not} $done$} \label{line:writer:whilebegin}
				\State $\config{cseq[\nu]}.$\act{put-data}$(\tup{\tg{},v})$ \label{line:writer:prop}
				\State $cseq\gets$\act{read-config}($cseq$)
				\If{$|cseq| = \nu$}
				\State $done \gets  true$
				\Else
				\State $\nu\gets |cseq|$ \label{line:writer:whileend}
				\EndIf
				\EndWhile
				\EndOperation
				\EndPart
				
				\Part{Read Operation}
				\State at each reader $\rdr_i$ 
				\State {\bf State Variables:}
				\State  $cseq[] s.t. cseq[j]\in\confSet\times\{F,P\}$ with members:
				%			\State\T $cseq[j].cfg\in\confSet$, the configuration identifier
				%			\State\T $cseq[j].status\in\{F,P\}$, the configuration status 
				\State {\bf Initialization:} 
				\State $cseq[0] = \tup{c_0,F}$
				
				\Statex
				
				\Operation{read}{ } 
				%\State $wCounter\gets wCounter+1$
				\State $cseq\gets$\act{read-config}($cseq$)  \label{line:reader:readconfig}%\Comment{Read the latest configuration sequence}
				\State $\mu\gets\max(\{j: cseq[j].status = F\})$ \label{line:reader:lastfin}
				\State $\nu\gets |cseq|$ 
				\For{$i=\mu:\nu$} \label{line:rw:getdata:start}
				\State $\tup{\tg{},v} \gets \max(\config{cseq[i]}.\act{get-data}(), \tup{\tg{},v})$ \label{line:reader:max}
				\EndFor \label{line:rw:getdata:end}
				\State $done\gets {\bf false}$
				\While{{\bf not} $done$}  \label{line:reader:whilebegin}
				\State $\config{cseq[\nu]}.\act{put-data}(\tup{\tg{},v})$ \label{line:reader:prop}
				\State $cseq\gets$\act{read-config}($cseq$)
				\If{$|cseq| = \nu$}
				\State $done \gets  true$
				\Else
				\State $\nu\gets |cseq|$ \label{line:reader:whileend}
				\EndIf
				\EndWhile
				\State {\bf return} $v$
				\EndOperation
				\EndPart
				
				%		\Procedure{get-tag}{$c$}
				%		%	\State {\bf send} $(\text{\act{query}},\rdr)$ to every server $s\in \bigcup_{cseq[i]}members(\qs_{cseq[i].conf})$
				%		\State {\bf send} $(\text{{\sc query-tag}})$ to each  $s\in \servers{c}$
				%		\State {\bf until}    $\exists \quo{}, \quo{}\in\quorums{c}$ s.t. 
				%		\State\TT$\wrtr_i$ receives $\tup{t_s,v_s}$ from $\forall s\in\quo{}$ 
				%		\State $t_{max} \gets \max(\{t_s : \wrtr_i \text{ received } \tup{t_s,v_s} \text{ from } s \})$
				%		\State {\bf return} $t_{max}$
				%		\EndProcedure
				%		
				%		\Statex				
				%		\Procedure{put-data}{$c, \tup{\tg{},v})$}
				%		\State {\bf send} $(\text{{\sc write}}, \tup{\tg{},v})$ to each $s \in \servers{c}$
				%		\State {\bf until} $\exists \quo,  \quo \in \quorums{c}$ s.t. $\wrtr_i$ receives {\sc ack} from $\forall s\in\quo{}$
				%		\EndProcedure
				%		
				%		
				%		\Statex
				
				%		\Procedure{read-config}{$seq$}
				%		\State $\mu = \max(\{j: seq[j].status = F\})$	\label{line:readconfig:final}
				%		%\State $\nu = |cseq|$
				%		\State $c \gets seq[\mu].cfg$
				%		%\State {\bf send} $(\text{{\sc read-config}}, recon_i)$ to each   $s\in \bigcup_{\mu \leq i \leq \nu} \servers{currCfg}$
				%		\While{$c \neq \bot$}
				%		%\State {\bf send} $(\text{\act{read-config}}, recon_i)$ to each $s\in \servers{c}$
				%		%\State {\bf until}  $\forall j,  \mu \leq j\leq \nu$  $\wedge$  
				%		%$\exists\quo{},  \quo{} \in \quorums{cseq[j].cfg}$ s.t. $ \forall s\in\quo{},  recon_i$  receives $cseq_s$ from $s$ 
				%		%\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\forall s\in\quo{}, recon_i$  receives $nextC_s$ from $s$
				%		%\State $ell \gets \max_{cseq'\text{ received }}(|cseq'|)$
				%		\State $nextC \gets$\act{get-next-config}$(c)$ 
				%		\If{$nextC.cfg\neq\bot$} 
				%		\State $\mu\gets \mu+1$				\label{line:readconfig:increment}
				%		\State $seq[\mu] \gets nextC$	\label{line:readconfig:assign}
				%		\State \act{put-config}$(seq[\mu-1].cfg, seq[\mu])$
				%		\State $c \gets seq[\mu].cfg$
				%		\Else
				%		\State $c \gets \bot$
				%		\EndIf
				%		\EndWhile
				%		\State {\bf return} $seq$
				%		\EndProcedure
				%		
				%		\Statex		
				%		
				%		\Procedure{get-next-config}{$c$}
				%		\State {\bf send} $(\text{{\sc read-config}})$ to each $s\in \servers{c}$
				%		\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\wrtr_i$ receives $nextC_s$, $\forall s\in\quo{}$
				%		\If{$\exists s\in \quo{}\text{ s.t. } nextC_s.cfg\neq\bot$} 
				%		\State {\bf return} $nextC_s$
				%		\Else
				%		\State {\bf return} $\bot$
				%		\EndIf 
				%		\EndProcedure
				%		
				%		\Statex
				%		
				%		\Procedure{put-config}{$c, cfgPtr)$}
				%		\State {\bf send} $(\text{{\sc write-config}}, cfgPtr)$ to each $s\in \servers{c}$
				%		\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\wrtr_i$ receives {\sc ack} from $\forall s\in\quo{}$
				%		\EndProcedure
		}\end{multicols}	
	\end{algorithmic}
	%\hrule \B
	\caption{Write and Read protocols at the clients for \ares.}
	\label{algo:writer}
	\vspace{-1em}
\end{algorithm*}
\subsection{Implementation of Read and Write operations.}
The read and write operations in \ares{} are expressed in terms of the DAP primitives  (see 
Section \ref{ssec:dap}). 
%A read  consists of  an execution of  $\act{get-data}$ primitive followed by a $\act{put-data}$ primitive,
%while a write consists of calls to $\act{get-tag}$ and  $\act{put-data}$ primitives. 
This provides the flexibility to \ares{} to use different implementation of DAP primitives in different configurations, without changing the basic structure of  \ares{}. 
At a high-level, a \act{write} (or \act{read})  operation is executed where the client: $(i)$ obtains the \textit{latest configuration sequence} by using the 
$\act{read-config}$ action of the reconfiguration service, $(ii)$ queries  the configurations, in $cseq$, starting from the last finalized configuration
to the end of the discovered configuration 
sequence, for the latest $\tup{tag,value}$ pair with a help of $\act{get-tag}$ (or $\act{get-data}$) operation \nn{as specified for each configuration}, and 
$(iii)$ repeatedly propagates  a new $\tup{tag', value'}$ pair (the largest $\tup{tag,value}$ pair)   with $\act{put-data}$ in the last configuration of its local sequence, until no additional configuration is observed. 
%Now
%{\sc get} and {\sc put} primitives 
%we  describe the execution 
In more detail, the algorithm of a  read or write operation $\pi$ is as follows (see Alg.~\ref{algo:writer}): 
%The server keeps a passive behavior and replies to any message it receives. 


%Here we present the read and write operations in more detail. 
%As we presented in Section \ref{sec:primitives}, for an algorithm to 
%preserve atomicity it needs to satisfy some properties on the 
%implementation of its {\sc get} and {\sc put} primitives. 

%Those primitives are implemented in our replication algorithm as follows:
%\begin{itemize}
%	\item {\sc get-tag}$(c)$: Send {\sc query-tag} messages to all the servers in $\servers{c}$ and wait 
%	for each server $s$ in a quorum $Q\in\quorums{q}$ to reply with its local $\tg{s}$. Find and return the 
%	maximum of those tags. 
%	\item {\sc get-data}$(c)$: Send {\sc query} messages to all the servers in $\servers{c}$ and wait 
%	for each server $s$ in a quorum $Q\in\quorums{q}$ to reply with its local $\tup{\tg{s}, v_s}$ pair. 
%	Find the maximum of those tags, say $\tg{s'}$, and return the pair received by $s'$, $\tup{\tg{s'},v_{s'}}$.
%	\item {\sc put-data}$(c, \tup{\tg{},v})$: Send {\sc write-tag} messages, along with the  $\tup{\tg{},v}$ pair, 
%	to all the servers in $\servers{c}$ and wait for each server $s$ in a quorum $Q\in\quorums{q}$ to reply with an {\sc ack}. 
%\end{itemize}


A write (or read) operation is invoked at a client  $\pr$ when line~Alg.~\ref{algo:writer}:\ref{line:writer:readconfig} %for the writer  
(resp. line~Alg.~\ref{algo:writer}:\ref{line:reader:readconfig}) is executed.  
%for reader),
At first, $\pr$ issues a $\act{read-config}$ action to obtain the latest 
introduced configuration in $\gseq$, in both operations. 
%Note that each process contains a state 
%variable $cseq$ which initially contains the initial configuration $\tup{c_0,F}$. 
%Starting with a guess, $cseq$, for the latest global configuration sequence,
%As shown in the reconfiguration service, 
%process $\pr$ queries a quorum in each configuration $\config{cseq[i]}$, for $\max(j:\status{cseq[j]}=F)\leq i \leq |cseq|$,
%to discover newly introduced and/or newly finalized configurations, during the $\act{read-config}$ action. 

%We assume that each configuration has enough active servers to allow 
%$\pr$ to make progress	even when some configuration is has been replaced 
%by a newer configuration. 
%In case a system wants to garbage collect or decommission inactive servers,
%then a service similar to DNS can be used to provide an estimate of 
%the latest finalized configuration. Notice that such a service would affect 
%the liveness and not the safety of our current implementation so we do 
%not get into details on how such a service can be implemented in this paper. 

\nn{If $\op$ is a \act{write} %(resp. Alg.~\ref{algo:writer}:\ref{line:reader:lastfin} if $\op$ is a  read), 
	$\pr$ detects the last finalized entry in $cseq$, 
	say $\mu$, and performs a $cseq[j].conf.\act{get-tag}()$ action,
	for $\mu\leq j\leq|cseq|$ (line Alg.~\ref{algo:writer}:\ref{line:writer:lastfin}). Then $\pr$ discovers the
	\textit{maximum tag} among all the returned tags ($\tg{max}$),
	and it increments the maximum tag discovered 
	(by incrementing the integer part of $\tg{max}$), generating a new tag, say $\tg{new}$. It assigns 
	$\tup{\tg{}, v}$ to $\tup{\tg{new}, val}$, where $val$ is the
	value he wants to write (Line Alg.~\ref{algo:writer}:\ref{line:writer:increment}).}

\nn{
if $\op$ is a \act{read}, 
$\pr$ detects the last finalized entry in $cseq$, 
say $\mu$, and performs a  $cseq[j].conf.\act{get-data}()$ action, 
for $\mu\leq j\leq|cseq|$ (line Alg.~\ref{algo:writer}:\ref{line:reader:lastfin}). Then $\pr$ discovers the
\textit{maximum tag-value} pair ($\tup{\tg{max},v_{max}}$) among the replies, 
and assigns $\tup{\tg{}, v}$ to $\tup{\tg{max},v_{max}}$.}

%In lines Alg.~\ref{algo:writer}:\ref{line:writer:lastfin} if $\op$ is a write (resp. Alg.~\ref{algo:writer}:\ref{line:reader:lastfin} if $\op$ is a  read), 
% $\pr$ detects the last finalized entry in $cseq$, 
%say $\mu$, and performs a $cseq[j].conf.\act{get-tag}()$ action if $\op$ is a \act{write}, or $cseq[j].conf.\act{get-data}()$ action if $\op$ is a \act{read}, 
%for $\mu\leq j\leq|cseq|$. Then $\pr$ discovers the
%maximum tag among all the returned tags ($\tg{max}$) or tag-value pairs ($\tup{\tg{max},v_{max}}$) respectively.
%%sends \textit{query} messages to all the members of each configuration $cseq[j].conf$, for $\mu\leq j\leq|cseq|$.
%%Notice that any configuration $cseq[j].cfg$,  for $\mu< j\leq|cseq|$, is in a pending state and thus $cseq[j].status = P$.
%%When the client receives replies from a quorum in each configuration $cseq[j].cfg$, it discovers the maximum 
%%$\tup{\tg{max},v_{max}}$ among those replies (Lines A\ref{algo:writer}:\ref{line:writer:max} and A\ref{algo:reader}:\ref{line:reader:max}). 
%If $\op$ is a \act{write}, $\pr$ increments the maximum tag discovered 
%(by incrementing the integer part of $\tg{max}$), generates a new tag, say $\tg{new}$, and assigns 
%$\tup{\tg{}, v}$ to $\tup{\tg{new}, val}$, where $val$ is the
%value he wants to write (Line Alg.~\ref{algo:writer}:\ref{line:writer:increment}). If $\op$ is a \act{read}, then $\pr$ assigns 
%$\tup{\tg{}, v}$ to $\tup{\tg{max},v_{max}}$, i.e.,  the maximum discovered tag-value pair.
%

Once specifying the $\tup{\tg{}, v}$ to be propagated, both reads and writes 
% if $\op$ is a read, $\pr$ 
 %does the following until no new configuration is discovered: (i) 
execute the $\config{cseq[\nu]}.\act{put-data}(\tup{\tg{}, v})$ action, where $\nu=|cseq|$, 
%to a quorum in the last configuration in $cseq$, 
followed by executing  $\act{read-config}$ action, to examine whether new configurations were 
introduced in $\gseq$. The repeat these steps until no new configuration is discovered (lines  Alg.~\ref{algo:writer}:\ref{line:writer:whilebegin}--\ref{line:writer:whileend},
or lines  Alg.~\ref{algo:writer}:\ref{line:reader:whilebegin}--\ref{line:reader:whileend}).
%retrieving a config
Let $cseq'$ be the sequence returned by the $\act{read-config}$ action. 
If $|cseq'| = |cseq|$ then no new configuration is introduced, and
the read/write operation terminates; otherwise, $\pr$ sets $cseq$ to $cseq'$ and repeats the two actions. 
Note,  in an execution of  \ares,  two consecutive $\act{read-config}$ 
operations that return $cseq'$ and $cseq''$ respectively must hold that $cseq'$ is a prefix of $cseq''$,
and hence $|cseq'|=|cseq''|$ only if $cseq' = cseq''$.  Finally, if $\pi$ is a read operation the value with the highest
tag discovered is returned to the client.

\nnfix{\myparagraph{Discussion} \ares{} shares similarities with previous algorithms like RAMBO \cite{GLS03} and 
	the framework  in \cite{spiegelman:DISC:2017}. The reconfiguration technique used in \ares{} ensures the prefix property 
	on the configuration sequence (resembling a blockchain data structure \cite{N08bitcoin}) while the array structure in RAMBO allowed 
	nodes to maintain an incomplete reconfiguration history. 
	%While in RAMBO recon operation needed to write in both the old and the new configurations due to the possible non-continuity of the 
	%known configurations in the config array, in ARES the prefix property of the configuration sequence 
	%allows each recon operation to write only to the latest configuration it discovered. 
	On the other hand, the DAP usage, 
	%enables \ares{} to be oblivious on the underlying atomic memory implementation in each configuration. This 
	exploits a different viewpoint compared to \cite{spiegelman:DISC:2017}, allowing implementations of 
	atomic read/write registers without relying on strong objects, like ranked registers \cite{GD05}.	
	%	where the authors focus to provide a general framework 
	%	for reconfigurations that led to the use of read-write-modify objects, like ranked registers \cite{GD05},
	%	for the implementation of linearizable read/write objects.  
} 

%\vspace{-0.25em}
%\label{sec:correct}
%\input{correctenss_v3.tex}

%\paragraph{Read operation.}
% In the case of a read operation, the client just assigns its
%local tag-value pair to be equal to the maximum pair discovered (Line  A\ref{algo:reader}:\ref{line:reader:max}). 

%\begin{algorithm}[!ht]
%	%\hrule \F
%	\begin{algorithmic}[2]
%		\begin{multicols}{2}{\scriptsize
%				\State at each reader $\rdr_i$ 
%			%	\State {\bf State Variables:}
%			%	\State  $\tg{}\in\N^+\times\wSet,~v\in V, terminate\in\{true,false\}$
%			%	\State  $cseq[] s.t. cseq[j]\in\confSet\times\{F,P\}$ with members:
%			%	\State\T $cseq[j].conf\in\confSet$, the configuration identifier
%			%	\State\T $cseq[j].status\in\{F,P\}$, the pending or finalized status 
%			%	\State {\bf Initialization:} 
%			%	\State $tg{},\tg{max}\gets \tup{0,\bot}, v \gets \bot$
%			%	\State $cseq[0] = \tup{c_0,F}, terminate={\bf false}$
%				\State {\bf State Variables:}
%			%\State  $\tg{}\in\N^+\times\wSet,~v\in V$
%			\State  $cseq[] s.t. cseq[j]\in\confSet\times\{F,P\}$ with members:
%			\State\T $cseq[j].cfg\in\confSet$, the configuration identifier
%			\State\T $cseq[j].status\in\{F,P\}$, the configuration status 
%			\State {\bf Initialization:} 
%			\State $cseq[0] = \tup{c_0,F}$
%				
%				\Statex		
%				
%				\Operation{read}{ } 
%				%\State $wCounter\gets wCounter+1$
%				\State $cseq\gets$\act{read-config}($cseq$) %\Comment{Read the latest configuration sequence}
%				\State $\mu\gets\max(\{j: cseq[j].status = F\})$ \label{line:reader:lastfin}
%				\State $\nu\gets |cseq|$ 
%				\For{$i=\mu:\nu$}
%					\State $\tup{\tg{},v} \gets \max(\text{\act{get-data}}(\config{cseq[i]}), \tup{\tg{},v})$ \label{line:reader:max}
%				\EndFor
%				\State $done\gets {\bf false}$
%				\While{{\bf not} $done$}
%					\State \act{put-data}$(cseq[\nu].cfg, \tup{\tg{},v})$ \label{line:reader:prop}
%					\State $cseq\gets$\act{read-config}($cseq$)
%					\If{$|cseq| = \nu$}
%						\State $done \gets  true$
%					\Else
%						\State $\nu\gets |cseq|$
%					\EndIf
%				\EndWhile
%				\EndOperation
%				
%				\Statex
%				\Statex
%
%				\Procedure{get-data}{$c$}
%			%	\State {\bf send} $(\text{{\sc query}},\rdr)$ to every server $s\in \bigcup_{cseq[i]}members(\qs_{cseq[i].conf})$
%				\State {\bf send} $(\text{{\sc query}})$ to each  $s\in \servers{c}$
%				\State {\bf until}    $\exists \quo{}, \quo{}\in\quorums{c}$ s.t. 
%				\State\TT $\rdr_i$ receives $\tup{t_s,v_s}$ from $\forall s\in\quo{}$ 
%				\State $t_{max} \gets \max(\{t_s : \rdr_i \text{ received } \tup{t_s,v_s} \text{ from } s \})$
%				\State {\bf return} $\{\tup{t_s,v_s}:t_s=t_{max} \wedge ~\rdr_i \text{ received } \tup{t_s,v_s} \text{ from } s\}$
%				\EndProcedure
%				
%				\Statex				
%			\Procedure{put-data}{$c, \tup{\tg{},v})$}
%				\State {\bf send} $(\text{{\sc write}}, \tup{\tg{},v})$ to each $s \in \servers{c}$
%				\State {\bf until} $\exists \quo,  \quo \in \quorums{c}$ s.t. $\rdr_i$ receives {\sc ack} from $\forall s\in\quo{}$
%			\EndProcedure
%
%
%			\Statex
%			
%			\Procedure{read-config}{$seq$}
%			\State $\mu = \max(\{j: seq[j].status = F\})$	\label{line:readconfig:final}
%			%\State $\nu = |cseq|$
%			\State $c \gets seq[\mu].cfg$
%			%\State {\bf send} $(\text{{\sc read-config}}, recon_i)$ to each   $s\in \bigcup_{\mu \leq i \leq \nu} \servers{currCfg}$
%			\While{$c \neq \bot$}
%			%\State {\bf send} $(\text{\act{read-config}}, recon_i)$ to each $s\in \servers{c}$
%			%\State {\bf until}  $\forall j,  \mu \leq j\leq \nu$  $\wedge$  
%			%$\exists\quo{},  \quo{} \in \quorums{cseq[j].cfg}$ s.t. $ \forall s\in\quo{},  recon_i$  receives $cseq_s$ from $s$ 
%			%\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\forall s\in\quo{}, recon_i$  receives $nextC_s$ from $s$
%			%\State $ell \gets \max_{cseq'\text{ received }}(|cseq'|)$
%			\State $nextC \gets$\act{get-next-config}$(c)$ 
%			\If{$nextC.cfg\neq\bot$} 
%			\State $\mu\gets \mu+1$				\label{line:readconfig:increment}
%			\State $seq[\mu] \gets nextC$	\label{line:readconfig:assign}
%			\State \act{put-config}$(seq[\mu-1].cfg, seq[\mu])$
%			\State $c \gets seq[\mu].cfg$
%			\Else
%			\State $c \gets \bot$
%			\EndIf
%			\EndWhile
%			\State {\bf return} $seq$
%			\EndProcedure
%			
%			\Statex		
%			
%			\Procedure{get-next-config}{$c$}
%			\State {\bf send} $(\text{{\sc read-config}})$ to each $s\in \servers{c}$
%			\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\rdr_i$ receives $nextC_s$, $\forall s\in\quo{}$
%			\If{$\exists s\in \quo{}\text{ s.t. } nextC_s.cfg\neq\bot$} 
%			\State {\bf return} $nextC_s$
%			\Else
%			\State {\bf return} $\bot$
%			\EndIf 
%			\EndProcedure
%			
%			\Statex
%			
%			\Procedure{put-config}{$c, cfgPtr)$}
%			\State {\bf send} $(\text{{\sc write-config}}, cfgPtr)$ to each $s\in \servers{c}$
%			\State {\bf until} $\exists\quo{},  \quo{}\in\quorums{c}$ s.t. $\rdr_i$ receives {\sc ack} from $\forall s\in\quo{}$
%			\EndProcedure
%		}\end{multicols}	
%	\end{algorithmic}
%	%\hrule \B
%	\caption{Reader protocol of algorithm \ares{}  at each reader $\rdr$ }
%	\label{algo:reader}
%\end{algorithm}


%When a {\sc query} message is received, the server replies with its local tag-value pair, and if a {\sc query-tag}
%message is received then it replies with its local tag alone. If a {\sc write} message is received then the server
%compares its local tag with the tag enclosed in the incoming message. If the received tag is larger, 
%then the server updates its local tag-value pair and replies with an acknowledgment. 
%			\State $vp\gets v; v \gets val;$ \label{line:write:storevalues}
%			\State $ts\gets ts+1$ 			\label{line:write:incrementts}
%			\State $wcounter \gets wcounter+1$
%			\State {\bf send}($\tup{ts,v,vp},w, wcounter$) to all servers 
%			\State {\bf wait until} $|\srvSet|-f$ servers reply						
%			\State return(OK) 
%			\EndFunction	
%			
%			\Statex
%			\State at each reader $r_i$
%			\State{\bf Components:}
%			%\State  $ts\in\N^+,~maxTS\in\N^+,~maxPS\in\N^+,~rCounter\in\N^+,~v\in U$
%			\State  $ts\in\N^+,~maxTS\in\N^+,~v,vp\in V, rcounter \in\N^+$
%			\State  $srvAck\subseteq \srvSet\times M, ~maxTSmsg\subseteq M$ 
%			\State{\bf Initialization:}
%			\State  $ts\gets 0, ~maxTS\gets 0,v \gets \bot,vp \gets \bot, rcounter \gets 0$
%			\State $srvAck\gets\emptyset, ~maxTSmsg\gets\emptyset$
%			%\Statex	
%			\Function{read}{}
%			\State  $rcounter\gets rcounter+1$
%			\State {\bf send}($\tup{ts,v,vp}, \rdr_i, rcounter$) to all servers 
%			\State {\bf wait until} $|srvAck|=|\srvSet|-f$ servers reply \Comment{Collect the $(serverid,\tup{\tup{ts',v',vp'},views})$ pairs in $srvAck$} %s.t. $Counter=rCounter$ 
%			%\State  $rcvMsg \gets \{m|r_i \text{ received }m=(,~*,~*)\}$
%			\State  $maxTS \gets \max(\{m.ts'|(s,m)\in srvAck\})$  \label{line:reader:maxts}
%			\State  $maxAck \gets \{(s,m)|(s,m)\in srvAck ~\wedge~ m.ts'=maxTS \}$ \label{line:reader:maxack}
%			\State $\tup{ts,v,vp}\gets m.\tup{ts',v',vp'}$ for $(*,m)\in maxAck$	\label{line:reader:update}	
%			\If{ $\exists \alpha\in[1,|\rdSet|+1]$ s.t. $MS=\{s: (s,m)\in maxAck ~\wedge~ m.views \geq \alpha\}$ and $|MS|\geq |\srvSet|-\alpha f$}   \label{line:reader:predicate}
%			\State  return($v$)
%			\Else
%			\State  retutn($vp$)
%			\EndIf
%			\EndFunction
%			\Statex
%			
%			\State at each server $s_i$ 
%			\State{\bf Components:}
%			\State  $ts\in\N^+, seen\subseteq\rdSet\cup\{w\}, ~v,vp\in V, Counter[1\ldots|\rdSet|+1]$
%			%\State  $msgType\in\{~seen\subseteq\mathcal{V}\cup\{w\}$	
%			\State{\bf Initialization:}
%			\State  $ts\gets 0,~seen\gets \emptyset, ~v,vp\in V, Counter[i]\gets 0$ for $i\in\rdSet\cup\{w\}$ 
%			%\Statex	
%			\Function{rcv}{$\tup{ts',v',vp'}, q, counter$}\Comment{Called upon reception of a message}
%			%\State {\bf upon} receive($msgType,~ts',~rCounter',~vid$) from $q\in \{w,r_1,\ldots,r_R\}$ {\bf and} $rCounter'\geq counter[pid(q)]$ {\bf do} 
%			%\IF
%			\If { $Counter[q] < counter$ } 
%			\If {$ts'> ts$} 	\label{line:server:ts-comparison}
%			\State  $\tup{ts,v,vp}\gets \tup{ts',v',vp'}$ \label{line:server:update}
%			\State $seen\gets \{q\}$ 					\label{line:server:reset}
%			\Else
%			\State  $seen\gets seen\cup \{q\}$ 			\label{line:server:append}
%			\EndIf
%			%\State  $counter[pid(q)]\gets rCounter'$ 	\hfill%\COMMENT {$pid(q)$ returns 0 if $q=w$ and $i$ if $q=r_i$}
%			\State  send($\tup{ts,v,vp},~|seen|$) to $q$ 	\label{line:server:reply}
%			%\State {\bf{end if}}
%			\EndIf 
%			\EndFunction


%\input{ioa/recas-reader_ioa.tex}
%\input{ioa/recas-writer_ioa.tex}
%\input{ioa/recas-server_ioa.tex}


==> correctenss_v3.tex <==
\remove{We proceed by first introducing some definitions and notation, then by presenting some properties that are satisfied 
by the reconfiguration service in any execution, and then we show that given these properties our algorithm satisfies 
the safety (atomicity) conditions. 
%Due to space limitations the proofs of the main statements are omitted and can be found in \cite{ARES:Arxiv:2018}.
}

\remove{
\myparagraph{Notations and definitions.}
For a server $s$, we use the notation $\atT{s.var}{\state}$ to refer to the value of the state variable $var$, in $s$, at a state $\state$ of an  execution $\EX$. 
If server  $s$ crashes at a state $\state_f$ in an execution $\EX$ then $\atT{s.var}{\state}\triangleq\atT{s.var}{\state_f}$ for any state variable $var$ and for 
any state $\state$ that appears after $\state_f$ in $\EX$. 
%refers to the value of $v$ at $s$ at the state just before crashes. In other words, $\atT{s.v}{T}  \triangleq \atT{s.v}{\hat{T}}$, where $\hat{T}$ is the latest point in the execution, such that, $(a)$ $\hat{T} \leq T$ and $(b)$ $s$ is non-faulty.
 }
 
 \remove{
\begin{definition}[Tag of a configuration]  Let  $c \in \mathcal{C}$ be a configuration, $\state$ be a state in some execution $\EX$ then 
we define the tag of $c$ at state $\state$ as  
$ \atT{tag(c)}{\state} \triangleq \min_{Q \in \quorums{c}} \max_{s \in Q}~\atT{(s.tag}{\state}).$
We  drop the suffix $|_\state$, and simply denote as $tag(c)$,  when the state  is clear from the context.
\end{definition}

\begin{definition}
Let $\sigma$ be any point in an execution of \ares{} and suppose we use the notation $\cvec{\pr}{\state}$ for $ \atT{\pr.cseq}{\state}$,  i.e., the $cseq$ variable at process $p$ at the state $\state$. %be the value of a configuration sequence vector at a process $\pr$ at some state  $\st$ in an execution $\EX$. 
Then we define as $ \mu(\cvec{\pr}{\state})  \triangleq  \max\{ i : \cvec{\pr}{\state}[i].status = F\}$ 
and $ \nu(\cvec{\pr}{\state}) \triangleq |\cvec{\pr}{\state}|$, where $|\cvec{\pr}{\state}|$ is the length of the  configuration vector 
$\cvec{\pr}{\state}$. % that are not equal to $\bot$.  
\end{definition}

\begin{definition} [Prefix order]
Let $\mathbf{x}$ and $\mathbf{y}$ be any two configuration sequences. We say that $\mathbf{x}$ is a prefix of $\mathbf{y}$, denoted by 
$\mathbf{x} \preceq_p  \mathbf{y}$, if $\config{\mathbf{x}[j]}=\config{\mathbf{y}[j]}$, for all $j$ such that $\mathbf{x}[j]\neq\bot$.
\end{definition}

%\input{ssec-correct-recon.tex}
\nn{Next we analyze the properties  satisfied by  ~\ares{}. In brief, the reconfiguration algorithm
preserves three properties in any execution: 
$(i)$ \myemph{Configuration Uniqueness}, 
$(ii)$ \myemph{Configuration 
Prefix}, and 
$(iii)$ \myemph{Configuration Progress}. Configuration Uniqueness ensures that no two different 
configurations are assigned to the same index in a configuration sequence. Configuration
prefix ensures that any \act{read-config} action 
returns an extension of the configuration sequence returned by any previous \act{read-config} action. 
Finally, the configuration progress focuses on the status of the configurations in a sequence, 
and ensures that a \act{read-config} action observes at least as recent
\myemph{finalized} configuration as any preceding \act{read-config} action. The following theorem presents formally those 
properties.}

%The first lemma shows that any two configuration sequences have the same configuration identifiers
%in the same indexes. 
%
%\begin{lemma}[Configuration Uniqueness]
%	\label{lem:unique}
%	
%	%Let $\state_1$ and $\state_2$ be any two states of an execution $\EX$ of the algorithm,
%	%and $\pr, q$ two participating processes. 
%	%be the state after the response action of an operation $\op_1$ from process $p$,
%	%and $\state_2$ be the state after the first $\act{read-config}$ call of an operation $\op_2$ from $q$.
%	For any processes $\pr, q\in \idSet$ and any states $\state_1, \state_2$ in an execution $\EX$, it must hold that 
%	$\config{\cvec{\pr}{\state_1}[i]}=\config{\cvec{q}{\state_2}[i]}$,  $\forall i$ s.t. 
%	$\config{\cvec{\pr}{\state_1}[i]},\config{\cvec{q}{\state_2}[i]}\neq \bot$.
%\end{lemma}
%
%We can now move to an important lemma that shows that any \act{read-config} action 
%returns an extension of the configuration sequence returned by any previous \act{read-config} action. 
%First, we show that the last finalized configuration observed by any \act{read-config} action is at least as 
%recent as the finalized configuration observed by any subsequent \act{read-config} action. 
%%Using this lemma we will then show that when 
%
%\begin{lemma}[Configuration Prefix]
%	\label{lem:prefix}
%	Let $\op_1$ and $\op_2$ two 
%	%read/write/install operations 
%	completed \act{read-config} actions invoked by processes $\pr_1, \pr_2\in\idSet$ 
%	respectively, such that $\op_1\bef\op_2$ in an execution $\EX$. Let $\state_1$ be the state after the response 
%	step of $\op_1$ and $\state_2$ the state after the response step 
%	%termination of the first $\act{read-config}$ 
%	of $\op_2$. Then 
%	$\cvec{\pr_1}{\state_1}\preceq_p\cvec{\pr_2}{\state_2}$.
%\end{lemma}
%
%Thus far we focused on the configuration member of each element in $cseq$. As operations do get in account
%the \myemph{status} of a configuration, i.e. $P$ or $F$, in the next lemma we will examine the relationship of 
%the last finalized configuration as detected by two operations. First we present a lemma that shows the 
%monotonicity of the finalized configurations.
%
%
%\begin{lemma}  [Configuration Progress]
%	\label{lem:finalconf}
%	Let $\op_1$ and $\op_2$ two 
%	%read/write/install operations 
%	completed \act{read-config} actions invoked by processes $\pr_1, \pr_2\in\idSet$ 
%	respectively, such that $\op_1\bef\op_2$ in an execution $\EX$. 
%	Let $\state_1$ be the state after the response 
%	step of $\op_1$ and $\state_2$ the state after the response step 
%	%after the completion of $\op_1$ and $\state_2$ the state after the termination of the first $\act{read-config}$ 
%	of $\op_2$. Then 
%	$\mu(\cvec{\pr_1}{\state_1})\leq\mu(\cvec{\pr_2}{\state_2})$.
%\end{lemma}


\begin{theorem}[Reconfiguration Properties]
	Let $\op_1$ and $\op_2$ be two 
	%read/write/install operations 
	completed \act{read-config} actions invoked by processes $\pr_1, \pr_2\in\idSet$ 
	respectively, such that $\op_1\bef\op_2$ in an execution $\EX$ of ~\ares. 
	Let $\state_1$ be the state after the response 
	step of $\op_1$ and $\state_2$ the state after the response step 
	%after the completion of $\op_1$ and $\state_2$ the state after the termination of the first $\act{read-config}$ 
	of $\op_2$.
	%$\cvec{\pr_1}{\state_1}$ and $\cvec{\pr_2}{\state_2}$ at two states $\state_1$ and $\state_2$ 
	%in an execution $\EX$ of the algorithm  such that $\state_1$ appears before $\state_2$ in $\EX$. 
	Then the following holds: 
%	\begin{enumerate}
	%	\item [$(a)$] 
	$(a)$	$\cvec{\pr_2}{\state_2}[i].cfg = \cvec{\pr_1}{\state_1}[i].cfg$,  for $ 1 \leq i \leq \nu(\cvec{\pr_1}{\state_1})$,
	%	\item [$(b)$]
		%$(b)$  
	$(b)$	$\cvec{\pr_1}{\state_1}  \preceq_p \cvec{\pr_2}{\state_2}$, and
	%	\item [$(c)$] 
		%$(c)$  
	$(c)$	$\mu(\cvec{\pr_1}{\state_1}) \leq \mu(\cvec{\pr_2}{\state_2})$
		%; and 
		%\item [$(d)$]  
		%\nn{????$(d)$  $\cvec{\pr_2}{\state_2}[i]   = \cvec{\pr_1}{\state_1}[i]$,  for  $ 1 \leq i \leq \mu(\cvec{\pr_1}{\state_1})$????} 
%	\end{enumerate}
\end{theorem}
}

%\input{ssec-correct-safety_v2.tex}

%\subsection{\ares{} Liveness}
%\label{ssec:liveness}
%\input{ssec-correct-liveness.tex}

%The propagation of the information of the distributed object in \ares{} is achieved using the $\act{get-tag}$, $\act{get-data}$, 
%and $\act{put-data}$ actions.  
Given the properties satisfied by the reconfiguration algorithm of \ares{} 
and assuming that the DAP used satisfy properties $C1$ and $C2$, as presented
in Section \ref{ssec:dap}, then  we have the following result. 

\begin{theorem}[Atomicity]
    Consider  any execution of \ares{} such that in every configuration used   the DAP primitives  satisfy  the DAP consistency properties then ~\ares{} satisfy atomicity property.
	%, given that the 
	%$\act{get-data}$, $\act{get-tag}$, and $\act{put-data}$ primitives used satisfy properties
	%\textbf{C1} and \textbf{C2} of Definition \ref{def:consistency}.
\end{theorem}

%In  \ares{},  each configuration 
%may implement the DAPs in a different way as stated below:

\begin{remark}
	Algorithm \ares{} satisfies atomicity even when the DAP primitives used in two 
	different configurations $c_1$ and $c_2$ are not the same, given that the $c_i.\act{get-tag}$,
	$c_i.\act{get-data}$, and the $c_i.\act{put-data}$ primitives 
	used in each $c_i$ satisfy properties \textbf{C1} and \textbf{C2} of Definition \ref{def:consistency}.  
\end{remark}





































==> dap_v1.tex <==

\nn{In this section we introduce a set of  primitives, 	we refer to as  \textit{data access primitives (DAP)},
	which are invoked by the clients during \act{read/write/reconfig} operations and are defined 
 %implemented by the  set of servers  of 
 for any configuration $c$ in \ares{}. 
% We refer to such 
% primitives as the  \textit{data access primitives (DAP)} of the  configuration.
%
%describe an algorithm for implememting  atomic memory, say  	$A$, in a modular way, given  
%which can be associated with a configuration $c$.
 %To allow \ares{} to be modular we  introduce a set of  primitives, implemented on a set of servers 
%(configuration),  which we refer to as  \textit{data access
%primitives} (
The DAPs allow us:  $(i)$ to describe 
%an atomic memory algorithm, specifically~
\ares{} in  a \myemph{modular} manner, 
%$(ii)$ to adaptively change DAP implementation per configuration (thus changing the operation protocol), 
and $(ii)$ a cleaner reasoning about the correctness of \ares{}.
%implementation of an atomic memory service, specifically~\ares{}.
%Additionally, we also require some properties  for the  DAPs to prove the atomicity property of ~\ares{}.
}

%\nn{In this section we present simple abstractions, we call 
	%the next section, we present the \treas{} algorithm  \nnrev{based on  of}{using} three 
%	\textit{data access primitives} (DAP), which can be used to describe an algorithm for implememting  atomic memory, say  
%	$A$, in a modular way, given  
%which can be associated with 
%a configuration $c$.} 


\nn{We define three data access primitives for each $c\in\confSet$:}
%in the context of $c$ are: $(i)$ 
$\daputdata{c}{\tup{\tg{},v}}$, via which 
a client can ingest the tag value pair $\tup{\tg{},v}$ in to the configuration $c$;
 $(ii)$ $\dagetdata{c}$, used to retrieve the most up to date 
 tag and vlaue pair stored in the configuration $c$; 
 and $(iii)$ $\dagettag{c}$, used to retrieve the most up to date tag for an object stored in a configuration $c$.
  \nn{More formally,} assuming  a tag $\tg{}$ from 
  %$\tg{}$ be a logical timestamp from 
  a set of totally ordered tags $\tsSet$, 
  %over a comparison function $<_{\tg{}}$, $v$ be a value within the 
   a value $v$ from a domain 
   %of the distributed atomic object 
   $\valSet$, and a configuration $c$ from 
  %$c$ be the identifier of 
  a set of identifiers $\confSet$, the  
  %We define below the 
  three primitives are defined 
  %over a configuration $c\in\confSet$, tag $\tg{}\in\tsSet$, and a value $v\in\valSet$ 
  as follows:
  %which we collectively refer to as the \myemph{data-primitives}:
  %	\kmkrev{\nn{The following theorem captures the main result of this subsection.}} {Below we provide the specification and properties  of the DAPs.}
  
    \begin{definition}[Data Access Primitives] %Let $c$, $c \in C$,  be any configuration identifier  and  any read, write or client that invokes any of the following interfaces:
  	Given a configuration identifier $c\in\confSet$, any non-faulty client process $\pr$ may invoke the following data access primitives during an execution $\EX$, where $c$ 
  	is added to specify the configuration specific implementation of the primitives:
  	\begin{enumerate}
  		\item [$D1$:]  $\dagettag{c}$ that returns  a tag $\tg{}\in\tsSet$;  
  		%completes by responding with some tag $t \in \mathcal{T}$
  		\item[$D2$:] $\dagetdata{c}$ that  
  		%the response is though returning 
  		returns a tag-value pair $(\tg{}, v) \in \tsSet \times \valSet$, 
  		\item[$D3$:] $\daputdata{c}{\tup{\tg{}, v}}$ which accepts the tag-value pair $(\tg{}, v) \in \tsSet \times \valSet$ as argument. 
  	\end{enumerate} 
  		%returns a tag-value pair $(t, v) \in \mathcal{T} \times \mathcal{V}$
  \end{definition}
%
%
% in which a large family of tag-based atomic read/write object implementations can be transformed to. 
% Such conversion
% 
% For a read/write algorithm
% that uses the presented data-primitives, it can provide atomic guarantees if the data primitives 
% satisfy the following consistency properties: 
% 
%  To implement the \treas{} algorithm, which is based on the DAP primitives, the DAP primitives must satisfy the following
%  consistency properties.

\remove{
\begin{algorithm}[!ht]
	\begin{algorithmic}[2]
		\begin{multicols}{2}
			{\scriptsize
				%\Part{Generic Algorithm $A_1$}
				\Operation{read}{} 
				%\State $wCounter\gets wCounter+1$
				\State $\tup{t, v} \gets \dagetdata{c}$
				\State $\daputdata{c}{ \tup{t,v}}$
				\State return $ \tup{t,v}$
				\EndOperation
				\Statex
				\Operation{write}{$v$} 
				%\State $wCounter\gets wCounter+1$
				\State $t \gets \dagettag{c}$
				\State $t_w \gets inc(t)$
				\State $\daputdata{c}{\tup{t_w,v}}$
				\EndOperation
				%\EndPart
			}
		\end{multicols}
	\end{algorithmic}
	\caption{Read and write operations of generic algorithm $A_1$}
	\label{algo:atomicity:generic1}
	\vspace{-1em}
\end{algorithm}

A number of known tag-based algorithms that implement atomic read/write objects 
	(e.g., ABD \cite{ABD96}, \fast \cite{CDGL04} -- see \cite{ARES:Arxiv:2018}), can be expressed 
	in terms of DAP. In particular, many algorithms can be transformed in an algorithmic template, say $A_1$, 
	presented in Alg. \ref{algo:atomicity:generic1}. 
	In brief, a read operation in $A_1$ performs $\dagetdata{c}$ to retrieve a tag-value pair, $\tup{\tg{},v}$ from a configuration $c$, and then 
	it performs a $c.\act{put-data}(\tup{\tg{},v})$ to propagate that pair to the configuration $c$. A write operation is similar to the read but before 
	performing the $\act{put-data}$ action it generates a new tag which associates with the value to be written.
	%
	It can be shown 
	%\cite{ARES:Arxiv:2018} 
	that an algorithm described in the form $A_1$ satisfies atomic guarantees and liveness,
	if the DAP satisfy the following consistency properties:
}
  
  \kmk{In order for the DAPs to be useful in designing the \ares{} algorithm we further require the following consistency
   properties. As we see later in Section \ref{sec:safety:b}, the safety property of \ares{} 
   %hinges 
   holds, given that these properties hold for the DAPs in each configuration.} %as we see later in Section \ref{sec:safety:b}.}
 
 \begin{property}[DAP Consistency Properties]\label{property:dap}  In an execution $\EX$ 
 	we say that a DAP operation in an execution $\EX$ is complete if both the invocation and the 
 	matching response step  appear in $\EX$. 
 	If $\Pi$ is the set of complete DAP operations in execution $\EX$ then for any $\phi,\pi\in\Pi$: 
 	%be an execution of some algorithm that executes the data-primitives 
 \begin{enumerate}
 \item[ C1 ]  If $\phi$ is  $\daputdata{c}{\tup{\tg{\phi}, v_\phi}}$, for $c \in \confSet$, $\tup{\tg{\phi}, v_\phi} \in\tsSet\times\valSet$, % and $v_1 \in \valSet$,
 and $\pi$ is $\dagettag{c}$ (or  $\dagetdata{c}$) 
 %in $\EX$ such that 
 that returns $\tg{\pi} \in \tsSet$ (or $\tup{\tg{\pi}, v_{\pi}} \in \tsSet \times \valSet$) and $\phi$ completes \nn{before $\pi$ is invoked} in $\EX$, then $\tg{\pi} \geq \tg{\phi}$.
 \item[ C2 ] \sloppy If $\phi$ is a $\dagetdata{c}$ that returns $\tup{\tg{\pi}, v_\pi } \in \tsSet \times \valSet$, 
 then there exists $\pi$ such that $\pi$ is $\daputdata{c}{\tup{\tg{\pi}, v_{\pi}}}$ and $\phi$ did not complete before the invocation of $\pi$. 
 If no such $\pi$ exists in $\EX$, then $(\tg{\pi}, v_{\pi})$ is equal to $(t_0, v_0)$.
 \end{enumerate} \label{def:consistency}
 \end{property}\vspace{-0.5em}

\nn{In Section \ref{ssec:dap:impl} we show how to implement a set of DAPs, where erasure-codes are used to reduce storage and communication costs. 
	%We show that 
	Our DAP implementation satisfies Property \ref{property:dap}.}

   \nn{
 	As noted earlier, expressing \ares{}
 	%an atomic memory implementation  algorithm 
 	in terms of the DAPs 
 	%primitives 
 	allows one to achieve a modular 
	design. Modularity enables the usage of different DAP
	implementation per configuration, during any execution of \ares{},
	as long as the DAPs implemented in each configuration satisfy Property \ref{property:dap}.
	For example, the DAPs in a configuration $c$ may be implemented using replication,
	while the DAPs in the next configuration say $c'$, may be implemented using erasure-codes.}	
\nnfix{
%	This enables the use of different coding algorithms based on the application 
% 		or even per configuration in the same system
%		without affecting the correctness of \ares{}.
		Thus, a system may use a scheme that offers higher fault tolerance (e.g. replication)
	when storage is not an issue, while switching to a more storage efficient (less fault-tolerant)
scheme when storage gets limited. }

%	This in turn, allows the usage of different coding algorithms and 
%	code parameters in each individual configuration without affecting 
%	the correctness of \ares{}.

	
	\nn{
		In Section \ref{sec:dap:flexible}, we show that the presented DAPs are not only suitable
	for algorithm \ares{}, but can also be used to implement a large family of atomic read/write
	storage implementations. By describing an algorithm $A$ according to a simple algorithmic 
	template (see Alg.~\ref{algo:atomicity:generic1}), we show that $A$ preserves safety (atomicity) if 
	the used DAPs satisfy Property \ref{property:dap}, and $A$ preserves liveness (termination),
	if every invocation of the used DAPs terminate,  under the failure model assumed.
}
%		
%	%for such algorithm. First and foremost, every configuration introduced during any execution of ~\ares{} may have varying number of servers or values of code parameters. 
%	The modular framework allows use to implement atomic memory using ~\ares{}
%with a wide range of configuration parameters.	
%	Moreover, describing an algorithm according to the algorithmic  template $A_1$ (Alg.~\ref{algo:atomicity:generic1} in Section ~\ref{sec:dap:flexible}) allows  to prove the algorithm preservers \textit{safety property} (atomicity) 
%	% it enables ease of reasoning about the safety of the algorithm  
%	% given that atomicity holds if 
%	by simply showing that the  DAP consistency properties hold, and the algorithm is \textit{live} \nn{if each
%	invocation of a DAP terminates, under the failure model assumed.} 
%	Second, the safety and liveness proofs for complex algorithms, such as  \ares{},  % algorithm  
%	become easier as one may reason about the  atomictiy property of ~\ares{} based on the consistency propertyies of the underlying  DAP primitives 	without involving the underlying implementation of those primitives.. Next the consistency properties of these DAPs can be argued  based on the configuration specific
%	implementation of them.
%%	 that are satisfied by the primitives used,
%%	without involving the underlying implementation of those primitives. 
%	Also, describing a reconfigurable algorithm using DAPs, provides the flexibility 
%	to use different implementation mechanics for the DAPs in each reconfiguration, as long as the DAPs satisfy the necessary properties.} %Hence, makes our algorithm \myemph{adaptive}.}
%Now we show that if DAP properties are satisfied from the DAP, then algorithmic template $A_1$ (Alg.~\ref{algo:atomicity:generic1})  implements an atomic read/write algorithm. 
 %We can show that $A_1$ satisfy atomic guarantees and liveness if the DAP in the above algorithms satisfy the DAP consistency properties. Our liveness guarantees are applicable only when we consider one instance of {\treas}, but livess cannot be
 %guaranteed for {\ares}.
 
 \remove{
 {\bf we should move it to a later section}
 \begin{theorem}[\nn{Correctness} of $A_1$]\label{atomicity:A1}
 Suppose the DAP implementation satisfies the consistency properties $C1$ and $C2$ of  Definition \ref{def:consistency}
 for a configuration $c\in\confSet$. 
 Then any execution $\EX$  of \nn{algorithm $c.A_1$}
 %the  atomicity protocols $A_1$  on a 
 %fixed set of servers $S$, of some 
 %configuration $c\in\confSet$,  
 %as in Fig. ~\ref{algo:atomicity:generic1} satisfies atomic read and write and is live if the  primitive functions are live in $\xi$.
 is atomic and live if each DAP \nn{invocation terminates} in $\EX$ \nn{under the failure model $c.\mathcal{F}$}.
 \end{theorem}
%\nn{[NN: How can those primitives be used to show correctness of an algorithm? I think this is important to discuss. Also we should mention that these primitives are universal and can be used to implement other tag-based algorithms.]}
}

==> plots/EC_ABD_separated/sec_discussions_v1.tex <==
 %For a read/write algorithm
%that uses the presented data-primitives, it can provide atomic guarantees if the data primitives 
%satisfy the following consistency properties: 
%To implement an algorithm, which is based on the DAP primitives, the DAP primitives must satisfy the following
%consistency properties.


In this section, we argue that  various implementations of DAPs  can be used in \ares{}. In fact, via \act{reconfig} 
operations, one can implement a highly adaptive 
%strongly consistent 
atomic DSS: 
replication-based can be transformed into erasure-code based DSS; increase or decrease the number of storage servers; 
 study 
the performance of the DSS under various code parameters, etc. 
The insight to implementing various DAPs comes from the observation that the  simple  algorithmic 
	template $A$ (see Alg.~\ref{algo:atomicity:generic1}) for reads and writes protocol combined with 
	any implementation of DAPs, satisfying Property~\ref{property:dap} gives rise to a MWMR atomic memory service.
	Moreover, the read and writes operations terminate as long as the implemented DAPs complete. 
%	implements an atomic  storage if the implementation of the  DAPs satisfy Property \ref{property:dap}, and $A$ preserves liveness (termination),
%	if every invocation of the used DAPs terminate.
\begin{algorithm}[!ht]
	\begin{algorithmic}[2]
		\begin{multicols}{2}
			{\scriptsize
				%\Part{Generic Algorithm $A_1$}
				\Operation{read}{} 
				%\State $wCounter\gets wCounter+1$
				\State $\tup{t, v} \gets \dagetdata{c}$
				\State $\daputdata{c}{ \tup{t,v}}$
				\State return $ \tup{t,v}$
				\EndOperation
				%\Statex
				\Operation{write}{$v$} 
				%\State $wCounter\gets wCounter+1$
				\State $t \gets \dagettag{c}$
				\State $t_w \gets inc(t)$
				\State $\daputdata{c}{\tup{t_w,v}}$
				\EndOperation
				%\EndPart
			}
		\end{multicols}
	\end{algorithmic}
	\caption{Template $A$ for the client-side read/write steps.}
	\label{algo:atomicity:generic1}
	\vspace{-1em}
\end{algorithm}	
	

	A read operation in $A$ performs $\dagetdata{c}$ to retrieve a tag-value pair, $\tup{\tg{},v}$ from a configuration $c$, and then 
	it performs a $c.\act{put-data}(\tup{\tg{},v})$ to propagate that pair to the configuration $c$. A write operation is similar to the read but before 
	performing the $\act{put-data}$ action it generates a new tag which associates with the value to be written.
	%
The following result shows 
	%\cite{ARES:Arxiv:2018} 
	that $A$ is atomic and live,
	if the DAPs satisfy Property~\ref{property:dap} and live.
	 
 \begin{theorem}[\nn{Atomicity} of template $A$]\label{atomicity:A1}
 Suppose the DAP implementation satisfies the consistency properties $C1$ and $C2$ of  Property \ref{def:consistency}
 for a configuration $c\in\confSet$. 
 Then any execution $\EX$  of \nn{algorithm $A$ in configuration $c$}
 %the  atomicity protocols $A_1$  on a 
 %fixed set of servers $S$, of some 
 %configuration $c\in\confSet$,  
 %as in Fig. ~\ref{algo:atomicity:generic1} satisfies atomic read and write and is live if the  primitive functions are live in $\xi$.
 is atomic and live if each DAP \nn{invocation terminates} in $\EX$ \nn{under the failure model $c.\mathcal{F}$}.
 \end{theorem}
 \begin{proof}
 We  prove the atomicity by proving properties $A1$, $A2$ and $A3$ presented in Section \ref{model} for any execution of the algorithm.
					
	\emph{Property $A1$}: Consider two operations $\phi$ and $\pi$ such that $\phi$ completes before $\pi$ is invoked. 
	We need to show that it cannot be  the case that $\pi \prec \phi$. We break our analysis into the following four cases:

	Case $(a)$: {\em Both $\phi$ and $\pi$ are writes}. The $\daputdata{c}{*}$ of $\phi$ completes before 
	$\pi$ is invoked. 
	%which implies that by well-formedness 
	By property {\bf C1} the tag $\tg{\pi}$ returned by the $\dagetdata{c}$ at $\pi$ is 
	at least as large as $\tg{\phi}$. Now, 
	%since $\tg{\pi}$ is larger than $t_{\phi}$, by the steps of 
	since $\tg{\pi}$ is incremented by the write operation then $\pi$ puts a tag $\tg{\pi}'$ such that
	$\tg{\phi} < \tg{\pi}'$ and hence we cannot have $\pi \prec \phi$.
	
	Case $(b)$: {\em $\phi$ is a write and  $\pi$ is a read}. In execution $\EX$ since 
$\daputdata{c} {\tup{t_{\phi}, *}}$ of $\phi$ completes 
	before the $\dagetdata{c}$ of $\pi$ is invoked, by 
	%the well-formedness 
	property {\bf C1} the tag $\tg{\pi}$ obtained from the above
	$\dagetdata{c}$ is at least as large as $\tg{\phi}$. Now $\tg{\phi} \leq \tg{\pi}$ implies that we cannot have $\pi \prec \phi$.
	
	Case $(c)$: {\em $\phi$ is a read and  $\pi$ is a write}.  Let the id of the writer that invokes $\pi$ we $w_{\pi}$.  
	The 
$\daputdata{c}{\tup{\tg{\phi}, *}}$  call of $\phi$ completes
	before  $\dagettag{c}$ of $\pi$ is initiated. Therefore, by 
	%the well-formedness 
	property {\bf C1} %of data-primitives the above 
	$\act{get-tag}(c)$ returns $\tg{}$ such that, $\tg{\phi} \leq \tg{}$. Since $\tg{\pi}$ is equal to $inc(\tg{})$ 
	by design of the algorithm, hence $\tg{\pi} > \tg{\phi}$ and we cannot have $\pi \prec \phi$.
	
	Case $(d)$: {\em Both $\phi$ and $\pi$ are reads}. In execution $\EX$  
the $\daputdata{c}{\tup{t_{\phi}, *}}$ is executed as a part of $\phi$ and 
	completes before $\dagetdata{c}$ is called in $\pi$. By 
	%the well-formedness
	 property {\bf C1} of the data-primitives, 
	we have $\tg{\phi} \leq \tg{\pi}$ and hence we cannot have $\pi \prec \phi$.
	
	\emph{Property $A2$}: Note that because the tag set $\tsSet$ is well-ordered we can show that A2 holds by first showing that
	every write has a unique tag. This means that any two pair of writes can be ordered. 
	Note that 
	a read can be ordered w.r.t. any write operation trivially if the respective tags are different, and by definition, if the 
	tags are equal the write is ordered before the read.
	
	Observe that two tags generated from different writers are necessarily distinct because of the 
	id component of the tag. Now if the operations, say $\phi$ and $\pi$ are writes  from the same writer then, by 
	well-formedness property, the second operation will witness a higher integer part in the tag 
	%is invoked after the first completes, say without loss of generality $\phi$ completes before 
	%$\pi$ is invoked.   In that case the integer part of the tag of $\pi$ is higher 
	%because the well-formedness 
	by property  {\bf C1}, and since the $\dagettag{c}$  is followed by $\daputdata{c}{*}$. Hence $\pi$ is ordered after $\phi$. 
	
	\emph{Property $A3$}:  By {\bf C2} the $\dagetdata{c}$ may return a tag $\tg{}$, only 
	when there exists an operation $\op$ that invoked a $\daputdata{c}{\tup{\tg{},*}}$. Otherwise it returns the initial value. Since a write is the only operation to put a new tag $\tg{}$ in the system then Property $A3$ follows from {\bf C2}.
 \end{proof}
	
	\subsection{Representing  Known Algorithms in terms of data-access primitives}
\label{ssec:generic}

A number of known tag-based algorithms that implement atomic read/write objects 
	(e.g., ABD \cite{ABD96}, \fast \cite{CDGL04} ), can be expressed 
	in terms of DAP. In this subsection we demonstrate how we can transform the very celebrated ABD algorithm \cite{ABD96}.

\paragraph{\mwABD{} Algorithm.}
The multi-writer version of the ABD can be transformed to the generic algorithm Template $A$. Algorithm \ref{algo:dap:abd}
illustrates the three DAP for the ABD algorithm. The $\act{get-data}$ primitive encapsulates the query phase 
of \mwABD{}, while the $\act{put-data}$ primitive encapsulates the propagation phase of the algorithm. 
%Thus, given a configuration $c\in\confSet$ the DAPs in the transformation of ABD are implemented as follows:

\begin{algorithm}[!h]
	%\hrule \F
	\begin{algorithmic}[2]
		\begin{multicols}{2}{\scriptsize
				\Part{Data-Access Primitives at process $\pr$}
				\Procedure{c.put-data}{$\tup{\tg{},v})$}
				\State {\bf send} $(\text{{\sc write}}, \tup{\tg{},v})$ to each $s \in \servers{c}$
				\State {\bf until} $\exists \quo,  \quo \in \quorums{c}$ s.t. $\pr$ receives {\sc ack} from $\forall s\in\quo{}$
				\EndProcedure
				
				\Statex				
				
				\Procedure{c.get-tag}{}
				%	\State {\bf send} $(\text{\act{query}},\rdr)$ to every server $s\in \bigcup_{cseq[i]}members(\qs_{cseq[i].conf})$
				\State {\bf send} $(\text{{\sc query-tag}})$ to each  $s\in \servers{c}$
				\State {\bf until}    $\exists \quo{}, \quo{}\in\quorums{c}$ s.t. 
				\State\TT$\pr$ receives $\tup{\tg{s},v_s}$ from $\forall s\in\quo{}$ 
				\State $\tg{max} \gets \max(\{\tg{s} : \pr \text{ received } \tup{\tg{s},v_s} \text{ from } s \})$
				\State {\bf return} $\tg{max}$
				\EndProcedure
				
				\Statex
				
				\Procedure{c.get-data}{}
				%	\State {\bf send} $(\text{{\sc query}},\rdr)$ to every server $s\in \bigcup_{cseq[i]}members(\qs_{cseq[i].conf})$
				\State {\bf send} $(\text{{\sc query}})$ to each  $s\in \servers{c}$
				\State {\bf until}    $\exists \quo{}, \quo{}\in\quorums{c}$ s.t. 
				\State\TT $\pr$ receives $\tup{\tg{s},v_s}$ from $\forall s\in\quo{}$ 
				\State $\tg{max} \gets \max(\{\tg{s} : \rdr_i \text{ received } \tup{\tg{s},v_s} \text{ from } s \})$
				\State {\bf return} $\{\tup{\tg{s},v_s}:\tg{s}=\tg{max} \wedge ~\pr \text{ received } \tup{\tg{s},v_s} \text{ from } s\}$
				\EndProcedure
				\EndPart
			}\end{multicols}
				
			\\\hrulefill 
			
			\begin{multicols}{2}{\scriptsize
				\Part{Primitive Handlers at server $s_i$ in configuration $c$}
				\Receive{{\sc query-tag}}{} %\Comment{Called upon reception of a message}
				%\State $\act{handle-get-tag(c_k)}$
				\State send $\tg{}$ to $q$
				\EndReceive
				
				\Statex
				
				\Receive{{\sc query}}{}
				%\State $\act{handle-get-data(c_k)}$
					\State send $\tup{\tg{}, v}$ to $q$
				\EndReceive
				
				\Statex
				\Statex
				
				\Receive{{\sc write}, $\tup{\tg{in}, v_{in}}$}{}
				%\State $\act{handle-put-data(c_k)}$
					\If {$\tg{in}> \tg{}$} 	\label{line:server:tg-comparison}
						\State  $\tup{\tg{},v}\gets \tup{\tg{in},v_{in}}$ \label{line:server:update}
					\EndIf
					\State  send  {\sc ack} to $q$ 	\label{line:server:reply}
				\EndReceive
				\EndPart
				
		}\end{multicols}	
	\end{algorithmic}
	%\hrule \B
	\caption{Implementation of DAP for ABD at each process $\pr$ using configuration $c$}
	\label{algo:dap:abd}
\end{algorithm} 

Let us now examine if the primitives satisfy properties \textbf{C1} and \textbf{C2} of Property \ref{property:dap}.
We begin with a lemma that shows the monotonicity of the tags at each server.

\begin{lemma} 
	\label{lem:server:tag:monotonic}
	Let $\st$ and $\st'$ two states in an execution $\EX$ such that $\st$ appears before $\st'$ in $\EX$.
	Then for any server $s\in\srvSet$ it must hold that $\atT{s.tag}{\st}\leq\atT{s.tag}{\st'}$.
\end{lemma}

\begin{proof}
	According to the algorithm, a server $s$ updates its local tag-value pairs when it receives a message
	with a higher tag. So if $\atT{s.tag}{\st}=\tau$ then in a state $\st'$ that appears after $\st$ in $\EX$,
	$\atT{s.tag}{\st'}\geq \tau$.
\end{proof}

In the following two lemmas we show that property \textbf{C1} is satisfied, that is if a $\act{put-data}$ action completes,
then any subsequent $\act{get-data}$ and $\act{get-tag}$ actions will discover a higher tag than the one propagated 
by that $\act{put-data}$ action.

\begin{lemma}
	\label{lem:putdata:gettag}
	Let $\phi$ be a $\daputdata{c}{\tup{\tau,v}}$ action invoked by $\pr_1$ and $\gamma$ be a $\dagettag{c}$ action
	invoked by $\pr_2$ in a configuration $c$, such that 
	$\phi\bef\gamma$ in an execution $\EX$ of the algorithm. Then $\gamma$ returns a tag $\tau_\gamma \geq \tau$. 
\end{lemma}

\begin{proof}
	The lemma follows from the intersection property of quorums. In particular, during the $\daputdata{c}{\tup{\tau,v}}$ 
	action, $\pr_1$ sends the pair $\tup{\tau,v}$ to all the servers in $\servers{c}$ and waits until all the servers in 
	a quorum $Q_i\in\quorums{c}$ reply. When those replies are received then the action completes. 
	
	During a $\dagetdata{c}$ action on the other hand, $\pr_2$ sends query messages to all the servers in $\servers{c}$ 
	and waits until all servers in a quorum $Q_j\in\quorums{c}$ (not necessarily different than $Q_i$) reply. By definition 
	$Q_i \cap Q_j\neq\emptyset$, thus any server $s\in Q_i\cap Q_j$ reply to both $\phi$ and $\gamma$ actions.  
	By Lemma \ref{lem:server:tag:monotonic} and since $s$ received a tag $\tau$, then $s$ replies to $\pr_2$ with a tag
	$\tau_s\geq\tau$. Since $\gamma$ returns the maximum tag it discovers then $\tau_\gamma \geq \tau_s$. Therefore
	$\tau_\gamma \geq \tau$ and this completes the proof.
\end{proof}

With similar arguments and given that each value is associated with a unique tag then we can show the following lemma.

\begin{lemma}
	\label{lem:putdata:getdata}
	Let $\pi$ be a $\daputdata{c}{\tup{\tau,v}}$ action invoked by $\pr_1$ and $\phi$ be a $\dagetdata{c}$ action
	invoked by $\pr_2$ in a configuration $c$, such that $\pi\bef\phi$ in an execution $\EX$ of the algorithm. 
	Then $\phi$ returns a tag-value  $\tup{\tau_\phi, v_\phi}$
	such that $\tau_\phi \geq \tau$. 
\end{lemma}

Finally we can now show that property \textbf{C2} also holds. 

\begin{lemma}
	If $\phi$ is a $\dagetdata{c}$ that returns $\tup{\tg{\pi}, v_\pi } \in \tsSet \times \valSet$, 
	then there exists $\pi$ such that $\pi$ is a $\daputdata{c}{\tup{\tg{\pi}, v_{\pi}}}$ and $\phi \not \rightarrow \pi$.
\end{lemma}

\begin{proof}
	This follows from the facts that (i) servers set their tag-value pair to a pair received by a $\act{put-data}$ action, and (ii) 
	a $\act{get-data}$ action returns a tag-value pair that it received from a server. So if a $\dagetdata{c}$  operation $\phi$ 
	returns a tag-value pair $\tup{\tg{\pi}, v_\pi }$, there should be a server $s$  that replied to that operation with 
	$\tup{\tg{\pi}, v_\pi }$,  and $s$ received $\tup{\tg{\pi}, v_\pi }$ from some $\daputdata{c}{\tup{\tg{\pi}, v_\pi }}$
	action, $\pi$. Thus, $\pi$ can proceed or be concurrent with $\phi$, and hence $\phi\not\bef \pi$.
\end{proof}



==> ssec-correct-recon.tex <==
In this section we analyze the properties that we can achieve through our reconfiguration algorithm. 
The first lemma shows that any two configuration sequences have the same configuration identifiers
in the same indexes. 

\begin{lemma}
\label{lem:consconf}
	For any reconfigurer $r$ that invokes an $\act{reconfig}(c)$ action in an execution $\EX$ 
	of the algorithm, If $r$ chooses to install $c$ in index $k$ of its local $r.cseq$ vector, then $r$ invokes 
	the $Cons[k-1].propose(c)$ instance over configuration $r.cseq[k-1].cfg$.
\end{lemma}

\begin{proof}
	It follows directly from the algorithm. 
\end{proof}

\begin{lemma}
	\label{lem:server:monotonic}
	If a server $s$ sets $s.nextC$ to $\tup{c,F}$ at some state $\st$ in an execution $\EX$ 
	of the algorithm, then $s.nextC = \tup{c,F}$ for any state $\st'$ that appears after $\st$ in 
	$\EX$.
\end{lemma}

\begin{proof}
	Notice that a server $s$ updates the $s.nextC$ variable for some specific configuration $c_k$ 
	in a state $st$ if: (i) $s$ did not receive any value for $c_k$ before (and thus $nextC=\bot$), or (ii) $s$ 
	received a tuple $\tup{c,P}$ and before $\st$ received the tuple $\tup{c',F}$. By Observation \ref{obs:consensus}
	$c=c'$ as $s$ updates the $s.nextC$ of the same configuration $c_k$. Once the tuple becomes equal to 
	$\tup{c,F}$ then $s$ does not satisfy the update condition for $c_k$, and hence in any state $\st'$ after $\st$
	it does not change $\tup{c,F}$.
\end{proof}

\begin{lemma}[Configuration Uniqueness]
\label{lem:unique}

	%Let $\st_1$ and $\st_2$ be any two states of an execution $\EX$ of the algorithm,
	%and $\pr, q$ two participating processes. 
	%be the state after the response action of an operation $\op_1$ from process $p$,
	%and $\st_2$ be the state after the first $\act{read-config}$ call of an operation $\op_2$ from $q$.
	For any processes $\pr, q\in \idSet$ and any states $\st_1, \st_2$ in an execution $\EX$, it must hold that 
	$\config{\cvec{\pr}{\st_1}[i]}=\config{\cvec{q}{\st_2}[i]}$,  $\forall i$ s.t. 
	$\config{\cvec{\pr}{\st_1}[i]},\config{\cvec{q}{\st_2}[i]}\neq \bot$.
\end{lemma}

\begin{proof}
	The lemma holds trivially for $\config{\cvec{\pr}{\st_1}[0]}=\config{\cvec{q}{\st_2}[0]}=c_0$. 
	So in the rest of the proof we focus in the case where $i > 0$. Let us assume 
	w.l.o.g. that $\st_1$ appears before $\st_2$ in $\EX$.
	
	According to our algorithm a process $\pr$ sets $\pr.cseq[i].cfg$ to a configuration 
	identifier $c$ in two cases: (i) either it received $c$ as the result of the consensus 
	instance in configuration $\pr.cseq[i-1].cfg$, or (ii) $\pr$ receives $\config{s.nextC} = c$ from 
	a server $s\in\servers{\config{\pr.cseq[i-1]}}$. Note here that (i) is possible only 
	when $\pr$ is a reconfigurer and attempts to install a new configuration. On the 
	other hand (ii) may be executed by any process in any operation that invokes the 
	$\act{read-config}$ action. We are going 
	to proof this lemma by induction on the configuration index. 
	

	\emph{Base case:} The base case of the lemma is when $i=1$. 
	Let us first assume that $p$ and $q$ receive $c_p$ and $c_q$, as the result of the consensus instance at $\pr.cseq[0].cfg$
	and $q.cseq[0].cfg$ respectively. By Lemma \ref{lem:consconf}, since both processes want to install a configuration 
	in $i=1$, then they have to run $Cons[0]$ instance over the configuration stored in their local $cseq[0].cfg$ variable. 
	Since $\pr.cseq[0].cfg=q.cseq[0].cfg=c_0$ then 
	both $Cons[0]$ instances run over the same configuration $c_0$ and according to Observation \ref{obs:consensus}  
	return the same value, say $c_1$. Hence $c_p=c_q=c_1$ and $\pr.cseq[1].cfg=q.cseq[1].cfg=c_1$.
	 
	 Let us examine the case now where $p$ or $q$ 
	assign a configuration $c$ they received from some server $s\in\servers{c_0}$. According to the
	algorithm only the configuration that has been decided by the consensus instance on 
	$c_0$ is propagated to the servers in $\servers{c_0}$. If $c_1$ is the decided configuration, then 
	$\forall s\in\servers{c_0}$ such that $s.nextC(c_0)\neq\bot$, it holds that $s.nextC(C_0) = \tup{c_1,*}$.
	So if $p$ or $q$ set $\pr.cseq[1].cfg$ or $q.cseq[1].cfg$ to some received configuration, then 
	$\pr.cseq[1].cfg = q.cseq[1].cfg = c_1$ in this case as well. 
	
     \emph{Hypothesis:} We assume  that 
	$\cvec{\pr}{\st_1}[k]=\cvec{q}{\st_2}[k]$  for some $k$, $k \geq 1$.
	
	%\noindent{\bf Induction Hypothesis:} 
	\emph{Induction Step:}  We need to show that the lemma holds for $i=k+1$.
	If both processes retrieve $\config{\pr.cseq[k+1]}$ and $\config{q.cseq[k+1]}$ through consensus, 
	then both $\pr$ and $q$ run consensus
	over the previous configuration. Since according to our hypothesis 
	$\cvec{\pr}{\st_1}[k]=\cvec{q}{\st_2}[k]$ then both process will receive the same
	decided value, say $c_{k+1}$, and hence $\pr.cseq[k+1].cfg=q.cseq[k+1].cfg=c_{k+1}$. Similar to the base case,
	a server in $\servers{c_k}$ only receives the configuration $c_{k+1}$ decided by the consensus instance run over $c_k$. 
	So processes 
	$\pr$ and $q$ can only receive $c_{k+1}$ from some server in $\servers{c_k}$ 
	%even if the processes update their $\pr.cseq[k+1].cfg$ or $q.cseq[k+1].cfg$ with a received 
	%configuration that will be equal to 
	so they can only assign $\pr.cseq[k+1].cfg=q.cseq[k+1].cfg=c_{k+1}$ at Line \ref{algo:reconfigurer}:\ref{line:readconfig:assign}.
	That completes the proof. 
\end{proof}


Lemma \ref{lem:unique} showed that any two operations store the same
configuration in any cell $k$ of their $cseq$ variable. It is not known however 
if the two processes discover the same number of configuration ids. In the following
lemmas we will show that if a process learns about a configuration in a cell $k$ 
then it also learns about all configuration ids for every index $i$, such that $0\leq i\leq k-1$.

\begin{lemma}
\label{lem:confmonotonic}
	In any execution $\EX$ of the algorithm , If for any process $\pr\in\idSet$, $\cvec{\pr}{\st}[i]\neq\bot$ in some state $\st$ in $\EX$,
	then $\cvec{\pr}{\st'}[i]\neq\bot$ in any state $\st'$ that appears after $\st$ in $\EX$. 
\end{lemma}

\begin{proof}
	A value is assigned to $\cvec{\pr}{*}[i]$ either after the invocation of a consensus instance, or while executing
	the $\act{read-config}$ action. Since any configuration proposed for installation cannot be $\bot$ (A\ref{algo:reconfigurer}:\ref{line:install:valid}), 
	and since there is at least one configuration proposed in the consensus instance (the one from $\pr$), then by the validity of the consensus
	service the decision will be a configuration $c\neq\bot$. Thus, in this case $\cvec{\pr}{*}[i]$ cannot be $\bot$.
	Also in the $\act{read-config}$ procedure, $\cvec{\pr}{*}[i]$ is assigned to a value different than $\bot$ according
	to Line A\ref{algo:reconfigurer}:L\ref{line:readconfig:assign}. Hence, if $\cvec{\pr}{\st}[i]\neq\bot$ at state $\st$ 
	then it cannot become $\bot$ in any state $\st'$ after $\st$ in execution $\EX$.
\end{proof}


\begin{lemma}
\label{lem:nogaps}
	Let $\st_1$ be some state in an execution $\EX$ of the algorithm. Then for any 
	process $\pr$, if $k = max\{i: \cvec{\pr}{\st_1}[i]\neq \bot\}$, then 
	$\cvec{\pr}{\st_1}[j]\neq \bot$, for $0\leq j < k$.
\end{lemma}
\begin{proof}
	Let us assume to derive contradiction that there exists $j < k$ such that 
	$\cvec{\pr}{\st_1}[j]=\bot$ and $\cvec{\pr}{\st_1}[j+1]\neq\bot$.
	Suppose w.l.o.g. that $j = k-1$ and that $\st_1$ is the state immediately 
	after the assignment of a value to $\cvec{\pr}{\st_1}[k]$, say $c_k$. 
	Since $\cvec{\pr}{\st_1}[k]\neq\bot$, then $\pr$ assigned $c_k$ to $\cvec{\pr}{\st_1}[k]$ 
	in one of the following cases: 
	(i) $c_k$ was the result of the consensus instance, or
	(ii) $\pr$ received $c_k$ from a server during a $\act{read-config}$ action.
	The first case is trivially impossible as according to Lemma \ref{lem:consconf} 
	$\pr$ decides for $k$ when it runs consensus over configuration $\config{\cvec{\pr}{\st_1}[k-1]}$. 
	Since this is equal to $\bot$, then we cannot run consensus over a non-existent set of 
	processes. 	In the second case, $\pr$ assigns $\cvec{\pr}{\st_1}[k] = c_k$  in Line A\ref{algo:parser}:\ref{line:readconfig:assign}.
	The value $c_k$ was however obtained when $\pr$ invoked $\act{get-next-config}$ on 
	configuration $\config{\cvec{\pr}{\st_1}[k-1]}$. In that action, $\pr$ sends {\sc read-config}
	messages to the servers in $\servers{\config{\cvec{\pr}{\st_1}[k-1]}}$ and waits until a quorum 
	of servers replies. Since we assigned $\cvec{\pr}{\st_1}[k] = c_k$ it means that $\act{get-next-config}$
	terminated at some state $\st'$ before $\st_1$ in $\EX$, and thus: 
	(a) a quorum of servers in $\servers{\config{\cvec{\pr}{\st'}[k-1]}}$
	replied, and (b) there exists a server $s$ among those that replied with $c_k$. 
	According to our assumption however, $\cvec{\pr}{\st_1}[k-1] = \bot$ at $\st_1$. 
	So if state $\st'$ is before $\st_1$ in $\EX$, %is the state after the response step of $\act{get-next-config}$, 
	then by Lemma \ref{lem:confmonotonic}, it follows that $\cvec{\pr}{\st'}[k-1] = \bot$. This however 
	implies that $\pr$ communicated with an empty configuration, and thus no server replied to $\pr$. 
	This however contradicts the assumption that a server replied with $c_k$ to $\pr$. 
	
	Since any process traverses the configuration sequence starting from the initial 
	configuration $c_0$, then with a simple induction we can show that 
	$\cvec{\pr}{\st_1}[j]\neq \bot$, for $0\leq j\leq k$.
\end{proof}

We can now move to an important lemma that shows that any \act{read-config} action 
returns an extension of the configuration sequence returned by any previous \act{read-config} action. 
First, we show that the last finalized configuration observed by any \act{read-config} action is at least as 
recent as the finalized configuration observed by any subsequent \act{read-config} action. 
%Using this lemma we will then show that when 

\begin{lemma}
	\label{lem:config:propagation}
	If at a state $\st$ of an execution $\EX$ of the algorithm, if $\mu(\cvec{\pr}{\st}) = k$ % = \max\{i: \cvec{\pr}{\st}[i]\neq\bot\}$
	for some process $\pr$, then for any element $0\leq j < k$, $\exists Q\in \quorums{\config{\cvec{\pr}{\st}[j]}}$
	such that $\forall s\in Q, s.nextC(\config{\cvec{\pr}{\st}[j]})= \cvec{\pr}{\st}[j+1]$. 
\end{lemma}
\begin{proof}
	This lemma follows directly from the algorithm. Notice that whenever a process assigns a value to 
	an element of its local configuration (Lines  A\ref{algo:parser}:\ref{line:readconfig:assign} and 
	A\ref{algo:reconfigurer}:\ref{line:addconfig:assign}), it then propagates this value to a quorum of the 
	previous configuration (Lines  A\ref{algo:parser}:\ref{line:readconfig:put} and 
	A\ref{algo:reconfigurer}:\ref{line:addconfig:put}). So if a process $\pr$ assigned $c_j$ to an 
	element $\cvec{\pr}{\st'}[j]$ in some state $\st'$ in $\EX$, then $\pr$ may assign a value 
	to the $j+1$ element of $\cvec{\pr}{\st''}[j+1]$ only after $\act{put-config}(\config{\cvec{\pr}{\st'}[j-1]},\cvec{\pr}{\st'}[j])$
	occurs. During $\act{put-config}$ action, $\pr$ propagates $\cvec{\pr}{\st'}[j]$ in a quorum 
	$Q\in\quorums{\config{\cvec{\pr}{\st'}[j-1]}}$. Hence, if $\cvec{\pr}{\st}[k]\neq\bot$, then $\pr$ 
	propagated each $\cvec{\pr}{\st'}[j]$, for $0<j\leq k$ to a quorum of servers $Q\in\quorums{\config{\cvec{\pr}{\st'}[j-1]}}$.
	And this completes the proof. 
%	
%	Let examine a single element $\cvec{\pr}{\st'}[j]$ that is added in the configuration vector at some state $\st'$ 
%	that appears before $\st$ in $\EX$. Whenever a configuration is assigned a process $\pr$ invokes $\act{put-config}$
%	action before adding the next configuration. According to this action, the process sends the discovered configuration
%	and sends it to a quorum of servers. As this process is repeated for every element inserted then the lemma follows. 
\end{proof}


\begin{lemma}[Configuration Prefix]
	\label{lem:prefix}
Let $\op_1$ and $\op_2$ two 
%read/write/install operations 
completed \act{read-config} actions invoked by processes $\pr_1, \pr_2\in\idSet$ 
respectively, such that $\op_1\bef\op_2$ in an execution $\EX$. Let $\st_1$ be the state after the response 
step of $\op_1$ and $\st_2$ the state after the response step 
%termination of the first $\act{read-config}$ 
of $\op_2$. Then 
$\cvec{\pr_1}{\st_1}\preceq_p\cvec{\pr_2}{\st_2}$.
\end{lemma}

\begin{proof}
	Let $\nu_1 = \nu(\cvec{\pr_1}{\st_1})$ and $\nu_2 = \nu(\cvec{\pr_2}{\st_2})$.
	By Lemma \ref{lem:unique} for any $i$ such that $\cvec{\pr_1}{\st_1}[i]\neq\bot$ and 
	$\cvec{\pr_2}{\st_2}[i]\neq\bot$, then $\config{\cvec{\pr_1}{\st_1}[i]}=\config{\cvec{\pr_2}{\st_2}[i]}$.
	Also from Lemma \ref{lem:nogaps} we know that for $0\leq j\leq \nu_1, \cvec{\pr_1}{\st_1}[j] \neq \bot$, 
	and $0\leq j\leq \nu_2, \cvec{\pr_2}{\st_2}[j] \neq \bot$. So if we can show that $\nu_1\leq \nu_2$ then the lemma follows. 
	
	Let $\mu = \mu(\cvec{\pr_2}{\st'})$ %, or simply $\mu$, 
	be the last finalized element which $\pr_2$ established in the beginning of 
	the $\act{read-config}$ action $\op_2$ (Line A\ref{algo:reconfigurer}:\ref{line:readconfig:final}) at some state $\st'$ before $\st_2$. 
	It is easy to see that $\mu\leq \nu_2$. If $\nu_1 \leq \mu$ then $\nu_1\leq \nu_2$ and 
	the lemma follows. Thus, it remains
	to examine the case where $\mu < \nu_1$. Notice that since $\op_1\bef\op_2$ then $\st_1$ appears before 
	$\st'$ in execution $\EX$. By Lemma \ref{lem:config:propagation}, we know that by $\st_1$, 
	%in all the configurations $\cvec{\pr_1}{\st_1}[j]$, for $0\leq j < \nu_1$,  
	$\exists Q\in\quorums{\config{\cvec{\pr_1}{\st_1}[j]}}$, for $0\leq j < \nu_1$,   such that 
	$\forall s\in Q, s.nextC = \cvec{\pr_1}{\st_1}[j+1]$. Since $\mu < \nu_1$, then it must be the case 
	that $\exists Q\in \quorums{\config{\cvec{\pr_1}{\st_1}[\mu]}}$ such that $\forall s\in Q, s.nextC = \cvec{\pr_1}{\st_1}[\mu+1]$.
	But by Lemma \ref{lem:unique}, we know that $\config{\cvec{\pr_1}{\st_1}[\mu]}= \config{\cvec{\pr_2}{\st'}[\mu]}$. 
	Let $Q'$ be the quorum that replies to the $\act{read-next-config}$ occurred in $\pr_2$, on configuration  $\config{\cvec{\pr_2}{\st'}[\mu]}$.
	By definition $Q\cap Q'\neq \emptyset$, thus there is a server $s\in Q\cap Q'$ that sends $s.nextC = \cvec{\pr_1}{\st_1}[\mu+1]$
	to $\pr_2$ during $\op_2$. Since $\cvec{\pr_1}{\st_1}[\mu+1]\neq\bot$ then $\pr_2$ assigns $\cvec{\pr_2}{*}[\mu+1]=\cvec{\pr_1}{\st_1}[\mu+1]$, and 
	repeats the process in the configuration $\config{\cvec{\pr_2}{*}[\mu+1]}$. Since every configuration $\config{\cvec{\pr_1}{\st_1}[j]}$, 
		for $\mu\leq j<\nu_1$, has a quorum of servers with $s.nextC$, then by a simple induction it can be shown that the process will 
		be repeated for at least $\nu_1-\mu$ iterations, and  every configuration
		$\cvec{\pr_2}{\st''}[j]=\cvec{\pr_1}{\st_1}[j]$, at some state $\st''$ before $\st_2$. 
		Thus, $\cvec{\pr_2}{\st_2}[j]=\cvec{\pr_1}{\st_1}[j]$, for $0\leq j\leq \nu_1$. Hence $\nu_1\leq\nu_2$ and the lemma follows in this case as well. 
\end{proof}

Thus far we focused on the configuration member of each element in $cseq$. As operations do get in account
the \emph{status} of a configuration, i.e. $P$ or $F$, in the next lemma we will examine the relationship of 
the last finalized configuration as detected by two operations. First we present a lemma that shows the 
monotonicity of the finalized configurations.

\begin{lemma}
	\label{lem:final:monotonic}
	Let $\st$ and $\st'$ two states in an execution $\EX$ such that $\st$ appears before $\st'$ in $\EX$.
 	Then for any process $\pr$ must hold that $\mu(\cvec{\pr}{\st})\leq \mu(\cvec{\pr}{\st'})$.  %\red{must refer to a read-config}
\end{lemma}

\begin{proof}
	This lemma follows from the fact that if a configuration $k$ is such that 
	$\status{\cvec{\pr}{\st}[k]}=F$ at a state $\st$, then $\pr$ will start any 
	future $\act{read-config}$ action from a configuration $\config{\cvec{\pr}{\st'}[j]}$
	such that $j\geq k$. But $\config{\cvec{\pr}{\st'}[j]}$ is the last finalized configuration 
	at $\st'$ and hence $\mu(\cvec{\pr}{\st'})\geq \mu(\cvec{\pr}{\st})$.
\end{proof}

\begin{lemma}  [Configuration Progress]
	\label{lem:finalconf}
	Let $\op_1$ and $\op_2$ two 
	%read/write/install operations 
	completed \act{read-config} actions invoked by processes $\pr_1, \pr_2\in\idSet$ 
	respectively, such that $\op_1\bef\op_2$ in an execution $\EX$. 
	Let $\st_1$ be the state after the response 
	step of $\op_1$ and $\st_2$ the state after the response step 
	%after the completion of $\op_1$ and $\st_2$ the state after the termination of the first $\act{read-config}$ 
	of $\op_2$. Then 
	$\mu(\cvec{\pr_1}{\st_1})\leq\mu(\cvec{\pr_2}{\st_2})$.
\end{lemma}

\begin{proof}
	By Lemma \ref{lem:prefix} it follows that $\cvec{\pr_1}{\st_1}$ is a prefix of $\cvec{\pr_2}{\st_2}$.
	Thus, if $\nu_1 = \nu(\cvec{\pr_1}{\st_1})$ and $\nu_2 = \nu(\cvec{\pr_2}{\st_2})$, $\nu_1\leq\nu_2$.
	Let $\mu_1=\mu(\cvec{\pr_1}{\st_1})$, such that $\mu_1\leq\nu_1$, be the last element in $\cvec{\pr_1}{\st_1}$,
	where $\status{\cvec{\pr_1}{\st_1}[\mu_1]} = F$. Let now $\mu_2=\mu(\cvec{\pr_2}{\st'})$, 
	be the last element which $\pr_2$ obtained in Line A\ref{algo:parser}:\ref{line:readconfig:final} 
	during $\op_2$ 
	%of the  $\act{read-config}$ action 
	such that $\status{\cvec{\pr_2}{\st'}[\mu_2]} = F$ in some state $\st'$ before $\st_2$. 
	If $\mu_2\geq\mu_1$, and since $\st_2$ is after $\st'$, then by Lemma \ref{lem:final:monotonic} 
	$\mu_2\leq \mu(\cvec{\pr_2}{\st_2})$ and hence $\mu_1\leq \mu(\cvec{\pr_2}{\st_2})$ as well. 
	
	It remains to examine the case where $\mu_2<\mu_1$. Process  $\pr_1$ 
	sets the status of $\cvec{\pr_1}{\st_1}[\mu_1]$ to $F$ in two cases: (i) either when finalizing 
	a reconfiguration, or (ii) when receiving an $s.nextC = \tup{\config{\cvec{\pr_1}{\st_1}[\mu_1]}, F}$ %with status $F$ 
	from some server $s$ during a $\act{read-config}$ action. In both cases $\pr_1$ propagates the 
	$\tup{\config{\cvec{\pr_1}{\st_1}[\mu_1]}, F}$ to a quorum of servers in  
	$\config{\cvec{\pr_1}{\st_1}[\mu_1-1]}$ before completing. We know by Lemma
	\ref{lem:prefix} that since $\op_1\bef\op_2$ then $\cvec{\pr_1}{\st_1}$ is a prefix 
	in terms of configurations of the $\cvec{\pr_2}{\st_2}$. So it must be the case 
	that $\mu_2 < \mu_1 \leq \nu(\cvec{\pr_2}{\st_2})$. Thus, during $\op_2$, %the $\act{read-config}$ action, 
	$\pr_2$ starts from the configuration at index $\mu_2$ and in some iteration 
	performs $\act{get-next-config}$ in configuration $\cvec{\pr_2}{\st_2}[\mu_1-1]$. 
	According to Lemma \ref{lem:unique}, $\config{\cvec{\pr_1}{\st_1}[\mu_1-1]} = \config{\cvec{\pr_2}{\st_2}[\mu_1-1]}$.
	Since $\op_1$ completed before $\op_2$, then it must be the case that $\st_1$ appears before 
	$\st'$ in $\EX$. However, $\pr_2$ invokes the $\act{get-next-config}$ operation in a state $\st''$
	which is either equal to $\st'$ or appears after $\st'$ in $\EX$. Thus, $\st''$ must appear after $\st_1$ in $\EX$.
	From that it follows that when the $\act{get-next-config}$ is executed by $\pr_2$ there is already 
	a quorum of servers in $\config{\cvec{\pr_2}{\st_2}[\mu_1-1]}$, say $Q_1$, that received 
	$\tup{\config{\cvec{\pr_1}{\st_1}[\mu_1]}, F}$from $\pr_1$. 
	Since, $\pr_2$ waits from replies from a quorum of servers from the same configuration, say $Q_2$, and since the 
	$nextC$ variable at each server is monotonic (Lemma \ref{lem:server:monotonic}), then there is a server $s\in \quo{1}\cap \quo{2}$, 
	such that $s$ replies to $\pr_2$ with $s.nextC = \tup{\config{\cvec{\pr_1}{\st_1}[\mu_1]}, F}$. So, 
	$\cvec{\pr_2}{\st_2}[\mu_1]$ gets $\tup{\config{\cvec{\pr_1}{\st_1}[\mu_1]}, F}$, and 
	hence $\mu(\cvec{\pr_2}{\st_2})\geq \mu_1$ in this case as well. This completes our proof.
\end{proof}

\begin{theorem}
	Let $\op_1$ and $\op_2$ two 
%read/write/install operations 
completed \act{read-config} actions invoked by processes $\pr_1, \pr_2\in\idSet$ 
respectively, such that $\op_1\bef\op_2$ in an execution $\EX$. 
Let $\st_1$ be the state after the response 
step of $\op_1$ and $\st_2$ the state after the response step 
%after the completion of $\op_1$ and $\st_2$ the state after the termination of the first $\act{read-config}$ 
of $\op_2$.
%$\cvec{\pr_1}{\st_1}$ and $\cvec{\pr_2}{\st_2}$ at two states $\st_1$ and $\st_2$ 
%in an execution $\EX$ of the algorithm  such that $\st_1$ appears before $\st_2$ in $\EX$. 
Then the following properties hold: 
\begin{enumerate}
\item [$(a)$] 
$\cvec{\pr_2}{\st_2}[i].cfg = \cvec{\pr_1}{\st_1}[i].cfg$,  for $ 1 \leq i \leq \nu(\cvec{\pr_1}{\st_1})$,
\item [$(b)$]
 %$(b)$  
 $\cvec{\pr_1}{\st_1}  \preceq_p \cvec{\pr_2}{\st_2}$, and
\item [$(c)$] 
%$(c)$  
  $\mu(\cvec{\pr_1}{\st_1}) \leq \mu(\cvec{\pr_2}{\st_2})$
  %; and 
%\item [$(d)$]  
%\nn{????$(d)$  $\cvec{\pr_2}{\st_2}[i]   = \cvec{\pr_1}{\st_1}[i]$,  for  $ 1 \leq i \leq \mu(\cvec{\pr_1}{\st_1})$????} 
\end{enumerate}
\end{theorem}

\begin{proof}
Statements $(a)$, $(b)$ and $(c)$ follow from Lemmas \ref{lem:unique}, \ref{lem:prefix}, and 
\ref{lem:final:monotonic}.
%are from  the atomic read-modify-write property of ${\recBox}.\act{add-config}(\cdot)$ 
%and $(d)$ is due to the recon client.
\end{proof}

==> time_analysis_short_v2.tex <==
\myparagraph{\ares{} Correctness.}
The correctness of \ares{} highly depends on the way the configuration 
sequence is constructed at each client process. Let $\cvec{p}{\state}$ 
denote the configuration sequence $cseq$ at process $p$ in a state $\state$ and 
$\mu(\cvec{\pr}{\state})$ the index of the last finalized configuration in $\cvec{p}{\state}$. 
Then the following properties are preserved by the reconfiguration service:

\begin{theorem}
	Let $\op_1$ and $\op_2$ two 
	%read/write/install operations 
	completed \act{read-config} actions invoked by processes $\pr_1, \pr_2\in\idSet$ 
	respectively, such that $\op_1\bef\op_2$ in an execution $\EX$. 
	Let $\state_1$ the state after the response 
	step of $\op_1$ and $\state_2$ the state after the response step 
	%after the completion of $\op_1$ and $\state_2$ the state after the termination of the first $\act{read-config}$ 
	of $\op_2$.
	%$\cvec{\pr_1}{\state_1}$ and $\cvec{\pr_2}{\state_2}$ at two states $\state_1$ and $\state_2$ 
	%in an execution $\EX$ of the algorithm  such that $\state_1$ appears before $\state_2$ in $\EX$. 
	Then the following properties hold: 
	%\begin{enumerate}
		%\item [$(a)$] 
		$(a)$ \textbf{Configuration Consistency}: 
		$\cvec{\pr_2}{\state_2}[i].cfg = \cvec{\pr_1}{\state_1}[i].cfg$,  for $ 1 \leq i \leq |\cvec{\pr_1}{\state_1}|$,
		%\item [$(b)$]
		$(b)$  
		\textbf{Seq. Prefix}: $\cvec{\pr_1}{\state_1}  \preceq_p \cvec{\pr_2}{\state_2}$, and
		%\item [$(c)$] 
		$(c)$  
		\textbf{Seq. Progress}: $\mu(\cvec{\pr_1}{\state_1}) \leq \mu(\cvec{\pr_2}{\state_2})$
		%; and 
		%\item [$(d)$]  
		%\nn{????$(d)$  $\cvec{\pr_2}{\state_2}[i]   = \cvec{\pr_1}{\state_1}[i]$,  for  $ 1 \leq i \leq \mu(\cvec{\pr_1}{\state_1})$????} 
	%\end{enumerate}
\end{theorem}

Given the properties satisfied by the reconfiguration algorithm of \ares{} 
and assuming that the DAP used satisfy Property~\ref{property:dap}, as presented
in Section \ref{ssec:dap}, then  we have the following result. 

\begin{theorem}[Atomicity]
	In  any execution $\EX$ of \ares{}, if in every configuration $c\in\gseq$,
	$\dagetdata{c}$, $\daputdata{c}{}$, and $\dagettag{c}$
	 %the DAP primitives  
	 satisfy Property~\ref{property:dap}, then ~\ares{} satisfy atomicity.
	%, given that the 
	%$\act{get-data}$, $\act{get-tag}$, and $\act{put-data}$ primitives used satisfy properties
	%\textbf{C1} and \textbf{C2} of Definition \ref{def:consistency}.
\end{theorem}

%In  \ares{},  each configuration 
%may implement the DAPs in a different way as stated below:

\begin{remark}
	Algorithm \ares{} satisfies atomicity even when the implementaton of the  DAPs in two 
	different configurations $c_1$ and $c_2$ are not the same, given that the $c_i.\act{get-tag}$,
	$c_i.\act{get-data}$, and the $c_i.\act{put-data}$ primitives 
	in each $c_i$ satisfy Property~\ref{property:dap}.  
\end{remark}

\subsection{Storage and Communication Costs for \ares{}.}\label{sec:safety:c}
We now briefly present the storage and communication costs associated with the presented DAPs.
%{\treas{}  %Due to space limitations the proofs appear in \cite{}.
Recall that by our assumption, the storage cost counts the size (in bits) of the coded elements 
%that are locally stored, which are 
stored in variable  $List$  at each server. We ignore the storage cost due to meta-data.
For  communication cost we measure the bits sent on the wire between the nodes.

\begin{theorem}\label{treas:performance}
 The \ares{} algorithm has: (i) storage cost $(\delta +1 )\frac{n}{k}$, (ii) communication 
cost for each write at most to $\frac{n}{k}$, and (iii) communication 
cost for each read at most $(\delta +2)\frac{n}{k}$.
\end{theorem}

\subsection{Latency Analysis for read and writes in \ares{}}\label{sec:safety:d}
Liveness properties cannot be specified for ~\ares{}, without restricting asynchrony  or the
rate of arrival of \act{reconfig} operations, or if the consensus protocol never terminates.
Here,  we provide some conditional performance analysis of the operation, based on 
%assumptions on the 
latency bounds on the message \nnrev{delay}{delivery}. %in the network.
 We assume that local computations take negligible time and the latency of an 
operation is  due to the delays in the messages exchanged during the execution. 
%Before proceeding with our 
%analysis we define an upper and lower communication bounds. 
We measure delays in \myemph{time units} of some global clock, which is visible only to an external viewer.
No process has access to the clock.
Let $\smdelay$ and $\lgdelay$ be the minimum and maximum durations taken by 
 messages, sent during an execution  of~\ares,  to reach their destinations.
%denote the minimum message delivery delay 
%between any two processes in the service; let $\lgdelay$ be the 
%maximum delivery delay. 
 Also, let $\opdelay{\op}$ denote the duration 
 of an operation (or action) $\op$. In the statements that follow, 
 we consider any execution $\EX$ of \ares, which contains $k$ \act{reconfig} operations.
 \kmk{For any configuration $c$ in an execution of~\ares{},  we assume that any 
 	$\consensus{c}.\act{propose}$ operation, takes at least $\opdelaymin{CN}$ time units.}
%  in it 
% and $\smdelay$ and $\lgdelay$ are the minimum and maximum durations taken by 
%any message sent during an execution to reach its destination.
% with the above time bounds 
%for messages transmitted. 
%%
%\myparagraph{Notations}
%Let $\smdelay$ and $\lgdelay$ be the minimum and maximum durations taken by 
%any message to go from one process to another.
%denote the minimum message delivery delay 
%between any two processes in the service; let $\lgdelay$ be the 
%maximum delivery delay. 
% Also, let $\opdelay{\op}$ denote the communication  delay of an operation (or action) $\op$. 
%The latency results are the following. 
%For the simplicity of our analysis, we assume that any 
%\act{propose} operation to a consensus instance takes at least   $\opdelaymin{CN}$ time units
 %and at most $\opdelaymax{CN}$. If $\op$ is any propose operation to a consensus service then 
%$\opdelaymin{CN} \leq \opdelay{\op} \leq \opdelaymax{CN}$.
 %time units.
\remove{
\begin{lemma}
\label{lem:opdelays}
Suppose $\pi$ and $\phi$ are operations of the type \act{put-config}, \act{read-next-config}, respectively, invoked by some non-faulty reconfiguration clients,  then the latency of these operations are bounded as follows: 
%\begin{itemize}
	%\item 
	$(i)$ $2\smdelay\leq \opdelay{\pi}\leq 2\lgdelay$
	%\item 
	and 
	$(ii)$ $2\smdelay\leq \opdelay{\phi}\leq 2\lgdelay$.
%\end{itemize}
\end{lemma}

From Lemma \ref{lem:opdelays} we can derive the delay of  a \act{read-config} action.
\begin{lemma}
	\label{lem:rcdelay}
	Let $\phi$ be a $\act{read-config}$ operation invoked by a non-faulty reconfiguration client, 
	with the input argument and returned values of $\phi$ as  $seq$ and  $seq'$, respectively. 
	If  $\mu = \mu(seq)$ and $\nu = \nu(seq')$, then 	
$4\smdelay(\nu-\mu+1)\leq \opdelay{\phi}\leq 4\lgdelay(\nu-\mu+1)$.
\end{lemma}

From Lemma \ref{lem:rcdelay} it is clear that the latency of a $\act{read-config}$ action 
is  dependent on the number of configurations installed since the last  finalized configuration known to the 
 recon client.
Let $\seqlen = \nu-\mu$ denote the number of newly installed configurations.
%Now let us examine when a new configuration gets inserted in the configuration 
%sequence by a \act{reconfig} operation.
Given the latency of a \act{read-config}, we can compute the minimum amount 
of time it takes for $k$ configurations to be installed.

\begin{lemma}
	\label{lem:configdelay}
	Let $\sigma$ be the last state of a fair execution of \ares{}, $\EX$. 
	Then $k$ configurations can be installed to $\cvec{}{\sigma}$, in time no less than
%	\begin{equation}
	$ \left(\opdelaymin{CN}+6\smdelay\right)k$.
%	\end{equation}
	%by the completion of its $\act{add-config}$ action 
%	in our execution construction.
\end{lemma}
}
\remove{
 In \ares{} a \act{reconfig} operation has 
four phases: $(i)$ $\act{read-config}(cseq)$,  reads the latest configuration sequence, 
$(ii)$ $\text{\act{add-config}}(cseq, c)$,  attempts to add  the new configuration 
at the end of the global sequence $\mathcal{G}_L$, 
$(iii)$ $\text{\act{update-config}}(cseq)$,   transfers the knowledge to the added configuration,
and 
$(iv)$  $\text{\act{finalize-config}}(cseq)$ finalizes the added configuration. 

%So, a new configuration is appended to the 
%end of the configuration sequence (and it becomes visible to any operation) during the 
%\act{add-config} action. 
 During the execution of \act{add-config} action, the recon client proposes to a consensus 
service  
to learn the configuration to accept, and then invokes a \act{put-config} action notify a quorum of servers in the configuration of the  decided configuration. 
%Any operation that is invoked after the \act{put-config} action 
%will observed the newly added configuration. 

When multiple reconfiguration operations  are invoked concurrently, each at a separate client, then it is possible 
that each of the clients  successfully append their  new  configurations to the end of $\mathcal{G}_L$. 
This is possible when 
the \act{read-config} action of each \act{reconfig} operation begins  after the completion of  \act{put-config}
action of another \act{reconfig} operation. 
}

%Next we 
The following lemma shows the maximum latency of a read or a write operation, invoked by any non-faulty client. 
From~\ares{} algorithm,  the latency of a read/write operation depends on the delays of the  DAPs  operations. 
%influence  the delay of a read and write operation. 
For our analysis we assume 
that all $\act{get-data}$, $\act{get-tag}$ and $\act{put-data}$ primitives use 
two phases of communication.  Each phase consists of a communication between the client and the servers.
%\kmkremove{Such an assumption is justified by atomic algorithms like ~\treas{} and ABD. }

\begin{lemma}
	\label{lem:dapdelays}
Suppose $\pi$,  $\phi$ and $\psi$ are operations of the type \act{put-data}, \act{get-tag} and  \act{get-data}, respectively, invoked by some non-faulty reconfiguration clients,  then the latency of these operations are bounded as follows: 
	$(i)$ $2\smdelay\leq \opdelay{\pi}\leq 2\lgdelay$; $(ii)$
	 $2\smdelay\leq \opdelay{\phi}\leq 2\lgdelay$; and $(iii)$
	  $2\smdelay\leq \opdelay{\psi}\leq 2\lgdelay$.
\end{lemma}
%Now we show the delay of a read or a write operation $\op$.

In the following lemma, we {estimate the time taken for a read or a write operation to complete,
	when it discovers $k$ configurations between its invocation and response steps.
%
%show that in a fair execution of ~\ares{} \nnrev{where there are at}{that contains} $k$ reconfiguration 
%operations, any read or write operation takes at most  $6\lgdelay\left(k+2\right)$.
 

\begin{lemma}
	\label{lem:rwdelay}
%Consider a execution of ~\ares{} where there are $k$ reconfiguration and a read or a write operation $\pi$ invoked by a non-faulty then   $6\lgdelay(k+1)$.
Consider any  execution of ~\ares{} where at most  $k$ reconfiguration operations are invoked.
Let $\sigma_s$ and $\sigma_e$ be the states before the invocation 
and after the completion step of a read/write operation $\op$,
in some fair execution $\EX$ of \ares{}. 
%If $k=\nu(\cvec{\pr}{\sigma_e}) - \mu(\cvec{\pr}{\sigma_s})$, 
Then we have 
$\opdelay{\op}\leq 6\lgdelay\left(k+2\right)$ to complete. 
\end{lemma}
\proofremove{
\begin{proof}
	Let $\state_s$ and $\state_e$ be the states before the invocation 
	and after the completion step of a read/write operation $\op$ by $\pr$ respectively,
	in some execution $\EX$ of \ares. 
	%Then $\op$ takes time at most:
%	\[
%		\opdelay{\op}\leq 6\lgdelay\left[\nu(\cvec{\pr}{\state_e}) - \mu(\cvec{\pr}{\state_s})+2\right]
%	\] 
	By algorithm examination we can 
	see that any read/write operation performs the following actions in this order:
	$(i)$  \act{read-config}, $(ii)$ \act{get-data} (or \act{get-tag}), $(iii)$ \act{put-data},
	and $(iv)$ \act{read-config}. Let $\state_1$ be the state when the first \act{read-config}, denoted by $\act{read-config}_1$, 
	action terminates. By Lemma \ref{lem:rcdelay} the action will take time:
	\[
		\opdelay{\act{read-config}_1} \leq 4\lgdelay(\nu(\cvec{\pr}{\state_1})-\mu(\cvec{\pr}{\state_s})+1)
	\]
	The $\act{get-data}$ action that follows the \act{read-config} (Lines Alg.~\ref{algo:writer}:\ref{line:rw:getdata:start}-\ref{line:rw:getdata:end}) is also executed at most $(\nu(\cvec{\pr}{\state_1})-\mu(\cvec{\pr}{\state_s})+1)$
	given that no new finalized configuration was discovered by the \act{read-config} action. 
	Finally, the \act{put-data}  and the second \act{read-config} actions of $\op$ may be invoked at most
	$(\nu(\cvec{\pr}{\state_e})-\nu(\cvec{\pr}{\state_1})+1)$ times, given that the \act{read-config} action discovers 
	one new configuration every time it runs. Merging all the outcomes, the total time of $\op$ can be at most:
	\begin{eqnarray*}
	\opdelay{\op} & \leq & 4\lgdelay(\nu(\cvec{\pr}{\state_1})-\mu(\cvec{\pr}{\state_s})+1) + 2\lgdelay(\nu(\cvec{\pr}{\state_1})-\mu(\cvec{\pr}{\state_s})+1) + (4\lgdelay+2\lgdelay)(\nu(\cvec{\pr}{\state_e})-\nu(\cvec{\pr}{\state_1})+1) \\
%	 & \leq & 6\lgdelay\nu(\cvec{\pr}{\state_1})-6\lgdelay\mu(\cvec{\pr}{\state_s})+6\lgdelay\nu(\cvec{\pr}{\state_e})-6\lgdelay\nu(\cvec{\pr}{\state_1})+12\lgdelay \\
	 & \leq & 6\lgdelay\left[\nu(\cvec{\pr}{\state_e}) - \mu(\cvec{\pr}{\state_s})+2\right] \leq 6D(k+1)
	\end{eqnarray*}
where  $\nu(\cvec{\pr}{\state_e}) - \mu(\cvec{\pr}{\state_s})\leq k + 1$ since there there can be at most $k$ new configurations installed. and the result of the lemma follows.
\end{proof}
}

It remains now to examine the conditions under which a read/write operation may “catch up” with an infinite number of reconfiguration operations.
For the sake of a worst case analysis we will assume that reconfiguration operations suffer 
the minimum delay $d$, whereas read and write operations suffer the maximum
delay $D$ in each message exchange. Also, we assume that any consensus operation takes the least amount of time to complete $\opdelaymin{CN}$.
The following theorem is the main result of this section, in which we define the relation between $\opdelaymin{CN}$, $d$ and $D$
%show that in any fair execution of ~\ares{}, if the  consensus operations are ``slow enough'' then  
so to guarantee that any read or write issued by a non-faulty client always terminates.

\begin{theorem}
%Consider a  read or  write operation $\pi$, invoked by a non-faulty client, in a fair and well-formed execution of ~\ares{}. Suppose at the point of invocation of $\pi$ the client has $|cseq| = p$. Then if $\opdelaymin{CN} \geq 6D(p + 2) -5d$ the operation $\pi$ completes.
 Suppose  $\opdelaymin{CN} \geq 3(6D-\smdelay)$, then  any  read or write operation $\op$ completes in any execution  $\EX$ of 
\ares{}  for any number of reconfiguration operations in $\EX$.
%$\smdelay \geq \frac{3\lgdelay}{k}-\frac{\opdelay{CN}}{2(k+2)}$
\end{theorem}

\remove{

It remains now to examine if a read/write operation may ``catch up'' with any ongoing 
reconfigurations. 
For the sake of a worst case analysis we will assume that reconfiguration operations
may communicate respecting the minimum delay $\smdelay$, whereas read and write 
operations suffer the maximum delay $\lgdelay$ in each message exchange. We will
split our analysis into three directions, with respect to the number of configurations 
installed $k$, and the bound on the minimum delay $\smdelay$:
$(i)$  $k$ is finite, and $\smdelay$ may be unbounded small; $(ii)$ 
$k$ is infinite, and $\smdelay$ may be unbounded small;
$(iii)$  $k$ is infinite, and $\smdelay$ can be bounded.

\myparagraph{$k$ is finite, and $\smdelay$ may be unbounded small.}
In this case we assume a finite number of installed configurations. Also,
as the $\smdelay$ is unbounded, it follows that reconfigurations may be 
installed almost instantaneously. Let us first examine what is the maximum 
delay bound of a any read/write operation. 

\myparagraph{$k$ is infinite, and $\smdelay$ is bounded.}
We will compute the bound on $\smdelay$ with respect to the $\lgdelay$ 
and the number of configurations to be installed $k$ if we want to allow a 
read/write operation to reach ongoing reconfigurations. 

\begin{lemma} \label{lem:delaybound}
	A read/write operation $\op$ may terminate in any execution $\EX$ of 
	\ares{} given that $k$ configurations are installed during $\op$, if
	$
	\smdelay \geq \frac{3\lgdelay}{k}-\frac{\opdelaymin{CN}}{2(k+2)}
	$
\end{lemma}
%\proofremove{
\begin{proof}
	By Lemma \ref{lem:configdelay}, $k$ configurations may be installed in at least:
		$\opdelay{k} \geq 4\smdelay\sum_{i=1}^{k}i+ k\left(\opdelaymin{CN}+2\smdelay\right)$.	
	Also by Lemma \ref{lem:rwdelay}, we know that operation $\op$ takes at most 
$	\opdelay{\op}\leq 6\lgdelay\left(\nu(\cvec{\pr}{\state_e}) - \mu(\cvec{\pr}{\state_s})+2\right)$.
	Assuming that $k=\nu(\cvec{\pr}{\state_e}) - \mu(\cvec{\pr}{\state_s})$, the total number of 
	configurations observed during $\op$, then $\op$ may terminate before a $k+1$ configuration 
	is added in the configuration sequence if 
	  $6\lgdelay(k+2) \leq  4\smdelay\sum_{i=1}^{k}i+ k\left(\opdelaymin{CN}+2\smdelay\right)$ then we have
	  $d \geq \frac{3\lgdelay}{k}-\frac{\opdelaymin{CN}}{2(k+2)}$.
	And that completes the lemma. 
\end{proof}
%}
}

%\begin{theorem*}{\bf \ref{safety:ares:treas}} (Atomicity)
%	Algorithm \ares-\treas{} implements a reconfigurable atomic storage service, given that the 
%	$\act{get-data}$, $\act{get-tag}$, and $\act{put-data}$ primitives used satisfy properties
%	\textbf{C1} and \textbf{C2} of Definition \ref{def:consistency}.
%\end{theorem*}
%
%\begin{proof}
%The figure above \ref{fig:reconfig:ares:treas}
%\end{proof}


==> transferstate_v1.tex <==

\algblockdefx[Receiv]{Receiv}{EndReceiv}%
[3]{{\bf Upon recv} (#1)$_{\text{ #2 }}${\bf from} #3}%
{{\bf end receive}} 
In this section, we provide an optimization on the reconfiguration process presented in \ares{}. 
%show that \treas{} can be 
In particular, we discuss how to reduce the communication overhead caused by the state transfer during the transition from a \emph{finalized} to a \emph{newly installed} configuration, by 
%adapt \ares{} to 
allowing servers to exchange directly object values,
and avoiding the recon client intervention.
%reconfiguration where the object values are transferred directly
%from the servers a \emph{finalized} configuration,  to the servers of a \emph{newly installed} configuration, 
% and without the recon client handling object values.
% This will  caused by the state transfer, as object state will be transferred from server to server without the intervention from a recon client. 
%
According to \ares{} a recon client is required to 
collect the object values from the servers of the old
configuration and pass those object values over to the servers 
of the new configuration. With the proposed optimization, the recon client will first determine the
newly establish configuration and will inform the
servers of the old configuration to forward their 
object values to the servers of the new configuration.

To reach this goal, we modified the \act{update-config} procedure of the reconfiguration service, as well as 
%the changes needed to be applied to 
the protocol of the servers for allowing them to communicate the object values, as seen in Algs.~\ref{algo:reconfigurer:statetransfer:ares} and ~\ref{algo:server:statetransfer:treas}.
%to both the reconfiguration and the DAP implementation in \ares{}. 
%necessary to adapt \ares{} and \treas{} to achieve this. 
%Here every configuration uses \treas{} as the underlying atomic memory emulation algorithm, and  we refer to  this algorithm as \aresII{}.
%
%In \ares

 



More precisely, the procedure \act{update-config} (see Alg.~\ref{algo:reconfigurer}) is modified  as shown in 
Alg.~\ref{algo:reconfigurer:statetransfer:ares}. Consider a reconfiguration client $rc$, which invokes \act{update-config}, 
during a reconfiguration operation, where it iteratively gathers the tag-config ID pairs in the set variable $M$ by calling \act{get-tag} 
(lines Alg.~\ref{algo:reconfigurer:statetransfer:ares}: \ref{line:statetransfer:reconfig:start}-\ref{line:statetransfer:reconfig:end}). Suppose $\tup{\tau, C}$ is the tag and 
configuration ID pair corresponding to the highest tag 
in $M$ (lines Alg.~\ref{algo:reconfigurer:statetransfer:ares}:\ref{line:reconfig:max}). 
Next, $rc$ executes procedure  $\act{forward-code-element}(\text{{\sc req-fw-code-elem}}, \tau, C, C')$, 
 to send a request to the servers in $C$ to forward their respective 
coded elements corresponding to $\tau$, to  each server in   $\servers{C'}$.
% via  the call to the procedure 
%$\act{forward-code-element}(\text{{\sc req-fw-code-elem}}, \tau, C, C')$. 
Suppose the MDS code parameters in $C$ and $C'$ are $[n, k]$ and $[n', k']$, respectively, such that, $|\servers{C}| = n$, 
$|\servers{C'}| = n'$, and for some $k \geq \frac{2n}{3}$  and $k'\geq \frac{2n'}{3}$. In $\act{forward-code-element}$, 
the call to $\act{md-primitive}( \text{\sc req-fw-code-elem}, \tg{}, C')$, presented in ~\cite{KPKLMS16},  delivers the message 
({\sc req-fw-code-elem}, $\tg{}, C'$) 
to  either every non-faulty servers in $\servers{C}$ or  none. 

We rely on the  semantics of \act{md-primitive}~\cite{KPKLMS16} to avoid lingering of  coded elements for ever in 
$D$ due to crash failure of the $rc$, or servers in $\servers{C}$. For example, suppose  $rc$ communicates only to one server, say  $s_i$,  in $\servers{C}$ and crashes, then the rest of the servers in $C$ would not send their coded elements to the servers in $C'$. As a result, the coded element from $s_i$ will linger around in the  $D$ variables in the  servers in $\servers{C'}$ without ever being removed, thereby, progressively  increasing the storage cost.  
%
{\bf [NN: i cannot follow the next sentence. How does it solve the issue described in the previous sentens?]}Upon delivering these messages to any server $s_i$, in $\servers{C}$, 
 if   $(\tau, e_i)$ in $List$ in $s_i$,
%--possibly due to another ongoing reconfiguration, or $k'$ coded elements for $\tau$ have already arrived at $s_j'$--
 %\nn{[NN: How this is possible? When the server added this tag? These are the servers of the new config right?]} 
 then $s_i$ sends   $(\text{\sc fwd-code-elem}, \tup{\tg{}, e_i}, rc)$ to servers in $C'$. 

{\bf[NN: the paragraph below is a bit difficult to follow]}
Next upon receiving any of the  {\sc fwd-code-elem} messages, at any server $s'_j$ in $\servers{C'}$  if $rc \in Recons$ in  $s'_j$
(Alg.~\ref{algo:server:statetransfer:treas}:\ref{line:statetransfer:notify:check}) then it  ignores it because $rc$ has already been updated by $s'_j$ regarding the object value of $\tau$. Otherwise, $s'_j$ checks if $\tup{\tg, e_j} \in List$ (Alg.~\ref{algo:server:statetransfer:treas}:\ref{line:statetransfer:notify:checkList}), if is not, then $s'_j$ adds the incoming  pair
 $\tup{\tau, e_i}$ to $D$.
 Next,  $s'_j$ checks  if  the value for $\tau$ is decodable (Alg.~\ref{algo:server:statetransfer:treas}:\ref{line:statetransfer:notify:decodable}), from the coded elements in $D$, if it is,  then $s'_j$ decodes the value 
 $v$, using decoder for $C'$, with parameters $[n, k]$, and re-encodes, according to parameters $[n', k']$ to get $e_j' \equiv \Phi_{C'}(v)_j$. 
 Then $s'_j$  proceeds to store $\tup{\tau, e_j'}$
   in a similar steps as in the \act{put-data} response in the \treas{} (Alg.~\ref{algo:server:statetransfer:treas}). 
   Then in lines  Alg.~\ref{algo:server:statetransfer:treas}:\ref{line:statetransfer:notify:begin}-\ref{line:statetransfer:notify:end} if 
   $\tup{\tg{}, *} \in List$
   then  $s'_j$ adds $rc$ to the  list $Recons$ and $s_j'$ sends $rc$ an {\sc ack}. Finally, once $rc$ receives {\sc ack}s 
   from  $\left\lceil \frac{n' + k'}{2}\right\rceil$ servers in $\servers{C'}$ it completes the call to \act{update-config}.  
   Finally, it can be shown that 
   %\aresII{} 
   the updated implements an atomic memory service as stated in the following theorem.
%\nn{[NN:Is $t$ and $\tau$ the same in the algorithms?]}
\begin{algorithm}[!h]
	%\hrule \F
	\begin{algorithmic}[2]
		\begin{multicols}{2}{\scriptsize				
				\Procedure{update-config}{$seq$}
				\State $\mu\gets\max(\{j: seq[j].status = F\})$
				\State $\nu\gets |seq|$ 
				
				\State $M \gets \emptyset$

				\For{$i=\mu:\nu$}\label{line:statetransfer:reconfig:start}
				\State  \sout{$t  \gets \dagetdata{\config{seq[i]}}$} 
				\State  $t  \gets \dagettag{\config{seq[i]}}$
				\Statex
				\State \sout{$M  \gets M \cup  \{ \tup{\tg{}, v} \}$} 
				\State $M  \gets M \cup  \{ \tup{t, \config{seq[i]}  } \}$ \label{line:statetransfer:reconfig:end}
				\EndFor
				\Statex
			        \State \sout{$\tup{\tg{},v} \gets \max_{t} \{ \tup{t, v}: \tup{t, v} \in M\}$}
				\State  $\tup{\tg{},C} \gets \max_{t} \{ \tup{t, cfg}: \tup{t, cfg} \in N\}$ \label{line:reconfig:max}
				%\State $\tup{\tg{},v} \gets \text{\act{get-data}}(cseq, \mu, \nu)$
				\Statex
				\Statex ~~~~~/* $ C' \equiv seq[\nu])$ */ 
                                     \State  \sout{$C'.\act{put-data}(\tup{\tg{},v})$} 
                                     \State forward-code-element$(\tg, C, C')$
			
				\EndProcedure
				\Statex
				\Procedure{forward-code-element}{  $\tg{}, C, C'$}
			        \State  Call \act{md-primitive} $( \text{\sc req-fw-code-elem}, \tg{}, C')$ on servers in $C$
				%\State Await {\sc ack}  from a quorum in $C$
				\State {\bf until}  {\sc ack} from $\left\lceil \frac{n' + k'}{2}\right\rceil$ servers in $\servers{C'}$
				\EndProcedure
		}\end{multicols}	
	\end{algorithmic}
	%\hrule \B
	\caption{Alternate \act{update-config} for the  reconfiguration protocol of  \ares.}
	\label{algo:reconfigurer:statetransfer:ares}
	\vspace{-1em}
\end{algorithm}
\begin{algorithm}[!ht]
	%\hrule \F
	\begin{algorithmic}[2]
		\begin{multicols}{2}{\scriptsize
			\State at each server $s_i$ in any configuration 
			\State{\bf Additional State Variables:}
			\Statex $D \subseteq  \mathcal{T} \times \mathcal{C}_s$, initially   $\{(t_0, \Phi_i(v_0))\}$
			\State $Recons$,  set of reconfig client ids, initially empty
			%\State  $\tg{}\in\N \times\wSet$, initially, $\tup{0,\bot}$

			%\State  $msgType\in\{~seen\subseteq\mathcal{V}\cup\{w\}$	
			%\State{\bf Initialization:}
			%\State $\tg{}\gets \tup{0,\bot}, v \gets \bot$
			
			\Statex
			\Statex /*$s_i$ in configuration $C$ */
			\Receiv{{\sc req-fw-code-elem}$, t, C'$}{$s_i$}{$rc$}
			\If{  $(t, e_i) \in List$ }
                                \State Send $(\text{\sc fwd-code-elem}, \tup{\tg{}, e_i}, rc)$ to servers in $C'$
                             \EndIf
			\EndReceiv
			
			\Statex
		%\Statex\Statex\Statex
		%	\Statex\Statex\Statex\Statex
			\Statex /*$s_j'$ in configuration $C'$ */		
			\Receiv{{\sc fwd-code-elem}, $\tup{\tg{},e_i}, rc$}{$s_j'$}{$s_i$}
			
			   \If {$rc \not\in Recons$ } \label{line:statetransfer:notify:check}
			         \If{ $(t, *) \not\in List$} \label{line:statetransfer:notify:checkList}
			               \State $D \gets D \cup \{   \tup{t, e_i}\}$
			               \If{ $\act{isDecodable}(D, t)$} \label{line:statetransfer:notify:decodable}
			                     \State $v \gets \act{decode}(D, t)$ with $\Phi^{-1}_C$
			                       \State $D \gets D \setminus \{   \tup{t, e_i}\} \cup  \{   \tup{t, \bot}\} $
			                     \State $e_j' \gets \Phi_{C'}(v)_j$
				\State $List \gets List \cup \{ \tup{\tg{}, e_j}  \}$ 
				\If{$|List| > \delta+1$}
					\State $\tg{min}\gets\min\{t: \tup{t,*}\in List\}$
                                              \Statex  ~~~~~~~~~~~~~~~~~~~/* remove the coded value, keep the tag */ 
					\State $List \gets List \backslash\{\tup{\tg{},e}: \tg{}=\tg{min} \wedge$
					\Statex ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\tup{\tg{},e}\in List\} \cup \{  (  \tg{min}, \bot)  \}$
				
									%\State $List \gets List \backslash\{\tup{\tg{},e}: \tg{}=\tg{min} ~\wedge~\tup{\tg{},e}\in List\} \cup \{  (  \tg{min}, \bot)  \}$
				%					\State $List \gets List \backslash\{\tup{\tg{},e}: \tg{}=\tg{min} ~\wedge~\tup{\tg{},e}\in List\} \cup \{  (  \tg{min}, \bot)  \}$						
				\EndIf
				
				 \EndIf
                                        \EndIf
				                  
				    \If{ $(t, *) \in List$}     \label{line:statetransfer:notify:begin}        
				                      \State $Recon \gets Recons \cup \{ rc\}$
				                      \State Send ACK to $rc$  \label{line:statetransfer:notify:end}
				     \EndIf
	                   \EndIf
			\EndReceiv
%			\Statex	
%			
%			\Receive{{\sc query-tag}}{$s_i,c_k$} %\Comment{Called upon reception of a message}
%				\State $\act{handle-get-tag(c_k)}$
%				%\State send $\tg{}$ to $q$
%			\EndReceive
%			
%			\Statex
%			
%			\Receive{{\sc query}}{$s_i,c_k$}
%				\State $\act{handle-get-data(c_k)}$
%				%\State send $\tup{\tg{}, v}$ to $q$
%			\EndReceive
%			
%			\Statex
%			
%			\Receive{{\sc write}, $\tup{\tg{in}, v_{in}}$}{$s_i,c_k$}
%				\State $\act{handle-put-data(c_k)}$
%%				\If {$\tg{in}> \tg{}$} 	\label{line:server:tg-comparison}
%%					\State  $\tup{\tg{},v}\gets \tup{\tg{in},v_{in}}$ \label{line:server:update}
%%				\EndIf
%%				\State  send  {\sc ack} to $q$ 	\label{line:server:reply}
%			\EndReceive
%			
		}\end{multicols}	
	\end{algorithmic}
	%\hrule \B
	\caption{Additional server protocol and state-variable at a server in  \treas.}
	\label{algo:server:statetransfer:treas}
	\vspace{-1em}
\end{algorithm}

\begin{theorem}[Atomicity]\label{safety:ares:treas}
	Algorithm \ares-\treas{} implements a reconfigurable atomic storage service, if 
	$\act{get-data}$, $\act{get-tag}$, and $\act{put-data}$ primitives used satisfy 
	\textbf{C1} and \textbf{C2}  of Definition \ref{def:consistency}.
\end{theorem}

%\begin{theorem}
%State when it is live
%\end{theorem}













